Model Checking Contest @ Petri Nets, Report on the 2013 edition

This document presents the results of the Model Checking Contest held at Petri Nets 2013 in Milano. This contest aimed at a fair and experimental evaluation of the performances of model checking techniques applied to Petri nets. This is the third edition after two successful editions in 2011 and 2012. The participating tools were compared on several examinations (state space generation and evaluation of several types of formul{\ae} -- reachability, LTL, CTL for various classes of atomic propositions) run on a set of common models (Place/Transition and Symmetric Petri nets). After a short overview of the contest, this paper provides the raw results from the contest, model per model and examination per examination. An HTML version of this report is also provided (http://mcc.lip6.fr).

==> Makefile <==

build:
	pdflatex mcc-report.tex
	bibtex mcc-report.aux
	pdflatex mcc-report.tex
	pdflatex mcc-report.tex

generate:
	bash export_to_latex.sh -summary_and_scores
	bash export_to_latex.sh -reports
	bash gen_examination_section.sh
	bash gen_performance_section.sh

all: generate build

clean:
	rm -f *.toc *.aux *.synctex.gz *.ind *.ilg *.idx *.blg *.bbl *latexmk *.log *.acn

# all: plot
# 	pdflatex $(MAINLATEX).tex
# 	bibtex $(MAINLATEX)
# 	pdflatex $(MAINLATEX).tex
# 	pdflatex $(MAINLATEX).tex
# 	latex $(MAINLATEX).tex
# 	sh -c 'case `uname -s` in \
# 					 "Darwin") open $(MAINLATEX).pdf ;; \
# 					 "Linux") xpdf $(MAINLATEX).pdf & ;; \
# 					 *) ;; \
# 				 esac'
# 
# plot:
# 	sh generate-charts.sh
# 
# clean:
# 	rm -f mcc-report.pdf
# 	rm -f mcc-report.aux mcc-report.bbl mcc-report.blg mcc-report.cb mcc-report.cb2 mcc-report.dvi mcc-report.fdb_latexmk mcc-report.fls mcc-report.log mcc-report.out mcc-report.synctex.gz
# 	rm -f *~
# 	rm -f sections/*/*.eps sections/*/*-eps-converted-to.pdf


==> StateSpace_handling.tex <==
Table xxx


==> annexes/Makefile <==

build:
	pdflatex mcc-annex1.tex
	pdflatex mcc-annex1.tex
	pdflatex mcc-annex2.tex
	pdflatex mcc-annex2.tex

generate:
	bash export_to_latex.sh -summary_and_scores
	bash export_to_latex.sh -reports
	bash gen_examination_section.sh
	bash gen_performance_section.sh

all: generate build

clean:
	rm -f *.toc *.aux *.synctex.gz *.ind *.ilg *.idx *.blg *.bbl *latexmk *.log *.acn

# all: plot
# 	pdflatex $(MAINLATEX).tex
# 	bibtex $(MAINLATEX)
# 	pdflatex $(MAINLATEX).tex
# 	pdflatex $(MAINLATEX).tex
# 	latex $(MAINLATEX).tex
# 	sh -c 'case `uname -s` in \
# 					 "Darwin") open $(MAINLATEX).pdf ;; \
# 					 "Linux") xpdf $(MAINLATEX).pdf & ;; \
# 					 *) ;; \
# 				 esac'
# 
# plot:
# 	sh generate-charts.sh
# 
# clean:
# 	rm -f mcc-report.pdf
# 	rm -f mcc-report.aux mcc-report.bbl mcc-report.blg mcc-report.cb mcc-report.cb2 mcc-report.dvi mcc-report.fdb_latexmk mcc-report.fls mcc-report.log mcc-report.out mcc-report.synctex.gz
# 	rm -f *~
# 	rm -f sections/*/*.eps sections/*/*-eps-converted-to.pdf


==> annexes/annex_CTLCardinalityComparison.tex <==

\index{Execution!CTLCardinalityComparison}
\input{exec_report_known_CTLCardinalityComparison.tex}
\input{exec_report_surprise_CTLCardinalityComparison.tex}


==> annexes/annex_CTLFireability.tex <==

\index{Execution!CTLFireability}
\input{exec_report_known_CTLFireability.tex}
\input{exec_report_surprise_CTLFireability.tex}


==> annexes/annex_CTLMarkingComparison.tex <==

\index{Execution!CTLMarkingComparison}
\input{exec_report_known_CTLMarkingComparison.tex}
\input{exec_report_surprise_CTLMarkingComparison.tex}


==> annexes/annex_CTLMix.tex <==

\index{Execution!CTLMix}
\input{exec_report_known_CTLMix.tex}
\input{exec_report_surprise_CTLMix.tex}


==> annexes/annex_CTLPlaceComparison.tex <==

\index{Execution!CTLPlaceComparison}
\input{exec_report_known_CTLPlaceComparison.tex}
\input{exec_report_surprise_CTLPlaceComparison.tex}


==> annexes/annex_LTLCardinalityComparison.tex <==

\index{Execution!LTLCardinalityComparison}
\input{exec_report_known_LTLCardinalityComparison.tex}
\input{exec_report_surprise_LTLCardinalityComparison.tex}


==> annexes/annex_LTLFireability.tex <==

\index{Execution!LTLFireability}
\input{exec_report_known_LTLFireability.tex}
\input{exec_report_surprise_LTLFireability.tex}


==> annexes/annex_LTLMarkingComparison.tex <==

\index{Execution!LTLMarkingComparison}
\input{exec_report_known_LTLMarkingComparison.tex}
\input{exec_report_surprise_LTLMarkingComparison.tex}


==> annexes/annex_LTLMix.tex <==

\index{Execution!LTLMix}
\input{exec_report_known_LTLMix.tex}
\input{exec_report_surprise_LTLMix.tex}


==> annexes/annex_LTLPlaceComparison.tex <==

\index{Execution!LTLPlaceComparison}
\input{exec_report_known_LTLPlaceComparison.tex}
\input{exec_report_surprise_LTLPlaceComparison.tex}


==> annexes/annex_ReachabilityCardinalityComparison.tex <==

\index{Execution!ReachabilityCardinalityComparison}
\input{exec_report_known_ReachabilityCardinalityComparison.tex}
\input{exec_report_surprise_ReachabilityCardinalityComparison.tex}


==> annexes/annex_ReachabilityDeadlock.tex <==

\index{Execution!ReachabilityDeadlock}
\input{exec_report_known_ReachabilityDeadlock.tex}
\input{exec_report_surprise_ReachabilityDeadlock.tex}


==> annexes/annex_ReachabilityFireability.tex <==

\index{Execution!ReachabilityFireability}
\input{exec_report_known_ReachabilityFireability.tex}
\input{exec_report_surprise_ReachabilityFireability.tex}


==> annexes/annex_ReachabilityMarkingComparison.tex <==

\index{Execution!ReachabilityMarkingComparison}
\input{exec_report_known_ReachabilityMarkingComparison.tex}
\input{exec_report_surprise_ReachabilityMarkingComparison.tex}


==> annexes/annex_ReachabilityMix.tex <==

\index{Execution!ReachabilityMix}
\input{exec_report_known_ReachabilityMix.tex}
\input{exec_report_surprise_ReachabilityMix.tex}


==> annexes/annex_ReachabilityPlaceComparison.tex <==

\index{Execution!ReachabilityPlaceComparison}
\input{exec_report_known_ReachabilityPlaceComparison.tex}
\input{exec_report_surprise_ReachabilityPlaceComparison.tex}


==> annexes/annex_StateSpace.tex <==

\index{Execution!StateSpace}
\input{exec_report_known_StateSpace.tex}
\input{exec_report_surprise_StateSpace.tex}


==> annexes/exec_report_CTLCardinalityComparison.tex <==



==> annexes/exec_report_CTLFireability.tex <==



==> annexes/exec_report_CTLMarkingComparison.tex <==



==> annexes/exec_report_CTLMix.tex <==



==> annexes/exec_report_CTLPlaceComparison.tex <==



==> annexes/exec_report_LTLCardinalityComparison.tex <==



==> annexes/exec_report_LTLFireability.tex <==



==> annexes/exec_report_LTLMarkingComparison.tex <==



==> annexes/exec_report_LTLMix.tex <==



==> annexes/exec_report_LTLPlaceComparison.tex <==



==> annexes/exec_report_ReachabilityCardinalityComparison.tex <==



==> annexes/exec_report_ReachabilityDeadlock.tex <==



==> annexes/exec_report_ReachabilityFireability.tex <==



==> annexes/exec_report_ReachabilityMarkingComparison.tex <==



==> annexes/exec_report_ReachabilityMix.tex <==



==> annexes/exec_report_ReachabilityPlaceComparison.tex <==



==> annexes/exec_report_known_CTLCardinalityComparison.tex <==

\section{Executions Reported for CTLCardinalityComparison  (``Known'' models)}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500319_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500320_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{680.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{208.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500321_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1404.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500322_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1508.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500323_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1521.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500324_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2170.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1919.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301433_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301434_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301435_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301436_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{89.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301437_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1048.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301438_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1055.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301439_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1396.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301440_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{462.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100242_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{319.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100243_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501433_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501434_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501435_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501436_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1039.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501437_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1156.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501438_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1358.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{513.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501439_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1809.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2198.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501440_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101075_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101076_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{350.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{287.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101077_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{677.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1687.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101078_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101079_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{562.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101080_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{621.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600319_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{890.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600320_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600321_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600322_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600323_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600324_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100638_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100639_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100640_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{719.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{310.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100641_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{888.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100642_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2219.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{931.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100643_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1725.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1291.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100644_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100645_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{132.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100646_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100647_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{500.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548100648_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138401438_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1083.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{351.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138401439_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2058.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1323.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138401440_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2594.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{136.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905800535_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905800536_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{166.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905800537_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1707.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{284.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905800538_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905800539_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{409.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905900540_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800115_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{263.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{188.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{375.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200157_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200158_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{33.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200159_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1093.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200160_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1263.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200161_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1563.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941740600162_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{833.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200215_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200216_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2871.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{107.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800082_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800083_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{311.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800084_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800085_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{212.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800086_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{641.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800087_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800088_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{211.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800089_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800090_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{109.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100157_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100158_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100159_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100160_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1100.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100161_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1831.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100162_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2325.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200209_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200210_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200211_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1383.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{235.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200212_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2112.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{267.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200213_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1340.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200214_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200215_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{142.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200216_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300089_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400090_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{485.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900209_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900210_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{624.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{54.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900211_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{218.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900212_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{197.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900213_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900214_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{359.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900215_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{441.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900216_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500134_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500135_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500136_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500137_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500138_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500139_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500140_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700157_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{246.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700158_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{287.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700159_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{65.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700160_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700161_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700162_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{55.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000372_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000373_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{213.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000374_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{348.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{52.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000375_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3064.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1997.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000376_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{948.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{578.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000377_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2692.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000378_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{127.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300115_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{618.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{318.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{483.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{328.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700319_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700320_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700321_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700322_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{506.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700323_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700324_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{117.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530700230_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530700231_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530700232_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{751.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530700233_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530700234_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530700235_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530700236_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{226.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530700237_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{279.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530800238_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2742.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2231.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530800239_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1396.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530800240_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{918.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132300214_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132300215_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132300216_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{460.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700158_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700159_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{193.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{32.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700160_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{304.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700161_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1716.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700162_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600136_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600137_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600138_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600139_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600140_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700141_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700142_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1392.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700143_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{154.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700144_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700145_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700146_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700147_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700148_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700149_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700150_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1281.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700339_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700340_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700341_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700342_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700343_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700345_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700346_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700347_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700349_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700350_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700351_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897600195_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897600196_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{423.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{135.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897700197_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897700198_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897700199_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{906.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{164.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897700200_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2871.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{615.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000293_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000294_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000295_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000296_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000297_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1267.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500319_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500320_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{263.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{181.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500321_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500322_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{366.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500323_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500324_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700259_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700260_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700261_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1092.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700262_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1258.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700263_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1570.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700264_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{830.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400351_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400352_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2873.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{106.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200235_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200236_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{308.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200237_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2839.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300238_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{199.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300239_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{622.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300240_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{157.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300241_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{205.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300242_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300243_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{85.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300259_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400260_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400261_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400262_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1064.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400263_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1805.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400264_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2280.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400345_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400346_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400347_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1383.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{245.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2113.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{272.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400349_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1306.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400350_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400351_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{150.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400352_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600242_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600243_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{481.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400345_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400346_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{624.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{61.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400347_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{242.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{206.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400349_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400350_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{407.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400351_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{445.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400352_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900372_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900373_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900374_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900375_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900376_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900377_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900378_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200259_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{246.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200260_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{305.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200261_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{71.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200262_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200263_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200264_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{53.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700610_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700611_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{213.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{348.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700613_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3064.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1979.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700614_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{948.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{591.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2690.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{126.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900319_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900320_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{680.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900321_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900322_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{308.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900323_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{471.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900324_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{336.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400523_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400524_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400525_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{502.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{118.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533300638_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533400639_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533400640_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{851.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533400641_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533400642_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533400643_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533400644_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{226.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533400645_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{293.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533400646_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2742.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2247.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533400647_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1358.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533400648_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133000350_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133000351_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133100352_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{461.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000260_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000261_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{193.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{38.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000262_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{302.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000263_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1725.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000264_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800391_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800392_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800393_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800394_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800395_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800396_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800397_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1562.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028900398_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028900399_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028900400_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028900401_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028900402_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028900403_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028900404_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028900405_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1299.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100561_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100562_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100563_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100564_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100565_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100566_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100567_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100568_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100569_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100570_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100571_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100572_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898800535_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898800536_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{423.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{150.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898800537_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898800538_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898800539_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{906.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{161.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898800540_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{599.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926100480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926100481_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926100482_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926100483_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926100484_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1279.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200523_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200524_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{363.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{39.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200525_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200526_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{694.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200527_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200528_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200361_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{263.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200362_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300363_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1281.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300364_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1227.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300365_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1527.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300366_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1027.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700487_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{277.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700488_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2870.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{113.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700388_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800389_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800390_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800391_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800392_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800393_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800394_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800395_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{278.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800396_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700361_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{246.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700362_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{237.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700363_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700364_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700365_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700366_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600481_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{243.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600482_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600483_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{657.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{41.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600484_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{89.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600485_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2843.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600486_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{244.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600487_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{314.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{872.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600488_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800395_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800396_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{757.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800481_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800482_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{352.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800483_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1601.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{325.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800484_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{183.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800485_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800486_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{351.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800487_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1756.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800488_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400610_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400611_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400612_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400613_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400614_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400615_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400616_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600361_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{402.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600362_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{144.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600363_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600364_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{250.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600365_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{260.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600366_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400848_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400849_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{364.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400850_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{347.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{60.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400851_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{517.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400852_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{948.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{610.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400853_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2702.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400854_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400523_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400524_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400525_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400526_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400527_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400528_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100727_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100728_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100729_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100730_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{313.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100731_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100732_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{117.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536301046_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536401047_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536401048_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{473.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536401049_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536401050_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536401051_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536401052_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{227.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536401053_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{293.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536401054_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2741.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2193.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536401055_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1386.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536401056_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{994.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133800486_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133800487_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133800488_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{543.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200362_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{250.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200363_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{352.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300364_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{671.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300365_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2644.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300366_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300646_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300647_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300648_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300649_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{276.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300650_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300651_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300652_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{446.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030400653_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030400654_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030400655_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030400656_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030400657_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030400658_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030400659_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030400660_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{515.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500781_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{224.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500782_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{244.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500783_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500784_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{275.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500785_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500786_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{264.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500787_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500788_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500789_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500790_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{268.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{315.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500793_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{358.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900000875_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900000876_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{317.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{56.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900000877_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900000878_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900000879_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{906.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{156.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900000880_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{606.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200667_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{270.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200668_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200669_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1825.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200670_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1317.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200671_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{783.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000727_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000728_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000729_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000730_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{99.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000731_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000732_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800463_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800464_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800465_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{116.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800466_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800467_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800468_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{379.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900623_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2873.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{104.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300541_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300542_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{946.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300543_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1443.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300544_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300545_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300546_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{942.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300547_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2187.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300548_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300549_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2100.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000463_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000464_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000465_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000466_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000467_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000468_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900617_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900618_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900619_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900620_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900621_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900622_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900623_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100548_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{115.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100549_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{477.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{194.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300617_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300618_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300619_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300620_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300621_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300622_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300623_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900848_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900849_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900850_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900851_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900852_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900853_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900854_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200463_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200464_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200465_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{206.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200466_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200467_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200468_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{930.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101086_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101087_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{147.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{46.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101088_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{346.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{65.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101089_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1476.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101090_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{948.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{581.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101091_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2689.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101092_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{387.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900727_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900728_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{275.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900729_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900730_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{338.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900731_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{434.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900732_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900931_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900932_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900933_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900934_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2224.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900935_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900936_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{118.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539201454_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539201455_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539201456_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{729.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539201457_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539201458_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539201459_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539201460_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{226.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539201461_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{292.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539201462_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2742.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2141.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539301463_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1401.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539301464_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1043.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134600622_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134600623_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134600624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{413.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500464_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500465_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500466_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{727.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500467_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{260.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500468_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{96.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900901_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900902_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900903_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900904_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900905_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900906_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900907_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{200.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{655.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900908_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1223.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900909_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900910_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900911_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900912_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900913_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900914_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900915_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901002_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901003_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901004_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901005_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901006_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901007_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901008_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{503.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901009_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1438.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901010_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901011_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901012_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901013_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{209.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901014_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901501215_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901501216_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1854.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901501217_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901501218_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901501219_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{906.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{209.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901501220_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{594.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928200854_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928200855_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928200856_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{272.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928200857_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928200858_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{144.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700115_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700116_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700117_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700118_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700119_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700120_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800667_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800668_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119900669_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119900670_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119900671_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{751.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119900672_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{928.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309400895_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309400896_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1331.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{157.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800082_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{933.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800083_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800084_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800085_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800086_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{870.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800087_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1131.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800088_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800089_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{942.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800090_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1110.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600667_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600668_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600669_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600670_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600671_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600672_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300889_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300890_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300891_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300892_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300893_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{861.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300894_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2405.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1507.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300895_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2385.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300896_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1993.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151900089_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151900090_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1016.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200889_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200890_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200891_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200892_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200893_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1819.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{61.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200894_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200895_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200896_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700134_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700135_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700136_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{727.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{56.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700137_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{854.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700138_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700139_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700140_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{864.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900667_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900668_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900669_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{680.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900670_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{845.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900671_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900672_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2009.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801562_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801563_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801564_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801565_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{949.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801566_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1151.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801567_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801568_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{144.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200115_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{682.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{56.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200116_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{804.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200117_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{805.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200118_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200119_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1289.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2408.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200120_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1287.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601339_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601340_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{838.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{53.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601341_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701342_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701343_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701344_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525500230_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525600231_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525600232_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525600233_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525600234_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{681.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525600235_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{735.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525600236_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{67.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525600237_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1101.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525600238_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1213.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2514.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525600239_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1290.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525600240_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135800894_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135800895_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135800896_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{772.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100668_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100669_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{716.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100670_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100671_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100672_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{709.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900136_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900137_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900138_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900139_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900140_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900141_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900142_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900143_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{672.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900144_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{697.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900145_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900146_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900147_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900148_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900149_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900150_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{714.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801444_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{671.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801445_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801446_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801447_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801448_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801449_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{62.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801450_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801451_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801452_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801453_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1177.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801454_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801455_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801456_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{92.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500195_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500196_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500197_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500198_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500199_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{146.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500200_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930301228_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930301229_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930301230_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1123.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1363.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930301231_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1112.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930301232_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700931_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700932_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700933_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700934_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800935_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800936_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400565_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400566_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400567_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400568_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400569_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400570_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100759_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100760_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900694_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900695_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900696_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900697_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900698_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900699_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900700_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900701_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900702_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300565_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300566_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300567_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300568_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300569_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300570_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100753_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100754_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100755_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100756_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100757_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100758_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100759_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100760_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153500701_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153500702_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700753_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700754_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700755_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700756_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700757_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700758_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700759_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700760_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401086_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401087_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401088_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401089_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401090_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401091_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401092_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600565_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600566_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600567_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600568_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600569_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600570_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901324_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901325_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{96.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901326_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{343.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901327_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{246.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{63.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901328_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{931.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{571.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901329_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2627.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901330_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500931_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500932_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500933_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500934_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500935_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500936_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801135_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801136_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801137_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801138_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801139_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801140_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{114.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542101862_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542101863_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542101864_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542101865_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542101866_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542101867_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542201868_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{226.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542201869_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{800.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{291.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542201870_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2741.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2225.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542201871_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1462.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542201872_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1051.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135100758_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135200759_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135200760_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800566_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800567_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800568_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800569_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800570_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301156_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301157_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301158_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301159_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301160_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301161_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301162_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301163_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301164_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301165_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301166_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301167_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301168_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301169_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301170_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401223_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401224_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401225_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401226_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401227_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401228_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401229_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401230_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{74.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401231_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401232_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401233_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401234_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401235_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902601555_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902601556_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902601557_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902601558_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902601559_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902601560_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929401041_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929401042_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929401043_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929401044_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929401045_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_CTLFireability.tex <==

\section{Executions Reported for CTLFireability  (``Known'' models)}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!CTLFireability}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400295_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400296_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{241.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400297_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1370.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400298_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1508.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400299_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1579.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1573.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400300_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2170.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2275.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301417_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301418_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301419_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301420_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301421_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{160.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301422_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{545.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{163.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301423_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1400.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301424_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{461.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100224_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{341.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100225_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401417_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401418_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401419_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401420_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1072.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401421_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{823.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{262.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401422_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1358.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{515.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401423_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1810.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2202.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401424_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{238.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001063_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001064_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{268.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001065_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{440.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001066_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001067_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{562.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001068_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{621.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500295_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{896.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500296_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500297_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500298_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500299_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500300_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547700590_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547700591_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547700592_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{786.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{240.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547800593_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1613.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{249.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547800594_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1620.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{257.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547800595_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1650.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{283.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547800596_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547800597_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{134.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547800598_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{227.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547800599_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{503.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547800600_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138301422_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1080.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{363.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138301423_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2062.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1088.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138301424_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2594.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{160.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905700495_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905700496_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905700497_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1706.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{299.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905700498_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{134.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905700499_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{409.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905700500_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901602133_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901602134_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1746.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901602135_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1890.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{88.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901602136_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!CTLFireability}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800091_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800092_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{167.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800093_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{401.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800094_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{176.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800095_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800096_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{685.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100145_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100146_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100147_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100148_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100149_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200150_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{728.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200199_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200200_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2907.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{163.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700064_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700065_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700066_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700067_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700068_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700069_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700070_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700071_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700072_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000145_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000146_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000147_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000148_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000149_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000150_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200193_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200194_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200195_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200196_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200197_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200198_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200199_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200200_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300071_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300072_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1757.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{421.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800193_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800194_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900195_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900196_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900197_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900198_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900199_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900200_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400106_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400107_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400108_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400109_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400110_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400111_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400112_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600145_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600146_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600147_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600148_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600149_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600150_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900345_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{202.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{66.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900346_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900347_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{471.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900349_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900350_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1561.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300091_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300092_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300093_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300094_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300095_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300096_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600295_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600296_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600297_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600298_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{873.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600299_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{461.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600300_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530400182_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530400183_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530400184_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530400185_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530400186_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{120.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530500187_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{199.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530500188_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530500189_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530500190_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{82.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530500191_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{160.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{164.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530500192_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2813.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{670.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132200198_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132200199_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132200200_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{762.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700146_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700147_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{194.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{48.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700148_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700149_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700150_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1381.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500106_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500107_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500108_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500109_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500110_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500111_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500112_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500113_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500114_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500115_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600313_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600314_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600315_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600316_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600317_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600318_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600319_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600320_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600321_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600322_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600323_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600324_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700325_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500155_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500156_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500157_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500158_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1678.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500159_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1256.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500160_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{485.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900271_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000273_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1456.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000274_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000275_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2002.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895100297_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895100298_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895100299_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{867.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895100300_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{33.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!CTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400295_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400296_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{166.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400297_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{411.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400298_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{181.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400299_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400300_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{766.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600247_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600248_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600249_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600250_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600251_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941740800252_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{728.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2913.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{139.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200217_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200218_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200219_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200220_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200221_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200222_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200223_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200224_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200225_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300247_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300248_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300249_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300250_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300251_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300252_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400329_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400330_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400331_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400332_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400333_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600224_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600225_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1755.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{488.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300329_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300330_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300331_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300332_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300333_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800344_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800345_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800346_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900347_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900348_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900349_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900350_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100247_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100248_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100249_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100250_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100251_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100252_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600582_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600583_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{202.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{66.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600584_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600585_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600586_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{457.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600587_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600588_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1562.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800295_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800296_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800297_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800298_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800299_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800300_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300499_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300500_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300501_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300502_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{853.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300503_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{477.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300504_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000590_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000591_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000592_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000593_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000594_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{138.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000595_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{195.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000596_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000597_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{52.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000598_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{82.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000599_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{159.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{176.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533000600_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2815.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{669.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133000334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133000335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133000336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{773.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000248_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000249_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{194.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000250_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000251_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000252_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1375.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700361_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700362_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700363_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700364_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700365_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700366_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700367_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700368_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700369_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700370_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700371_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700372_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700373_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700374_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700375_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000534_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000535_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000536_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000537_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000538_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000539_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000540_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000541_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000542_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000543_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000544_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000545_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000546_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700495_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700496_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700497_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700498_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1543.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700499_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1145.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700500_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{480.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926000458_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926000459_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926000460_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1433.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926000461_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926000462_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1999.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895800501_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895800502_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895800503_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{867.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895800504_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!CTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100499_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100500_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{330.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100501_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1034.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100502_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{616.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100503_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100504_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{316.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200349_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{268.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200350_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{265.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200351_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200352_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200353_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{317.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200354_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{956.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600471_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{247.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600472_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2898.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{146.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700370_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700371_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700372_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700373_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700374_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700375_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700376_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700377_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700378_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600349_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600350_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600351_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600352_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{225.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600353_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{264.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600354_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{236.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600465_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{216.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600466_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{223.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600467_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{271.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600468_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{251.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600469_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600470_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{228.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600471_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{253.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600472_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{238.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800377_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{314.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800378_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1874.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{319.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800465_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{288.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800466_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{248.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800467_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{232.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800468_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{263.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800469_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{248.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800470_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800471_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{255.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800472_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400582_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400583_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400584_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400585_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400586_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400587_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400588_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600349_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600350_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{272.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600351_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{271.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600352_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{253.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600353_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{242.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600354_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{286.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300820_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300821_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{53.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300822_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300823_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{327.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300824_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{350.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300825_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{334.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300826_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{483.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300499_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300500_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{283.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300501_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300502_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300503_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300504_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{283.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000703_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{248.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000704_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{258.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000705_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{280.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000706_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{305.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000707_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{322.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000708_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536000998_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{280.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536000999_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536001000_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536001001_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536001002_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{107.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536101003_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{851.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536101004_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536101005_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{114.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536101006_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{348.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536101007_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{425.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{169.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536101008_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2560.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{866.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133700470_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{246.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133700471_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{322.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133700472_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{918.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200350_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{264.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200351_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{352.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200352_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{221.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200353_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1924.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200354_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{826.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100616_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200617_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200618_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200619_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200620_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200621_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200622_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200623_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{288.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200624_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200625_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200626_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200627_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200628_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200629_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200630_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400755_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{244.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400756_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400757_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{232.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400758_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{264.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400759_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{288.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400760_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400761_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400762_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400763_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{242.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400764_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400765_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400766_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{315.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400767_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900835_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900836_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900837_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900838_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1598.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900839_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900840_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{480.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200645_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{237.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200646_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200647_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2829.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200648_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200649_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{960.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896400705_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{236.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896400706_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896400707_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{357.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896400708_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{40.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!CTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900703_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900704_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900705_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{229.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900706_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900707_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900708_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700451_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700452_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{134.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700453_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{134.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700454_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700455_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700456_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{379.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900607_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900608_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2913.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{137.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200523_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2465.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200524_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{946.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200525_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1468.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200526_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1616.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200527_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200528_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200529_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2209.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200530_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{987.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200531_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2231.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900451_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900452_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900453_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900454_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900455_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900456_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800601_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800602_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800603_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800604_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800605_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800606_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800607_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800608_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100530_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{122.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100531_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1756.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{335.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200601_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200602_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200603_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200604_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{627.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200605_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200606_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200607_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200608_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900820_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900821_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900822_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900823_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900824_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900825_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900826_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100451_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100452_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100453_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{443.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100454_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{589.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100455_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100456_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{957.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001058_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001059_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{84.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{167.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001060_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1780.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001061_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1401.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001062_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{554.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001063_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{515.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001064_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{404.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800703_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800704_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{247.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900705_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{238.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900706_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{325.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900707_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{392.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900708_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800907_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800908_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800909_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800910_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1758.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800911_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800912_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538901406_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538901407_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538901408_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538901409_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538901410_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{884.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538901411_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538901412_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539001413_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539001414_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{86.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539001415_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{166.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539001416_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{206.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134500606_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134500607_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{73.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{717.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134500608_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{778.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500452_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500453_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500454_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500455_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{254.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500456_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{95.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700871_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700872_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700873_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700874_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700875_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700876_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{47.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700877_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700878_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1198.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700879_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1702.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800880_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800881_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800882_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800883_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800884_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800885_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800976_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2387.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900977_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900978_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900979_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900980_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900981_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900982_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{900.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900983_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900984_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900985_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900986_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900987_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{92.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900988_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{439.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901301175_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901301176_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{852.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901301177_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901301178_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{117.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901301179_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901301180_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{476.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928000832_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928000833_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928000834_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{210.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1638.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928000835_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928000836_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{84.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897100909_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897100910_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897100911_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{131.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897100912_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!CTLFireability}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700091_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700092_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1243.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{396.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700093_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700094_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700095_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700096_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800655_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800657_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{792.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800658_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800659_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{751.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800660_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{929.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309400879_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309400880_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1467.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{492.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700064_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700065_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1104.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700066_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700067_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700068_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{870.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700069_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1105.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700070_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700071_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700072_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1110.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600655_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{661.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600657_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600658_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600659_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{887.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600660_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{718.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300873_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300874_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300875_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300876_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300877_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300878_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2550.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1882.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300879_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2298.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300880_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1993.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800071_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{117.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800072_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1080.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100873_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100874_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100875_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100876_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1006.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100877_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100878_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100879_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100880_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600106_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600107_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{733.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600108_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1168.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1096.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600109_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{854.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600110_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{831.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600111_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700112_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800655_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800657_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{799.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800658_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1577.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{57.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800659_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800660_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2009.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701534_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701535_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701536_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701537_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701538_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1151.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701539_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{105.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701540_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{144.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200091_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{903.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{194.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200092_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{804.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200093_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200094_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200095_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1290.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2612.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200096_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1294.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2413.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501315_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501316_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501317_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501318_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601319_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{771.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601320_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300182_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300183_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300184_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300185_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1155.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{83.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300186_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1157.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300187_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300188_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1169.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300189_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300190_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{99.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300191_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1288.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525300192_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{354.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135700878_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135700879_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{710.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135700880_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{805.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000657_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000658_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{724.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000659_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000660_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700106_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700107_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700108_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700109_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800110_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800111_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{677.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800112_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800113_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1173.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800114_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{738.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800115_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800116_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800117_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{671.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800118_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{695.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800119_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800120_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1181.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701418_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{705.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701419_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701420_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701421_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701422_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701423_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701424_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{788.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1193.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701425_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{989.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701426_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701427_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1178.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701428_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701429_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701430_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{98.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895300155_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895300156_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895300157_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895400158_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895400159_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1201.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895400160_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930101206_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930101207_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930101208_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930101209_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1111.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930101210_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1077.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898501317_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898501318_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{713.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898501319_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{725.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898501320_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1607.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!CTLFireability}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700907_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700908_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700909_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700910_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2862.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700911_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2862.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700912_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{149.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300553_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300554_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300555_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300556_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300557_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300558_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{188.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100743_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2867.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100744_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1132.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800676_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800677_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{536.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800678_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2260.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800679_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1374.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800680_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800681_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{74.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800682_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800683_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800684_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{113.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200553_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200554_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200555_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200556_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200557_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200558_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000737_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000738_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100739_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100740_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100741_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100742_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100743_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100744_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153400683_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153400684_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{397.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1047.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700737_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700738_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700739_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700740_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700741_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700742_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700743_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700744_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401058_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401059_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401060_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401061_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401062_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401063_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401064_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500553_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500554_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500555_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{472.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500556_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500557_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500558_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801296_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801297_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801298_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801299_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{79.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801300_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2873.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{55.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801301_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{159.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{82.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801302_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1300.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{154.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400907_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400908_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400909_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400910_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{141.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400911_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400912_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701111_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{119.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701112_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1121.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701113_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701114_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{844.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701115_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2867.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701116_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2870.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2378.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801814_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801815_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801816_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801817_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801818_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801819_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{64.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801820_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{277.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{347.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801821_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{373.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801822_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{75.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801823_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{139.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541801824_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{245.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135100742_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{557.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135100743_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135100744_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{156.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700554_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700555_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700556_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700557_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800558_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101126_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101127_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101128_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101129_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101130_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101131_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101132_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101133_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101134_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201135_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201136_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201137_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201138_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{437.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201139_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{429.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201140_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301197_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301198_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301199_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301200_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301201_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301202_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301203_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301204_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301205_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301206_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301207_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301208_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301209_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{97.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501515_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501516_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501517_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501518_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501519_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{109.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501520_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{413.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{224.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929201019_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{79.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929301020_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2508.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929301021_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929301022_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{67.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929301023_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{783.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897801113_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2468.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897801114_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897801115_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{91.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897801116_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{937.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_CTLMarkingComparison.tex <==

\section{Executions Reported for CTLMarkingComparison  (``Known'' models)}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500331_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500332_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500333_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{365.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{52.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500334_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1508.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500335_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1579.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1588.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500336_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2170.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2125.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100251_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{312.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100252_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600331_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{209.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600332_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600333_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600334_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600335_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600336_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548200662_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548200663_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548200664_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548200665_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548300666_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548300667_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548300668_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548300669_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548300670_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{217.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548300671_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{499.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548300672_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138401446_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138401447_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{797.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138401448_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2592.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{159.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905900555_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905900556_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905900557_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1707.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{273.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905900558_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{128.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905900559_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{410.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905900560_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901802169_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901802170_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{397.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901802171_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1888.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{85.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901802172_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900127_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900128_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900129_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1331.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900130_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{578.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900131_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900132_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{401.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200223_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200224_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{61.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400098_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400099_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{512.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500148_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500149_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500150_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500151_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500152_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500153_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500154_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000386_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000387_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100388_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1142.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100389_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100390_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100391_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{108.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2317.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400127_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400128_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400129_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400130_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{694.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400131_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1509.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400132_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{906.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700331_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700332_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{641.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700333_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{628.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{603.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{788.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{625.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900254_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900255_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900256_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{160.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900257_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{68.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900258_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{84.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900259_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{177.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900260_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900261_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{252.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900262_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2867.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{96.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900263_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{182.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{113.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530900264_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2893.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{723.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132300222_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132300223_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{201.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132300224_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{457.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897700215_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897700216_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{414.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{93.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897700217_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{901.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897700218_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1316.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897700219_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1802.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897700220_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2898.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{617.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925100304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925100305_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925100306_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925100307_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2416.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925100308_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2181.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895200333_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895200334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895200335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{76.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895200336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500331_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500332_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500333_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1408.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500334_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{665.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500335_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500336_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{387.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500359_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500360_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600251_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600252_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{515.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900386_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900387_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900388_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900389_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900390_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900391_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900392_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700625_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700626_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1135.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700627_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700628_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873700629_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{108.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800630_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2322.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900331_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900332_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900333_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900334_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{685.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900335_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1517.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900336_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{964.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400535_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400536_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{641.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400537_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{609.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400538_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{592.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400539_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{785.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400540_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{614.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600662_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600663_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600664_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{159.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600665_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600666_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{100.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600667_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{199.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600668_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{146.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600669_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{277.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600670_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2871.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{68.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600671_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{182.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{133.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533600672_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2903.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{778.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133100358_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133100359_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{188.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133100360_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{457.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898900555_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898900556_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{414.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{106.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898900557_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{845.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898900558_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1235.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898900559_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1888.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898900560_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2898.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{596.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926200491_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926200492_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926200493_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926200494_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2384.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926200495_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2179.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895900537_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895900538_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895900539_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{76.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895900540_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200535_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200536_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200537_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1697.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200538_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200539_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{277.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851200540_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700495_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{279.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700496_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800404_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{307.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800405_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{780.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400624_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500625_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500626_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500627_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500628_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500629_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500630_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400862_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400863_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400864_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400865_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400866_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{317.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400867_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{367.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400868_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400535_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400536_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400537_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400538_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400539_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400540_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100739_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100740_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100741_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100742_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100743_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{321.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100744_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{378.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501070_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501071_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501072_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{328.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501073_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{319.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501074_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{176.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501075_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{303.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501076_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2609.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501077_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{449.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501078_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2871.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{186.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501079_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{447.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{145.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536501080_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2888.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{588.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133900494_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133900495_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{199.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133900496_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{595.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900100895_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900100896_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{315.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900100897_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1528.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900100898_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1830.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900100899_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1291.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900100900_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2903.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{598.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927300678_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927300679_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{246.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927300680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927300681_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{930.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927300682_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1080.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896500741_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896500742_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896500743_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{341.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896500744_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{738.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000739_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000740_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000741_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000742_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{102.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000743_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{194.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852000744_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900631_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900632_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2875.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100557_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{115.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100558_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{286.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000862_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000863_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000864_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000865_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000866_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000867_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000868_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201100_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201101_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{85.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{229.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201102_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1727.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201103_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1411.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201104_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{725.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201105_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{463.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201106_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{384.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000739_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000740_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000741_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000742_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{332.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000743_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{430.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000744_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{675.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900943_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900944_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900945_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1346.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900946_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2096.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900947_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890900948_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401478_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401479_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401480_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{684.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401481_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1067.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401482_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{935.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401483_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{243.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401484_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401485_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401486_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{91.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401487_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{166.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539401488_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{280.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134600630_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134600631_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1198.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134600632_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{420.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601235_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601236_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1713.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601237_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601238_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601239_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1063.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601240_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2902.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{603.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928200865_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928200866_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928200867_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{210.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928200868_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{279.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928200869_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{152.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897300945_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897300946_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897300947_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897300948_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{604.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800127_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800128_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800129_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800130_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800131_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800132_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1142.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309400903_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309400904_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1331.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{166.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151900098_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{38.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151900099_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{505.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{39.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700148_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700149_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700150_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{759.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{65.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700151_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{851.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700152_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700153_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700154_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{864.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801576_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801577_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{800.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801578_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801579_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{949.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801580_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1151.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801581_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1186.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876901582_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1195.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300127_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{683.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{71.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300128_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{790.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300129_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{804.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300130_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300131_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1289.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2499.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300132_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1287.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701351_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701352_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701353_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{744.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701354_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701355_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701356_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700254_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700255_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700256_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700257_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700258_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{681.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700259_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{735.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700260_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{91.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700261_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700262_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{99.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700263_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1289.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525700264_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135800902_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135800903_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135800904_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{157.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500215_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500216_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500217_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500218_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500219_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1206.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895500220_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{28.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930401239_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930401240_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930401241_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1123.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1362.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930401242_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930401243_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1079.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898601353_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898601354_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898601355_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{702.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898601356_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1154.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800943_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800944_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800945_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800946_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800947_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800948_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200767_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{844.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200768_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{551.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153500710_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153500711_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{344.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501100_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501101_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501102_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501103_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501104_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501105_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501106_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001338_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001339_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001340_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001341_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001342_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001343_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001344_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{179.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{377.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600943_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600944_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600945_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600946_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600947_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{673.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600948_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801147_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801148_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801149_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801150_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801151_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891901152_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2882.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2268.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542301886_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542301887_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{705.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542301888_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542301889_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542301890_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542301891_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542301892_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542301893_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{87.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542401894_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542401895_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542401896_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135200766_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135200767_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2608.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135200768_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{385.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701575_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701576_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701577_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701578_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701579_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701580_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{408.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929401052_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929401053_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{220.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929401054_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929401055_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929501056_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2862.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{77.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897901149_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1688.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897901150_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897901151_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897901152_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_CTLMix.tex <==

\section{Executions Reported for CTLMix  (``Known'' models)}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!CTLMix}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500343_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500344_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500345_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1509.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854500346_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1568.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854600347_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1579.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1778.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854600348_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2187.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1958.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301449_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435401450_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435401451_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435401452_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{117.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435401453_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{443.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435401454_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1297.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{354.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435401455_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1397.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435401456_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{461.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154200260_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{345.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154200261_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501449_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501450_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501451_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501452_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{565.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{253.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501453_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1076.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501454_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1358.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{517.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501455_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1809.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2212.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571501456_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101087_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101088_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101089_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{504.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101090_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101091_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{562.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101092_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{621.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600343_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{896.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600344_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600345_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600346_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600347_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892600348_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548400686_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548400687_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548400688_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{818.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{332.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548400689_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1624.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{520.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548400690_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1642.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{234.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548400691_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1651.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{264.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548400692_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548400693_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{125.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548400694_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{213.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548500695_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{500.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548500696_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138501454_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1077.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{227.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138501455_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2046.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1106.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138501456_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2592.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{122.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906000575_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906000576_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{102.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906000577_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1706.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{297.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906000578_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{134.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906000579_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{411.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906000580_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901802181_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901802182_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1774.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901802183_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1890.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{95.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901802184_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!CTLMix}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900139_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900140_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{220.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{94.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900141_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1139.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900142_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{449.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900143_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849900144_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200169_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200170_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200171_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{879.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1737.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200172_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300173_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2250.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300174_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{636.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300231_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300232_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2901.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800100_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{38.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800101_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800102_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{153.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800103_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{118.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800104_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800105_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{411.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800106_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800107_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800108_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100169_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100170_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100171_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100172_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100173_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100174_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1672.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200225_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200226_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200227_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{882.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{98.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200228_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200229_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200230_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{265.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200231_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200232_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{124.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400107_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{320.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400108_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{472.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900225_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000226_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{954.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{84.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000227_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{282.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000228_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000229_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{156.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000230_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{165.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000231_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2844.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{113.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000232_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{158.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500162_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500163_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500164_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500165_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500166_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500167_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500168_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700169_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700170_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{98.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700171_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{246.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700172_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{74.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700173_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{189.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700174_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100400_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100401_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100402_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{229.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100403_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3209.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2245.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100404_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1272.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1196.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1932.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400139_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400140_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{431.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400141_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{204.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400142_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400143_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1683.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400144_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{796.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700343_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700345_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888700346_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{209.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800347_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2889.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{196.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531000278_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531000279_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531000280_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{254.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531000281_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531000282_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531000283_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531000284_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{176.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531000285_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{383.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{114.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531000286_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3367.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{471.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531000287_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1391.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531100288_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{976.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132400230_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132400231_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{143.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132400232_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{461.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800170_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800171_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{186.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{42.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800172_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{308.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800173_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800174_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1762.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027700166_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800167_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800168_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800169_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800170_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800171_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800172_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{279.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800173_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{949.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800174_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800175_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800176_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800177_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800178_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800179_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{421.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800180_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{418.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700365_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{171.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700366_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700367_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700368_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700369_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700370_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700371_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700372_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700373_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700374_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700375_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700376_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700377_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897800235_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897800236_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{413.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{137.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897800237_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{507.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897800238_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897800239_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{902.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{211.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897800240_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2883.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{623.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925100315_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925100316_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925100317_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925100318_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2306.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925100319_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2512.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895300345_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895300346_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895300347_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{868.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895300348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!CTLMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500343_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500344_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{220.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{104.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500345_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1205.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500346_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{402.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850500347_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600348_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700271_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800273_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{879.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1714.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800274_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800275_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2253.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800276_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{641.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500367_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500368_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2904.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{94.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300253_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2841.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300254_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300255_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{139.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300256_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{108.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300257_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300258_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{386.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300259_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300260_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300261_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400271_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400273_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400274_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400275_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400276_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1688.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400361_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400362_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400363_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{882.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{111.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500364_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500365_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500366_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{273.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500367_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500368_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{128.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600260_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{320.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600261_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{479.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400361_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400362_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{954.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{103.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400363_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{300.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400364_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400365_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{174.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400366_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{184.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400367_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{126.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400368_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{171.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000400_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000401_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000402_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000403_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000404_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000405_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000406_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200271_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{94.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200273_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{234.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200274_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{81.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200275_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{189.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200276_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800638_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800639_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800640_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{229.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{28.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800641_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3208.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2254.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800642_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800643_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1272.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1183.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800644_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1933.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900343_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900344_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{402.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900345_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{192.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000346_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000347_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1598.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000348_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{783.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400547_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400548_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889400549_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500550_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{198.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500551_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500552_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2889.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{186.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533700686_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533700687_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533700688_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{198.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533700689_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533700690_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533700691_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533800692_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{174.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533800693_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{383.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{110.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533800694_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3372.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{508.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533800695_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1374.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533800696_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{976.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133100366_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133100367_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{154.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133100368_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{461.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000273_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{186.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{41.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000274_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{319.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000275_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000276_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1766.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028900421_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000422_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000423_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000424_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000425_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000426_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000427_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{308.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000428_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1010.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000429_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000430_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000431_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000432_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000433_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000434_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{414.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000435_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{424.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100586_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{157.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100587_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100588_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100589_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100590_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100591_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100592_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100593_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100594_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100595_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100596_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100597_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898900575_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898900576_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{413.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{163.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898900577_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{480.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898900578_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899000579_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{902.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{205.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899000580_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2884.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{601.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926300502_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926300503_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926300504_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926300505_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2333.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926300506_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2557.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895900549_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895900550_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895900551_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{869.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895900552_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!CTLMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300547_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{286.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300548_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{335.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{33.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300549_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1493.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300550_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1778.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300551_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300552_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300373_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300374_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{319.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300375_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{753.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{675.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300376_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{272.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300377_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2268.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941741000378_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{849.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700503_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{264.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700504_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2904.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{75.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800406_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800407_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{280.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800408_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800409_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800410_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{272.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800411_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800412_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800413_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800414_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{274.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700373_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700374_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{245.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700375_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{267.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700376_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{242.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700377_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{252.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700378_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700497_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700498_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{251.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700499_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{530.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700500_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700501_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700502_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1964.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700503_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700504_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800413_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{585.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{41.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900414_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{748.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900497_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900498_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{483.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900499_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{313.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{70.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900500_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{241.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900501_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{197.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900502_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{160.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900503_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{126.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900504_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{324.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500638_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500639_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500640_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500641_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500642_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500643_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500644_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700373_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{254.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700374_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{38.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700375_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{117.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700376_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700377_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{160.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700378_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{262.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500876_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{286.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500877_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500878_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{230.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500879_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500880_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500881_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1271.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1185.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500882_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1938.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400547_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400548_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400549_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400550_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400551_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500552_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890100751_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200752_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200753_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{278.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200754_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{307.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200755_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{220.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200756_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{399.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536601094_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536601095_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536701096_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{296.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536701097_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536701098_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{460.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536701099_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536701100_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{174.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536701101_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{383.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{110.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536701102_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3371.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{596.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536701103_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1372.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536701104_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{977.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133900502_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{235.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133900503_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{144.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133900504_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{605.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300374_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{258.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300375_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{352.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300376_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{709.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300377_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{286.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300378_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{940.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030500676_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{288.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030500677_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{288.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030500678_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030500679_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030500680_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030500681_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030500682_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{320.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030500683_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030500684_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030500685_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600686_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600687_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600688_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600689_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{418.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1236.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600690_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2295.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500807_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{235.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500808_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500809_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{286.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500810_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{263.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500811_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{236.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500812_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500813_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{251.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500817_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500818_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{315.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500819_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{358.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900100915_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200916_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{313.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{71.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200917_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2172.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200918_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{102.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200919_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1164.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{213.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200920_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2882.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{600.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927300689_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{248.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927300690_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{245.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927300691_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{239.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927300692_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{912.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927300693_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1080.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896600753_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{279.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896600754_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896600755_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{357.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896600756_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!CTLMix}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100751_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100752_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100753_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100754_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{100.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100755_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100756_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900475_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900476_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2305.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900477_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{109.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900478_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{378.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900639_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900640_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2903.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400559_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{785.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400560_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{939.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400561_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400562_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1671.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400563_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400564_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1797.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400565_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2220.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400566_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400567_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{90.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000475_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000476_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000477_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000478_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900633_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900634_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900635_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900636_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900637_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900638_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900639_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900640_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100566_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{376.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100567_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{206.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300633_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300634_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300635_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300636_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{640.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300637_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300638_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300639_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300640_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000876_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000877_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000878_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000879_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000880_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000881_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000882_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300475_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300476_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300477_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{446.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300478_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{580.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{952.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201114_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201115_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201116_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{229.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201117_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1095.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201118_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201119_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1272.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1205.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875201120_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1933.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000751_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000752_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{245.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000753_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{253.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000754_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000755_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{409.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000756_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000955_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000956_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000957_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000958_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1914.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000959_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000960_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2890.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2069.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539501502_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539501503_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539501504_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{725.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539501505_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539501506_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{957.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539601507_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539601508_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{174.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539601509_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{383.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{109.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539601510_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{600.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539601511_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1374.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539601512_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1034.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134600638_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134600639_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{510.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134600640_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{417.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500476_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500477_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500478_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{997.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{258.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{95.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032000931_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100932_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100933_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100934_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100935_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100936_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100937_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{200.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{312.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100938_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1225.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100939_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{87.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100940_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100941_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100942_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100943_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100944_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100945_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901028_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2366.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901029_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001030_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001031_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001032_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001033_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{74.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001034_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{346.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001035_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001036_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001037_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001038_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001039_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{135.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001040_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{598.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601255_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601256_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{857.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601257_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601258_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601259_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{903.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{268.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901601260_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2886.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{597.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928300876_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928300877_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928300878_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928300879_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928300880_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{151.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897300957_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897300958_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{49.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897300959_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897300960_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!CTLMix}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800139_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800140_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{809.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800141_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800142_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800143_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848800144_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119900679_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119900680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119900681_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119900682_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119900683_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{753.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119900684_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{925.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309400911_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309400912_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2042.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800100_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{933.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800101_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800102_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800103_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800104_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{870.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800105_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800106_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800107_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{940.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800108_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1110.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600679_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{661.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600681_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600682_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{676.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600683_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600684_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1186.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300905_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300906_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300907_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300908_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{674.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300909_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{886.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300910_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2405.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1652.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300911_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300912_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1993.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151900107_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{710.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{54.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151900108_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1016.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200905_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200906_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200907_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200908_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{762.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569300909_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1827.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{68.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569300910_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569300911_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569300912_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700162_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700163_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700164_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1177.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{460.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700165_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700166_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{831.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700167_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{800.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700168_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900679_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900681_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{680.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900682_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{845.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900683_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1178.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900684_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2009.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876901590_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876901591_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876901592_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876901593_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876901594_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{78.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876901595_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876901596_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1197.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300139_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{720.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{105.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300140_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{790.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300141_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300142_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1307.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300143_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888300144_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1288.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701363_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{673.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892701364_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{868.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{48.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892801365_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892801366_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892801367_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{771.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892801368_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{814.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800278_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800279_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800280_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800281_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{797.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800282_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800283_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1060.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{70.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800284_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{79.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800285_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1185.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800286_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1213.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2163.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800287_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1290.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525800288_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135900910_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{672.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135900911_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135900912_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{772.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100681_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100682_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{724.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100683_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100684_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{709.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000166_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000167_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000168_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000169_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000170_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000171_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{675.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000172_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{714.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000173_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{674.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000174_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1173.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000175_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000176_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025000177_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025100178_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025100179_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{826.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025100180_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1175.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801470_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{672.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801471_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801472_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801473_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801474_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801475_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801476_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{820.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1164.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801477_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{989.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801478_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801479_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1177.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626901480_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{49.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626901481_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626901482_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{111.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895600235_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895600236_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895600237_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{717.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{82.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895600238_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895600239_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{146.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895600240_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930401250_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930401251_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930401252_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930401253_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1111.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930401254_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1078.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898601365_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898601366_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{714.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898601367_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{74.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898601368_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1607.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!CTLMix}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800955_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800956_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800957_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800958_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800959_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852800960_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400577_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400578_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400579_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400580_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400581_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400582_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{187.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200775_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200776_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{724.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1517.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900712_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900713_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{108.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900714_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900715_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900716_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900717_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900718_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{200.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000719_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000720_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{122.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300577_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300578_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300579_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300580_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300581_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300582_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100769_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100770_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100771_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100772_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100773_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100774_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100775_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100776_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153600719_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{871.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153600720_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{261.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1177.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800769_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800770_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800771_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800772_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800773_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800774_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800775_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800776_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501114_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501115_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600577_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600578_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600579_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600580_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600581_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600582_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001352_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{75.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001353_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001354_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{234.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{32.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001355_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{413.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{133.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001356_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876001357_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1259.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1195.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876101358_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1982.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600955_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600956_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600957_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600958_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600959_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600960_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891901159_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891901160_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891901161_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891901162_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891901163_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2867.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891901164_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{76.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501910_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501911_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501912_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501913_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501914_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501915_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501916_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{174.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501917_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{422.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{109.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501918_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{579.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{374.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501919_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1448.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542501920_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1102.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135200774_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135200775_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135200776_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2888.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800578_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800579_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800580_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800581_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800582_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033401186_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033401187_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033401188_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033401189_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033401190_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033401191_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033401192_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033401193_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033401194_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033401195_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501196_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501197_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501198_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501199_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501200_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401249_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401250_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401251_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401252_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401253_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401254_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401255_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401256_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401257_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401258_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401259_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401260_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401261_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701595_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701596_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701597_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701598_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701599_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{245.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{851.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902701600_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{425.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{209.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929501063_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929501064_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929501065_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{87.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929501066_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929501067_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898001161_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2862.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{847.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898001162_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{214.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898001163_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{97.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898001164_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{932.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_CTLPlaceComparison.tex <==

\section{Executions Reported for CTLPlaceComparison  (``Known'' models)}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400307_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400308_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{587.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{115.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400309_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{506.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{199.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400310_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1508.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400311_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1579.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1572.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854400312_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2170.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2042.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301425_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301426_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301427_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{76.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301428_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{605.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{198.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301429_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{998.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1418.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301430_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1361.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1314.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301431_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1398.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301432_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{462.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100233_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{321.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100234_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401425_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401426_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{99.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401427_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{394.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{274.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401428_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1065.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401429_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1266.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401430_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1358.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{528.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401431_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1809.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2216.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401432_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{238.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101069_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101070_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{345.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101071_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{962.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101072_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101073_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{562.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597101074_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{621.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500307_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{209.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500308_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500309_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500310_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500311_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500312_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547900614_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547900615_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547900616_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{98.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547900617_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{865.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547900618_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1105.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547900619_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1695.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{645.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547900620_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547900621_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{126.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548000622_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548000623_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{499.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968548000624_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138301430_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1075.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{167.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138301431_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2057.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1364.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138301432_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2594.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{140.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905700515_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905700516_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905800517_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1707.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{298.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905800518_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905800519_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{412.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905800520_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800103_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800104_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{176.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800105_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1267.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800106_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1391.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800107_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{375.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800108_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{685.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200151_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200152_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200153_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{874.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1722.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200154_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200155_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117200156_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{258.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200207_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200208_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2870.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{107.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700073_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700074_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{70.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700075_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{224.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700076_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{61.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700077_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700078_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700079_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700080_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2839.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700081_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000151_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000152_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000153_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1973.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000154_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000155_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1384.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000156_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1878.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200201_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200202_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200203_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{92.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200204_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{422.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200205_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200206_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{848.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200207_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1049.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200208_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{82.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300080_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300081_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{484.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900201_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900202_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900203_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{347.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900204_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{239.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900205_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{329.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900206_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900207_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{409.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566900208_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{209.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400121_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400122_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400123_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400124_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400125_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400126_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600151_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{386.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600152_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700153_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{171.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700154_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{99.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700155_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593700156_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{121.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000358_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000359_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{173.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{66.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000360_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000361_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2867.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1585.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000362_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1623.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000363_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873000364_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{152.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300103_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300104_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300105_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1140.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300106_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{302.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300107_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889300108_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{781.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600307_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600308_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{738.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600309_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{694.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600310_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{229.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600311_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{631.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600312_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{230.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600206_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600207_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600208_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{180.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600209_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{150.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600210_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{191.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600211_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{424.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600212_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{79.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600213_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2868.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{281.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600214_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2879.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{145.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600215_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2903.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{216.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530600216_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2964.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2057.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132200206_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132200207_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{206.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132200208_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{455.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700152_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700153_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{225.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{62.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700154_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{373.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700155_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1915.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700156_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1687.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500121_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600122_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600123_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600124_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600125_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600126_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{792.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{187.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600127_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600128_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{362.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600129_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{115.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600130_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600131_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600132_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600133_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600134_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027600135_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{94.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700326_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{434.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700327_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700328_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700329_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700330_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700331_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700332_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700333_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{79.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700337_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700338_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897600175_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897600176_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{413.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{40.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897600177_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{801.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897600178_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1925.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897600179_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2568.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897600180_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{602.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000282_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000283_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000284_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000285_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2049.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925000286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400307_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400308_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{176.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{40.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400309_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1287.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400310_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1329.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400311_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{379.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400312_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{693.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600253_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600254_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600255_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{874.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1668.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700256_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700257_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117700258_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{259.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400343_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2868.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{115.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200226_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200227_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{68.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200228_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{210.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200229_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{60.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200230_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200231_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200232_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200233_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200234_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300253_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300254_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300255_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1994.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300256_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300257_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1375.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300258_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1739.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400337_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400338_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400339_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{92.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400340_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{415.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400341_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400342_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{803.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400343_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{955.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{88.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600233_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600234_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{477.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300337_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300338_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400339_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{317.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400340_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{223.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400341_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{308.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400342_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400343_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{376.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{225.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900358_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900359_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900360_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900361_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900362_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900363_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390900364_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100253_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{386.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{28.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100254_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100255_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{169.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100256_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{104.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100257_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200258_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{123.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600596_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600597_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{173.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{75.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2867.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1600.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1624.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600601_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{125.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600602_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{149.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800307_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800308_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800309_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1132.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800310_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{337.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800311_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889900312_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{721.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300511_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300512_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{738.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300513_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{679.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300514_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{204.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300515_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{655.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300516_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{220.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200614_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200615_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200616_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{182.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200617_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{171.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200618_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{191.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200619_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{406.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200620_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{83.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200621_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2868.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{209.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200622_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2877.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{223.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200623_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2899.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{172.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533200624_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2965.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133000342_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133000343_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{193.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133000344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{455.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000254_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000255_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{225.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000256_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{385.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000257_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1932.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000258_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1743.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700376_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700377_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700378_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700379_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800380_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800381_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{792.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{222.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800382_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800383_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{367.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800384_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{113.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800385_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800386_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800387_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800388_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800389_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028800390_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{103.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000547_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{437.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000548_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000549_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000550_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000551_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100552_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100553_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100554_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100555_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100556_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100557_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100558_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700515_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700516_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{413.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{38.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700517_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{747.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700518_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1848.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700519_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2648.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898700520_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{607.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926000469_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926000470_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926000471_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926000472_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2066.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926100473_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100511_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100512_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{330.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100513_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2042.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100514_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100515_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{428.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851100516_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{332.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200355_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200356_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{305.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200357_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{660.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200358_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{221.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200359_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{258.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2868.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{104.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700379_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{268.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700380_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700381_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700382_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700383_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700384_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700385_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700386_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700387_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{285.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600355_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600356_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{249.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600357_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600358_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{230.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700359_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700360_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600473_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600474_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600475_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{307.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600476_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{186.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600477_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600478_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1334.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1276.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1424.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1353.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800386_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800387_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{751.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800473_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800474_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{260.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800475_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{353.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{796.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800476_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{128.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800477_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{786.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1607.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800478_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{251.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1402.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{109.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400596_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400597_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400598_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400599_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400600_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400601_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391400602_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600355_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{465.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600356_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600357_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{107.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600358_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2844.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{47.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600359_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600360_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2844.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{54.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300834_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300835_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{69.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300836_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400837_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{339.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400838_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{346.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400839_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{390.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874400840_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{417.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400511_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400512_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{271.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400513_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400514_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400515_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890400516_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000715_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000716_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000717_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000718_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000719_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{321.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000720_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{334.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536201022_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536201023_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536201024_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{241.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536201025_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{180.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536201026_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536201027_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{424.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536201028_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2559.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536201029_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2870.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{400.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536201030_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2880.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{263.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536201031_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{810.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536301032_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{781.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133800478_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{239.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133800479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{196.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133800480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{546.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200356_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{272.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200357_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{369.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200358_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{701.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200359_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2291.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200360_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{987.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200631_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200632_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200633_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{275.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030200634_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300635_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300636_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{321.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{56.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300637_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300638_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300639_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300640_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300641_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300642_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300643_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300644_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030300645_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400768_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{505.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400769_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{246.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500770_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{242.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500771_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500772_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{245.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500773_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500774_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{280.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500775_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500776_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{252.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500777_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500778_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500779_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{315.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500780_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900855_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900856_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{313.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900857_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900858_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1814.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900859_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1163.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899900860_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{612.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200657_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200658_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1979.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200659_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1088.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927200660_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900715_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900716_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900717_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900718_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{95.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900719_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900720_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800457_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800458_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1207.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800459_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{116.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800460_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800461_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118800462_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{379.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2870.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{114.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300532_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300533_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{955.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300534_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1483.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300535_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1690.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300536_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300537_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{911.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300538_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2191.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300539_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856300540_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{244.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900457_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900458_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900459_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900460_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000461_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000462_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800609_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800610_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800611_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800613_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800614_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100539_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{115.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100540_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{477.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{107.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300609_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300610_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300611_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300613_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300614_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568300616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900834_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900835_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900836_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900837_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900838_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900839_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391900840_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200457_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200458_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200459_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{455.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200460_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{580.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200461_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595200462_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{923.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101072_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101073_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{84.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{149.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101074_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101075_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{835.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101076_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{629.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101077_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{126.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875101078_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{177.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900715_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900716_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900717_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{245.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900718_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{333.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900719_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890900720_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{676.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800919_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800920_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800921_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1328.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800922_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2386.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800923_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890800924_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101430_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101431_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101432_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101433_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{849.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101434_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{955.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101435_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{274.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101436_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101437_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{79.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101438_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{116.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101439_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{227.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539101440_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{315.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134500614_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134500615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1283.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134500616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{408.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500458_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500459_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500460_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1030.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500461_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{260.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500462_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{95.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800886_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800887_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800888_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800889_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800890_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800891_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800892_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800893_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1238.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800894_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1739.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800895_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031800896_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900897_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900898_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900899_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031900900_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1223.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900989_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2367.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900990_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900991_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900992_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900993_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900994_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900995_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{108.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{506.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900996_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900997_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900998_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625900999_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901000_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{139.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625901001_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{401.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901401195_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901401196_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{890.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901401197_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901401198_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{105.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901401199_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{931.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901401200_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{599.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928100843_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928100844_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928100845_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{210.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928100846_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928100847_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700103_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700104_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700105_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700106_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700107_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848700108_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1141.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800661_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800662_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800663_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800664_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800665_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{751.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800666_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{926.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309400887_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309400888_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1331.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700073_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{933.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700074_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1099.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700075_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700076_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700077_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{870.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700078_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1105.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800079_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800080_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853800081_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600661_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{661.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600662_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{661.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600663_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600664_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600665_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891600666_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300881_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300882_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300883_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300884_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{673.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300885_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{861.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300886_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2405.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1548.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300887_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300888_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1993.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151900080_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{53.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151900081_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1016.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200881_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200882_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200883_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200884_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{751.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200885_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200886_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200887_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569200888_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700120_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700121_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700122_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{727.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700123_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{853.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700124_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{831.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700125_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389700126_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{862.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800661_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800662_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800663_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{680.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800664_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{845.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900665_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1180.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595900666_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2009.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701548_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701549_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{800.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701550_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801551_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{953.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801552_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1151.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801553_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876801554_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{144.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200103_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200104_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{805.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200105_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{804.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200106_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200107_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1283.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200108_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1294.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2409.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601327_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601328_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601329_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601330_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601331_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{771.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892601332_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525400206_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525400207_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525400208_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525400209_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525400210_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{681.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525400211_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{735.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525400212_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{81.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525400213_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1185.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{944.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525400214_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1214.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525400215_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1290.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525500216_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135800886_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135800887_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135800888_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{157.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000662_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000663_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{716.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100664_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{724.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100665_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219100666_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800121_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800122_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800123_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800124_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800125_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800126_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800127_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800128_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800129_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800130_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800131_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024800132_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900133_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900134_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024900135_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701431_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701432_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801433_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801434_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801435_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801436_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801437_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{787.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{611.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801438_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{989.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801439_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2379.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801440_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1177.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801441_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{28.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801442_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626801443_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{97.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895400175_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895400176_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895400177_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895400178_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895400179_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1199.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895400180_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930201217_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930201218_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930201219_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1123.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1360.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930201220_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1110.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930201221_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1077.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700919_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700920_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700921_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700922_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700923_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852700924_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300561_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300562_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300563_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300564_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100751_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100752_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800685_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800686_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800687_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800688_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800689_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800690_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800691_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900692_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856900693_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200561_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300562_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300563_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300564_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100745_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100746_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100747_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100748_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100749_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100750_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100751_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100752_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153500692_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153500693_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700745_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700746_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700747_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700748_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700749_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700750_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700751_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700752_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401072_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401073_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401074_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401075_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401076_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401077_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401078_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500561_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500562_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500563_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500564_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901310_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901311_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901312_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901313_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901314_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901315_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875901316_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500919_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500920_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500921_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500922_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500923_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891500924_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701123_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701124_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701125_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701126_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701127_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891801128_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541901838_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542001839_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542001840_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542001841_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542001842_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542001843_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{832.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542001844_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542001845_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{217.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542001846_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542001847_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{91.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542001848_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{168.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135100750_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135100751_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135100752_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800561_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800562_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800563_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800564_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201141_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201142_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201143_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201144_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201145_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201146_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201147_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201148_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201149_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201150_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201151_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201152_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033201153_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301154_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033301155_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301210_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301211_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301212_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301213_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301214_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301215_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301216_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301217_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301218_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301219_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301220_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301221_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301222_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501535_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501536_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501537_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501538_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501539_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902501540_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{392.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2071.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929301030_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929301031_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929301032_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929301033_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929301034_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_LTLCardinalityComparison.tex <==

\section{Executions Reported for LTLCardinalityComparison  (``Known'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000175_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000176_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000177_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000178_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000179_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000180_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300187_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300188_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300189_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300190_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300191_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300192_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300255_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300256_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900127_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900128_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900129_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900130_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900131_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900132_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900133_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900134_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900135_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100187_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200188_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200189_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200190_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200191_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200192_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300249_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300250_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300251_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300252_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300253_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300254_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300255_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300256_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400134_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400135_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000249_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000250_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000251_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000252_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000253_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000254_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000255_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000256_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600204_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600205_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600206_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600207_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600208_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600209_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600210_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800187_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800188_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800189_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800190_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800191_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800192_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200442_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200443_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200444_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200445_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{816.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{300.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200446_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1826.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1194.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200447_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1231.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1225.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200448_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1933.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500175_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500176_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500177_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500178_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500179_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500180_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900379_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900380_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900381_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900382_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900383_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900384_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400350_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400351_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400352_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400353_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400354_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400355_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400356_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{225.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400357_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{795.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{281.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400358_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2738.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2239.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400359_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1430.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531400360_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{912.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132500254_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132500255_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132500256_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800188_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800189_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800190_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800191_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800192_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000211_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000212_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000213_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000214_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000215_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000216_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000217_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000218_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000219_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000220_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000221_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000222_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000223_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000224_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000225_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800404_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800409_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800410_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800411_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800412_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800413_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800414_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800415_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800416_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898000295_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898000296_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898000297_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898000298_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898000299_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898000300_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925300348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925300349_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925300350_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925300351_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925300352_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700379_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700380_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700381_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700382_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700383_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700384_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900289_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900290_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900291_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900292_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900293_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900294_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500391_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400280_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400281_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400282_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400283_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400284_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400285_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400286_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400287_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400288_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400289_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400290_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400291_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400292_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400293_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400294_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500385_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500386_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500387_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500388_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500389_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500390_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500391_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600287_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700288_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500385_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500386_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500387_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500388_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500389_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500390_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500391_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000442_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000443_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000444_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000445_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000446_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000447_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000448_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300289_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300290_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300291_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300292_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300293_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300294_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900681_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900682_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900683_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{816.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{297.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900684_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1826.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1187.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900685_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1231.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1177.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900686_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1933.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000379_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000380_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000381_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000382_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000383_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000384_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600583_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600584_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600585_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600586_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600587_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600588_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534200758_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534200759_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534200760_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534200761_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534200762_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534200763_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534200764_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{225.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534200765_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{796.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{293.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534200766_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2738.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2200.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534300767_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1362.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534300768_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1003.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133300390_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133300391_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133300392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100290_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100291_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100292_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100293_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100294_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200466_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200467_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200468_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200469_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200470_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200471_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200472_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200473_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200474_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200475_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200476_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200477_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029300478_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029300479_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029300480_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200625_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200626_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200627_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200628_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200629_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200630_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200631_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200632_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200633_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200634_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200635_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200636_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200637_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899100635_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899100636_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899200637_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899200638_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899200639_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899200640_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926500535_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926500536_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926500537_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926500538_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926500539_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400583_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400584_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400585_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400586_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400587_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400588_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400391_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400393_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400394_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400395_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400396_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900433_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900434_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900435_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900436_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900437_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900438_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900439_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900440_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900441_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700391_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700393_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800394_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800395_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800396_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700521_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700522_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700523_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700524_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700525_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900440_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900441_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900521_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900522_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900523_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000524_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000525_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600680_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600681_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600682_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600683_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600684_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600685_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600686_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594800391_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594800392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594800393_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594800394_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594800395_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594800396_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600918_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600919_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{82.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600920_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600921_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{816.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{331.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600922_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1826.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1222.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600923_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1231.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1194.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600924_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1932.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500583_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500584_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500585_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500586_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500587_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500588_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300787_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300788_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300789_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300790_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201166_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201167_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201168_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201169_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201170_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201171_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201172_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{225.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201173_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{796.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{288.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201174_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2738.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2243.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201175_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1415.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537201176_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1009.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134100526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134100527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134100528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300393_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300394_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300395_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300396_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700721_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700722_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700723_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700724_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800725_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800726_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800727_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800728_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800729_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800730_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800731_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800732_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800733_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800734_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030800735_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600846_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600847_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600848_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600849_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600850_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600851_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600852_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600853_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600854_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600855_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600856_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600857_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600858_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900400975_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900400976_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900400977_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900400978_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900400979_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900400980_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400722_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400723_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400724_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500725_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500726_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200787_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200788_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200789_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200790_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200791_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300792_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900493_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900494_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119000495_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119000496_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119000497_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119000498_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000663_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000664_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500586_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500587_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500588_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500589_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500590_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500591_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500592_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500593_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500594_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000493_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000494_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100495_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100496_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100497_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100498_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900657_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900658_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900659_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900660_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900661_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900662_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900663_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900664_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153200593_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153200594_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400657_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400658_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400659_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400660_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400661_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400662_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400663_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400664_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100918_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100919_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100920_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100921_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100922_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100923_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100924_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300493_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300494_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300495_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300496_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300497_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400498_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401156_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401157_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401158_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401159_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{321.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401160_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1826.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1217.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401161_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1231.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1210.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401162_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1928.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100787_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100788_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100789_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100790_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100791_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100792_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100991_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100992_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100993_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100994_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100995_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891200996_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101574_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101575_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101576_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101577_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101578_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101579_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101580_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{225.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101581_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{795.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{274.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101582_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2738.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2127.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101583_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1451.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540101584_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1039.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134700662_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134700663_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134700664_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600494_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600495_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600496_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600497_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600498_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300976_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300977_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300978_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300979_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300980_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300981_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032400982_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032400983_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032400984_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032400985_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032400986_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032400987_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032400988_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032400989_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032400990_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001067_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001068_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001069_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001070_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001071_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001072_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101073_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101074_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101075_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101076_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101077_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101078_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101079_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801315_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801316_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801317_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801318_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801319_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801320_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928500909_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928500910_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928500911_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928500912_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928500913_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900175_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900176_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2562.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{201.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900177_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{368.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{57.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900178_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900179_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900180_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500799_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600800_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{374.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{32.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600801_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{643.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{60.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600802_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2911.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{277.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600803_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600804_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000799_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000800_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000801_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{203.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000802_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000803_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000804_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601065_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601066_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601067_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601068_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{134.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601069_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601070_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601071_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601072_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901065_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901066_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901067_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901068_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901069_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901070_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901071_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901072_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100204_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100205_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{313.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{42.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100206_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{464.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{75.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100207_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{119.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100208_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1003.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{145.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100209_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1448.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{266.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100210_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1983.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{433.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200799_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200800_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200801_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300802_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300803_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300804_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801870_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1626.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{206.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801871_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801872_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801873_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801874_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801875_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801876_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893801603_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893801604_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{910.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{96.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893801605_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2246.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{229.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893801606_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893801607_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893801608_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546000350_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546000351_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{166.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546000352_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{255.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{33.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546000353_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546000354_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546000355_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546000356_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546000357_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546000358_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546000359_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546100360_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136701070_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{402.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136701071_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2989.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{321.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136701072_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500800_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500801_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{351.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500802_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{123.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500803_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500804_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900211_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900212_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{125.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900213_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900214_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900215_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{167.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900216_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{209.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900217_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900218_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{740.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{152.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900219_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3025.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{653.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900220_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{131.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900221_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{144.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900222_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{162.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900223_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{186.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900224_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{379.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{64.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900225_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{941.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{225.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401731_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{163.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401732_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{198.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401733_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{337.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401734_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{678.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401735_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2938.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{379.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401736_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{311.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401737_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{327.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401738_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{207.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401739_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{889.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{94.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401740_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401741_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{305.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401742_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2812.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{300.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904500295_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{162.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904500296_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{431.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904500297_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2570.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{426.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904500298_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904500299_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904500300_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931801470_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{151.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931801471_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{274.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931801472_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2914.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{283.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931801473_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2030.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{210.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931801474_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{278.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853000991_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853000992_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853000993_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853000994_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853000995_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853000996_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500595_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500596_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500597_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200799_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200800_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000739_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000740_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000741_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000742_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000743_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000744_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000745_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000746_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000747_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400595_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400596_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400597_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100793_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100794_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100795_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100796_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100797_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100798_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100799_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100800_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153600746_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153600747_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900793_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900794_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900795_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900796_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900797_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900798_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900799_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900800_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601156_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601157_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601158_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601159_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601160_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601161_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601162_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600595_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600596_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600597_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201394_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201395_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{82.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201396_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201397_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{816.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{300.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201398_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1826.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1193.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201399_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1231.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1182.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201400_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1935.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700991_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700992_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700993_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700994_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700995_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700996_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001195_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001196_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101197_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101198_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101199_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101200_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542901982_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542901983_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543001984_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543001985_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543001986_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543001987_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543001988_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{225.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543001989_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{796.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{292.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543001990_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2738.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2616.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543001991_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1466.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543001992_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1042.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135300798_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135300799_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135300800_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900596_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900597_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601231_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601232_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601233_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601234_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701235_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701236_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701237_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701238_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701239_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701240_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701241_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701242_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701243_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701244_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033701245_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501288_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501289_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501290_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501291_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501292_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501293_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501294_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501295_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501296_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501297_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501298_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501299_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501300_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901655_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901656_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901657_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901658_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901659_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901660_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701096_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701097_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701098_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701099_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701100_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_LTLFireability.tex <==

\section{Executions Reported for LTLFireability  (``Known'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!LTLFireability}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000151_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000152_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000153_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000154_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000155_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000156_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300175_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300176_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300177_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300178_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300179_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300239_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300240_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800109_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800110_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800111_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800112_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800113_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854800114_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900115_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100175_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100176_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100177_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100178_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100179_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100180_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200233_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300234_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300235_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300236_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300237_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300238_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300239_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300240_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000233_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000234_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000235_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000236_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000237_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000238_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000239_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000240_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500176_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500177_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500178_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500179_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500180_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500181_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390500182_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800175_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800176_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800177_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800178_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800179_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800180_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100414_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100415_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100416_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100417_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100418_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100419_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873100420_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400151_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400152_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400153_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400154_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400155_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400156_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800355_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800356_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800357_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800358_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800359_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800360_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531100302_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531100303_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531100304_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531200305_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531200306_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531200307_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531200308_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531200309_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531200310_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531200311_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531200312_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132400238_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132400239_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132400240_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800176_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800177_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800178_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800179_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800180_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800181_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800182_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800183_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800184_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800185_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800186_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027800187_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900188_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900189_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900190_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900191_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900192_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900193_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900194_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900195_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700378_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700379_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700380_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700381_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700382_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700383_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700384_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700385_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700386_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700387_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700388_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700389_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700390_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897800255_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897800256_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897900257_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897900258_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897900259_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897900260_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925200326_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925200327_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925200328_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925200329_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925200330_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895300357_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895300358_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895300359_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895300360_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{98.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!LTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600355_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600356_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600357_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600358_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600359_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600360_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800277_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800278_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800279_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800280_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800281_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800282_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500375_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500376_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300262_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300263_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300264_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300265_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300266_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300267_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855300268_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400269_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400270_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400277_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400278_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400279_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400280_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400281_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400282_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500369_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500370_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500371_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500372_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500373_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500374_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500375_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500376_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600269_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600270_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567400369_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500370_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500371_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500372_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500373_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500374_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500375_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500376_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000414_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000415_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000416_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000417_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000418_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000419_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000420_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200277_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200278_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200279_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594200280_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300281_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300282_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800652_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800653_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800654_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800655_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800657_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873800658_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000355_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000356_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000357_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000358_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000359_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000360_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500561_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500562_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500563_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500564_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533900710_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533900711_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533900712_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533900713_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533900714_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533900715_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533900716_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533900717_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968533900718_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534000719_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534000720_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133200374_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133200375_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133200376_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000278_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000279_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000280_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000281_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000282_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000436_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000437_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000438_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000439_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029000440_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100441_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100442_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100443_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100444_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100445_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100446_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100447_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100448_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100449_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100450_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100601_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100602_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100603_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100604_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100605_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100606_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100607_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100608_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100609_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625100610_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200611_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899000595_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899000596_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899000597_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899000598_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899000599_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899000600_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926300513_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926300514_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926400515_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926400516_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926400517_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896000561_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896000562_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896000563_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896000564_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{98.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!LTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300559_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300560_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300561_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300562_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300563_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851300564_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300379_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300380_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300381_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118300382_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400383_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400384_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700511_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700512_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800415_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800416_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800417_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855800418_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900419_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900420_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900421_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900422_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900423_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700379_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700380_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700381_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700382_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700383_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700384_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700505_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700506_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700507_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700508_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700509_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700510_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700511_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700512_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900422_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900423_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900505_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900506_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900507_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900508_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900509_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900510_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900511_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900512_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500652_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500653_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500654_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500655_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500656_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500657_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500658_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700379_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700380_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700381_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700382_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700383_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700384_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500890_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500891_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500892_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500893_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500894_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500895_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500896_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500559_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500560_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500561_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500562_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500563_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500564_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200763_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200764_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200765_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200766_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200767_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200768_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536801118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536801119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536801120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536801121_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536801122_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536901123_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536901124_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536901125_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536901126_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536901127_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968536901128_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134000510_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134000511_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134000512_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300380_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300381_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300382_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300383_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300384_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600691_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600692_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600693_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600694_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600695_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600696_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600697_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600698_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600699_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600700_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600701_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600702_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600703_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600704_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600705_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625500820_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600821_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600822_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600823_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600824_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600825_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600826_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600827_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600828_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600829_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600830_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600831_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600832_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200935_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200936_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200937_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200938_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200939_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900200940_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400700_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400701_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400702_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400703_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400704_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896600765_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896600766_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896600767_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896600768_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{98.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!LTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100763_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100764_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100765_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100766_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100767_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852100768_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900481_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900482_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900483_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900484_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900485_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900486_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900647_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900648_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400568_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400569_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400570_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400571_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400572_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400573_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400574_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400575_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400576_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000481_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000482_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000483_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000484_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000485_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000486_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900641_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900642_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900643_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900644_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900645_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900646_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900647_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900648_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100575_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100576_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400641_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400642_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400643_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400644_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400645_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400646_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400647_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400648_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000890_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000891_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000892_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000893_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000894_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000895_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392000896_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300481_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300482_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300483_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300484_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300485_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300486_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301128_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301129_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301130_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301131_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301132_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301133_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301134_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000763_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000764_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000765_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000766_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000767_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891000768_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000967_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000968_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000969_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000970_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000971_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891000972_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539701526_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539701527_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539701528_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539701529_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539701530_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539701531_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539701532_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539701533_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539701534_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539801535_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539801536_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134700646_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134700647_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134700648_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500482_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500483_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500484_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600485_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600486_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032100946_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200947_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200948_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200949_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200950_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200951_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200952_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200953_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200954_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200955_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200956_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200957_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200958_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200959_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200960_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001041_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001042_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001043_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001044_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001045_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001046_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001047_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001048_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001049_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001050_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001051_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001052_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001053_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901701275_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901701276_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901701277_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901701278_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901701279_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901701280_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928400887_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928400888_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928400889_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928400890_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928400891_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897300969_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897300970_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897400971_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897400972_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{98.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!LTLFireability}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853800151_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853800152_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{197.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853800153_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{368.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900154_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900155_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900156_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500787_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500788_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{374.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{27.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500789_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{641.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{52.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500790_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2911.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{279.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891900787_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891900788_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891900789_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{203.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891900790_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891900791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891900792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601049_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{134.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601050_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601051_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601052_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601053_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601054_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601055_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601056_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801049_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{128.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801050_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801051_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801052_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801053_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801054_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801055_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801056_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000176_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{140.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000177_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{311.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{693.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000178_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{465.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000179_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000180_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1002.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000181_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1447.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000182_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1982.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200787_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200788_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200789_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200790_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877701842_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1624.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877701843_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877701844_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877701845_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877701846_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877701847_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877701848_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701579_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{304.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701580_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{910.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701581_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2245.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{215.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701582_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701583_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701584_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545600302_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545700303_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{191.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{587.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545700304_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{254.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545700305_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545700306_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545700307_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545700308_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545700309_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545700310_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545700311_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545700312_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136601054_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{403.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136601055_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2989.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{310.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136601056_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219400788_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219400789_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{351.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219400790_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{114.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219400791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219400792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034700181_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{122.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034700182_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034700183_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034700184_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034700185_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{167.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034700186_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{210.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800187_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800188_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{740.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{153.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800189_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2226.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{621.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800190_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800191_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{144.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800192_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{162.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800193_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{186.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800194_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{379.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800195_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{940.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{179.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301705_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{163.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301706_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{198.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301707_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{336.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301708_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{679.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{63.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301709_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2941.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{387.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301710_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{302.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301711_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2866.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{312.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301712_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{207.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301713_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{889.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{119.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301714_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301715_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{319.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301716_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2813.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{324.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904200255_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1982.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904200256_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{432.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904200257_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2570.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{414.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904200258_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904300259_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904300260_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931701448_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{151.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931701449_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{28.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931701450_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{833.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931701451_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2031.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931701452_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{275.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899301581_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{214.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899301582_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1493.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{130.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899401583_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899401584_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!LTLFireability}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900967_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900968_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900969_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900970_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900971_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900972_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400583_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119400584_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500585_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500586_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500587_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500588_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{188.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200783_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200784_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1471.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000721_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000722_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000723_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000724_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000725_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000726_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000727_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000728_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000729_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300583_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300584_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300585_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300586_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891300587_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400588_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100777_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100778_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100779_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100780_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100781_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100782_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100783_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100784_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153600728_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153600729_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{365.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1635.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800777_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800778_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800779_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800780_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800781_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800782_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800783_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800784_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501128_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501129_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501130_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501131_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501132_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501133_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501134_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600583_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600584_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600585_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600586_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600587_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600588_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876101366_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876101367_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876101368_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876101369_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876101370_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876101371_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{91.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876101372_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{122.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600967_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600968_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600969_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600970_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600971_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891600972_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891901171_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001172_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001173_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001174_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001175_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001176_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542601934_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542601935_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542601936_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542601937_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542601938_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542601939_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542701940_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542701941_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542701942_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{75.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542701943_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542701944_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{245.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135300782_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135300783_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135300784_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800584_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800585_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800586_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800587_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800588_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501201_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501202_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501203_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501204_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501205_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501206_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501207_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501208_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501209_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501210_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501211_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501212_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501213_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501214_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033501215_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401262_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401263_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401264_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401265_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401266_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401267_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401268_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401269_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401270_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626401271_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501272_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501273_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501274_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902801615_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902801616_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902801617_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902801618_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902801619_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{109.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902801620_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{316.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{197.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929601074_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929601075_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929601076_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929601077_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929601078_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898001173_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898001174_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898001175_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{89.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898001176_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{892.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_LTLMarkingComparison.tex <==

\section{Executions Reported for LTLMarkingComparison  (``Known'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100187_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100188_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100189_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100190_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100191_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100192_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300263_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300264_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400143_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400144_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600218_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600219_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600220_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600221_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600222_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600223_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600224_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200456_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200457_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200458_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200459_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200460_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200461_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200462_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500187_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500188_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500189_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500190_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500191_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500192_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900391_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900393_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900394_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900395_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900396_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531500374_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531500375_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531500376_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531600377_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531600378_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531600379_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531600380_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531600381_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531600382_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531600383_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{86.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531600384_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{128.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132500262_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132500263_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132600264_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898000315_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898000316_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898100317_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898100318_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898100319_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{105.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898100320_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925300359_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925300360_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925300361_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925300362_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925400363_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895400393_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895400394_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895400395_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895400396_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700391_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700392_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700393_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700394_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700395_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700396_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500399_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500400_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700296_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700297_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100456_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100457_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100458_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100459_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100460_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100461_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100462_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000694_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000695_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000696_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000697_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000698_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000699_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000700_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100391_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100392_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100393_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100394_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100395_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100396_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600595_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600596_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600597_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889600600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400782_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400783_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400784_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400785_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400786_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400787_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400788_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400789_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400790_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400791_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{84.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534400792_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{128.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133300398_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133300399_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133300400_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899200655_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899200656_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899200657_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899200658_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899200659_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{111.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899200660_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926600546_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926600547_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926600548_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926600549_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926600550_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896100597_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896100598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896100599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896100600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500595_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500596_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500597_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500598_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500599_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500600_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700535_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700536_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900449_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900450_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600694_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600695_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600696_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600697_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600698_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600699_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600700_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600932_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600933_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600934_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600935_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600936_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600937_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600938_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600595_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600596_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600597_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600598_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600599_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600600_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300799_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300800_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300801_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300802_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300803_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300804_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401190_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401191_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401192_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401193_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401194_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401195_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401196_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401197_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401198_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401199_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{86.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537401200_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134100534_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134100535_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134100536_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900500995_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900500996_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900500997_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900500998_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900500999_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{111.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900501000_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500733_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500734_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500735_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500736_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500737_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896700801_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896700802_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896700803_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896700804_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300799_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300800_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300801_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300802_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300803_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300804_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000671_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000672_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153200602_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153200603_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100932_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100933_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100934_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100935_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100936_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100937_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100938_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401170_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401171_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401172_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401173_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401174_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401175_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875401176_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100799_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100800_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100801_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100802_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100803_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100804_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201003_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201004_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201005_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201006_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201007_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201008_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301598_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301599_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301600_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301601_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301602_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301603_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301604_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301605_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301606_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301607_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{86.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540301608_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134800670_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134800671_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134800672_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901901335_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901901336_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901901337_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901901338_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901901339_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{106.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901901340_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928600920_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928600921_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928600922_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928600923_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928600924_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897501005_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897501006_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897501007_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897501008_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000187_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000188_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{197.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000189_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{368.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000190_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000191_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000192_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100218_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100219_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{311.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100220_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{464.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{62.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100221_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{111.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100222_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1002.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{188.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100223_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1445.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{286.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100224_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1982.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{322.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901884_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1626.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{208.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901885_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901886_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901887_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901888_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901889_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901890_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893801615_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893801616_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{910.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{86.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893801617_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2245.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{215.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893801618_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901619_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901620_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546200374_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546200375_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{166.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546200376_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{254.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546200377_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546200378_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546200379_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546200380_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546200381_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546200382_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546200383_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546300384_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136701078_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{403.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136701079_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2990.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{309.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136701080_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904600315_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{162.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904600316_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{432.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{62.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904600317_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2570.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{405.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904700318_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904700319_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904700320_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901481_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{152.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901482_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901483_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{833.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{87.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901484_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2030.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{237.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901485_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{286.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501617_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{214.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501618_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1488.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{154.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501619_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501620_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853001003_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853001004_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853101005_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853101006_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853101007_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853101008_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200807_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200808_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153700755_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153700756_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601170_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601171_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601172_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601173_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601174_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601175_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601176_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201408_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201409_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301410_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301411_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301412_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301413_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301414_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891701003_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891701004_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891701005_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891701006_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891701007_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891701008_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101207_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101208_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101209_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101210_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101211_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101212_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543102006_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543102007_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543102008_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543102009_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543202010_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543202011_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543202012_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543202013_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543202014_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543202015_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{75.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543202016_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{128.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135400806_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135400807_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135400808_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903001675_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903001676_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903001677_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903001678_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903001679_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{106.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903001680_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701107_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701108_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701109_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701110_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701111_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898101209_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898101210_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898101211_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898101212_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_LTLMix.tex <==

\section{Executions Reported for LTLMix  (``Known'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!LTLMix}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100199_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100200_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100201_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100202_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100203_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850100204_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400199_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400200_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400201_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400202_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400203_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400204_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300271_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000145_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000146_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000147_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000148_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000149_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000150_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000151_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000152_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000153_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200199_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200200_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200201_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200202_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200203_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200204_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300265_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300266_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300267_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300268_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300269_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300270_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300271_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400152_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400153_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567100265_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567100266_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567100267_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567100268_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567100269_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567100270_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567100271_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567100272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600232_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600233_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600234_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600235_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600236_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600237_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600238_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900199_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900200_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900201_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900202_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900203_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900204_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873300470_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873300471_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873300472_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873300473_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{388.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{130.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873300474_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1107.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{707.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873300475_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873300476_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1931.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500199_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500200_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500201_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500202_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500203_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600204_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900403_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888900404_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889000405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889000406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889000407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889000408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{76.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531700398_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531700399_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531700400_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531700401_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531700402_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531700403_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531700404_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{87.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531700405_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{74.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531700406_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1893.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1521.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531800407_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1378.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531800408_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{115.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132600270_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132600271_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132600272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800200_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800201_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800202_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800203_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800204_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100241_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100242_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100243_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100244_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100245_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100246_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100247_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100248_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100249_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100250_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100251_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100252_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100253_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028100254_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028200255_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800433_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800434_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800435_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800436_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800437_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800438_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800439_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800440_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900441_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900442_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898100335_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898100336_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898100337_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898100338_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898100339_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898100340_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925400370_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925400371_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925400372_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925400373_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925400374_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895500405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895500406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895500407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895500408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{102.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!LTLMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700403_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700404_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700405_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700406_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850700407_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850800408_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900301_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900302_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900303_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117900305_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400298_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400299_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500300_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500301_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500302_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500303_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500304_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500305_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500306_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500301_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500302_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500303_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500305_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500306_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500401_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500402_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500403_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500404_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700305_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700306_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500401_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500402_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600403_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600404_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100470_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100471_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100472_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100473_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100474_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100475_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391100476_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400301_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400302_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400303_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400305_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400306_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000708_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000709_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000710_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000711_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{389.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{130.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000712_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1107.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{696.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000713_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874000714_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1934.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100403_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100404_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100405_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100406_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100407_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890100408_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889700607_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889700608_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889700609_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889700610_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889700611_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889700612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{75.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534500806_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534500807_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534500808_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534500809_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534500810_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534500811_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534500812_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{87.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534600813_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{77.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534600814_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1893.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1566.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534600815_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1383.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534600816_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{112.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133400406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133400407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133400408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100302_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100303_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100305_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100306_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400496_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400497_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400498_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400499_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400500_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400501_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400502_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400503_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400504_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400505_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400506_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400507_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400508_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029400509_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029500510_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200651_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200652_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200653_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200654_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200655_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200657_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200658_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200659_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200660_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200661_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200662_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200663_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899300675_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899300676_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899300677_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899300678_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899300679_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899300680_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926600557_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926600558_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926600559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926700560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926700561_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896100609_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896100610_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896100611_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896100612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{105.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!LTLMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500607_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500608_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500609_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500610_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500611_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851500612_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500403_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500404_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700543_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700544_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000451_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000452_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000453_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000454_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000455_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000456_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000457_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000458_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000459_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800403_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800404_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700537_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700538_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700539_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700540_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700541_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700542_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700543_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700544_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900458_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900459_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000537_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000538_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000539_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000540_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000541_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000542_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000543_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568000544_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600708_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600709_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600710_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600711_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600712_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600713_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600714_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594900403_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594900404_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594900405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594900406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594900407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594900408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874700946_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874700947_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874700948_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874700949_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{388.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{123.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874700950_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1107.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{695.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874700951_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874700952_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1928.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600607_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600608_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600609_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600610_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600611_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600612_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890400811_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890400812_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890400813_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890400814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890400815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890400816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{76.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537601214_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537601215_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537601216_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537601217_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537601218_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537601219_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537601220_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{86.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537601221_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{76.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537601222_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1893.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1493.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537601223_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1367.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537701224_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{113.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134200542_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134200543_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134200544_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300404_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400408_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030900751_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030900752_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030900753_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030900754_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030900755_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030900756_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030900757_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030900758_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030900759_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031000760_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031000761_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031000762_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031000763_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031000764_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031000765_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700872_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700873_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700874_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700875_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700876_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700877_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700878_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700879_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700880_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700881_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700882_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700883_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700884_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900601015_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900601016_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900601017_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900601018_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900601019_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900601020_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500744_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500745_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500746_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500747_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927500748_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896800813_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896800814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896800815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896800816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!LTLMix}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300811_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300812_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300813_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300814_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300815_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852300816_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119000505_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119000506_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119000507_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119000508_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119000509_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119000510_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000679_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500604_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500605_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500606_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500607_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600608_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600609_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600610_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600611_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600612_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100505_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100506_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100507_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100508_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100509_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100510_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900673_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900674_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900675_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900676_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900677_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900678_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000679_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153200611_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153200612_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500673_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500674_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500675_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500676_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500677_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500678_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500679_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100946_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100947_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100948_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100949_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100950_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100951_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100952_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400505_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400506_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400507_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400508_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400509_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400510_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875501184_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875501185_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875501186_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875501187_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{388.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{121.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875501188_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1107.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{694.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875501189_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875501190_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1932.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200811_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200812_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200813_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200814_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200815_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200816_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201015_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201016_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201017_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201018_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891201019_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891301020_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{76.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540401622_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540401623_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540401624_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540401625_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540401626_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540401627_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540501628_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{87.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540501629_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{77.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540501630_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1893.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1458.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540501631_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1442.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540501632_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{109.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134800678_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134800679_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134800680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600506_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600507_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600508_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600509_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600510_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501006_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501007_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501008_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501009_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501010_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501011_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501012_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501013_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501014_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501015_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501016_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501017_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501018_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501019_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032501020_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101093_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101094_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101095_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101096_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101097_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101098_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101099_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101100_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101101_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101102_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101103_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101104_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626101105_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901901355_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902001356_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902001357_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902001358_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902001359_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902001360_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928600931_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928700932_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928700933_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928700934_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928700935_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897501017_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897501018_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897501019_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897501020_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{105.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!LTLMix}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000199_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000200_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{197.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000201_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{368.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000202_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000203_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000204_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600811_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600812_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{374.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{38.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600813_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{641.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2911.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{285.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000811_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000812_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000813_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{203.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701081_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701082_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701083_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701084_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{134.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701085_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701086_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701087_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701088_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901081_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901082_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{128.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901083_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{131.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901084_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901085_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901086_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901087_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569901088_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100232_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100233_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{311.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{40.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100234_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1921.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100235_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{110.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100236_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1002.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{186.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100237_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1446.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393100238_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1982.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300811_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300812_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300813_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901898_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1629.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{223.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901899_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901900_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901901_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901902_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901903_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901904_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901627_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901628_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{910.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901629_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2245.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{224.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901630_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901631_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901632_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400398_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400399_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{166.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400400_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{262.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{565.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400401_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400402_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400403_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400404_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400405_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400406_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400407_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546400408_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136701086_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{403.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136701087_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2990.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{320.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136701088_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500812_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500813_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{351.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{125.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000241_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000242_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{125.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000243_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000244_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000245_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{167.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000246_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{209.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{32.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000247_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{28.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000248_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{741.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{142.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000249_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2227.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{587.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000250_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000251_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{144.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000252_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{162.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000253_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{186.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000254_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{378.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{66.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978035000255_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{940.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{178.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401757_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{163.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401758_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{198.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401759_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{336.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401760_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{678.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{65.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401761_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2943.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{387.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401762_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{305.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401763_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2866.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{318.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401764_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{207.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401765_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{890.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{95.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501766_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501767_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{325.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501768_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2813.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{316.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904800335_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{345.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1335.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904800336_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{431.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{68.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904800337_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2570.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{410.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904800338_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904800339_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904800340_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901492_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{152.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901493_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901494_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{833.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901495_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2030.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{263.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901496_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{302.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501629_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{213.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501630_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1490.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{128.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501631_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501632_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!LTLMix}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853101015_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853101016_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853101017_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853101018_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853101019_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853201020_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600607_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600608_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600609_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600610_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600611_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{187.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{499.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1444.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857100757_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857100758_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857100759_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857100760_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857100761_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857100762_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857100763_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857100764_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857100765_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400607_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400608_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400609_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400610_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400611_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200809_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200810_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200811_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200812_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200813_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153700764_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153700765_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{344.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1026.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900809_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900810_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900811_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900812_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900813_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392701184_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392701185_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392701186_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392701187_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392701188_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392701189_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392701190_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700607_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700608_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700609_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700610_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700611_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301422_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301423_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301424_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301425_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{409.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{131.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301426_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1126.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{707.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301427_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{91.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301428_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1980.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891801015_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891801016_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891801017_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891801018_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891801019_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891801020_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892101219_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201220_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201221_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201222_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201223_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201224_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{87.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543302030_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543302031_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543302032_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543302033_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543302034_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543302035_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543302036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{95.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543402037_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{313.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{74.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543402038_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1920.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1450.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543402039_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1487.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543402040_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{253.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135400814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135400815_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135400816_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900608_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900609_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900610_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900611_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801261_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801262_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801263_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801264_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801265_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801266_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801267_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801268_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801269_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801270_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801271_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801272_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801273_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801274_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033801275_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501314_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501315_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501316_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501317_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501318_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501319_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501320_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501321_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501322_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501323_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501324_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501325_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501326_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903001695_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903101696_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903101697_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903101698_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903101699_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{107.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903101700_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{348.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{204.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701118_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701119_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701120_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701121_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929701122_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201221_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201222_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201223_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{79.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201224_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{951.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_LTLPlaceComparison.tex <==

\section{Executions Reported for LTLPlaceComparison  (``Known'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000163_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000164_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000165_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000166_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000167_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850000168_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300181_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300182_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300183_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300184_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300185_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117300186_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300247_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300248_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900121_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900122_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900123_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900124_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900125_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854900126_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100181_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100182_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100183_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100184_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100185_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890100186_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300241_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300242_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300243_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300244_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300245_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300246_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300247_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300248_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400125_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152400126_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000241_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000242_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000243_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000244_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000245_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000246_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000247_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567000248_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600190_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600191_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600192_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600193_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600194_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600195_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390600196_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800181_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800182_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800183_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800184_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800185_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593800186_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200428_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200429_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200433_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873200434_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400163_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400164_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889400165_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500166_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500167_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889500168_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800367_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800368_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800369_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800370_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800371_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888800372_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300326_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300327_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300328_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300329_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300330_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300331_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300332_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300333_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300334_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300335_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968531300336_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132500246_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132500247_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132500248_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800182_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800183_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800184_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800185_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217800186_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900196_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900197_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900198_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900199_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900200_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900201_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900202_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900203_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900204_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900205_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900206_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900207_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900208_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027900209_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028000210_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700391_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624700392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800393_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800394_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800395_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800396_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800397_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800398_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800399_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800400_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800401_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800402_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624800403_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897900275_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897900276_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897900277_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897900278_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897900279_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897900280_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925200337_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925200338_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925200339_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925200340_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925200341_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600367_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600368_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600369_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600370_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600371_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850600372_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800283_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800284_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800285_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117800287_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941740800288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500383_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308500384_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400271_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400272_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400273_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400274_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400275_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400276_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400277_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400278_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855400279_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400283_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400284_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400285_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400287_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890400288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500377_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500378_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500379_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500380_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500381_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500382_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500383_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500384_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600278_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152600279_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500377_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500378_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500379_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500380_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500381_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500382_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500383_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567500384_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000428_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000429_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000430_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000431_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000432_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000433_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391000434_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300283_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300284_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300285_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300287_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594300288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900666_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900667_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900668_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900669_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900670_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900671_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873900672_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000367_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000368_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000369_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000370_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000371_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890000372_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500571_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500572_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500573_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500574_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500575_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889500576_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100734_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100735_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100736_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100737_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100738_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100739_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100740_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100741_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100742_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100743_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{100.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534100744_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133200382_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133200383_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133200384_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000284_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218000285_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100287_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100451_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100452_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100453_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100454_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100455_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100456_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100457_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100458_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100459_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100460_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100461_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100462_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029100463_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200464_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029200465_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200613_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200614_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200617_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200618_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200619_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200620_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200621_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200622_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200623_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625200624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899100615_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899100616_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899100617_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899100618_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899100619_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899100620_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926400524_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926400525_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926400526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926400527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926500528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400571_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400572_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400573_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400574_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400575_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851400576_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400385_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400386_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400387_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400388_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400389_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118400390_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700519_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308700520_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900424_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900425_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900426_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900427_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900428_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900429_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900430_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900431_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855900432_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700385_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700386_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700387_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700388_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700389_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890700390_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700513_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700514_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700515_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700516_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700517_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700518_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700519_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433700520_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900431_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900432_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900513_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900514_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900515_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900516_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900517_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900518_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900519_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567900520_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500666_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500667_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500668_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500669_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500670_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391500671_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391600672_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700385_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594700386_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594800387_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594800388_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594800389_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594800390_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500904_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500905_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874500906_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600907_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600908_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600909_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874600910_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500571_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500572_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500573_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500574_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500575_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890500576_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200775_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200776_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200777_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200778_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890200779_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890300780_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537001142_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537001143_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537001144_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537001145_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537001146_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537001147_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537001148_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537101149_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537101150_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537101151_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{100.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968537101152_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134000518_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134000519_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134000520_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300386_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300387_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300388_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300389_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218300390_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600706_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030600707_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700708_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700709_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700710_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700711_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700712_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700713_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700714_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700715_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700716_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700717_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700718_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700719_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030700720_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600833_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600834_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600835_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600836_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600837_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600838_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600839_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600840_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600841_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600842_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600843_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600844_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625600845_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900300955_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900300956_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900300957_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900300958_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900300959_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900300960_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400711_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400712_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400713_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400714_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927400715_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200775_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200776_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200777_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200778_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200779_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852200780_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900487_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900488_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900489_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900490_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900491_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118900492_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000655_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400577_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400578_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400579_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400580_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400581_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856400582_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500583_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500584_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856500585_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000487_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000488_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000489_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000490_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000491_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891000492_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900649_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900650_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900651_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900652_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900653_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900654_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900655_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433900656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100584_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153100585_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400649_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400650_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400651_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400652_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400653_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400654_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400655_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568400656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100904_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100905_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100906_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100907_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100908_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100909_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392100910_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300487_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300488_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300489_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300490_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300491_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595300492_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301142_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301143_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301144_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301145_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301146_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301147_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875301148_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100775_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100776_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100777_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100778_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100779_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891100780_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100979_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100980_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100981_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100982_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100983_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891100984_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901550_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901551_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901552_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901553_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901554_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901555_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901556_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901557_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901558_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901559_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{100.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968539901560_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134700654_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134700655_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134700656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600488_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600489_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600490_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600491_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600492_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200961_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200962_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032200963_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300964_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300965_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300966_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300967_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300968_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300969_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300970_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300971_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300972_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300973_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300974_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032300975_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001054_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001055_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001056_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001057_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001058_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001059_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001060_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001061_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001062_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001063_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001064_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001065_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626001066_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801295_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801296_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801297_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801298_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801299_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901801300_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928400898_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928400899_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928500900_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928500901_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928500902_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900163_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900164_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{197.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{27.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900165_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{368.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{56.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900166_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900167_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853900168_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500793_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500794_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{374.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{38.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500795_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{640.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{61.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500796_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2911.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{289.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500797_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120500798_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000793_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{125.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000794_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{134.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000795_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{203.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000796_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000797_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000798_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601057_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601058_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601059_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601060_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601061_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601062_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601063_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434601064_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801057_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801058_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801059_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801060_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801061_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801062_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801063_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569801064_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000190_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{33.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000191_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{312.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{46.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000192_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{464.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000193_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{106.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000194_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1003.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{203.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000195_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1446.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{280.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393000196_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1983.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{347.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200793_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200794_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{139.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200795_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200796_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200797_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596200798_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801856_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1625.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{215.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801857_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801858_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801859_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801860_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801861_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877801862_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701591_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701592_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{909.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{100.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701593_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2246.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{228.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701594_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701595_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893701596_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900326_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900327_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{166.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900328_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{255.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900329_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900330_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900331_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900332_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900333_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900334_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900335_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968545900336_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136601062_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{403.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136601063_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2989.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{305.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136601064_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219400794_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219400795_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{351.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219400796_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{124.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219400797_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219400798_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800196_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800197_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{125.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800198_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{128.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800199_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800200_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{167.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800201_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{209.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800202_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{38.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800203_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{742.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{114.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800204_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2225.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{628.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800205_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800206_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{144.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034800207_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{162.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900208_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{186.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900209_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{378.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034900210_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{940.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{221.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627301718_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{163.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401719_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{198.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401720_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{337.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401721_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{678.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{66.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401722_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2937.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{367.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401723_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{298.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401724_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2866.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{313.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401725_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{207.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401726_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{889.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{96.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401727_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401728_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{301.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627401729_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2813.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{305.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904300275_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{163.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904300276_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{431.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{61.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904300277_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2570.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{445.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904400278_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904400279_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904400280_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931701459_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{151.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931701460_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931701461_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{833.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{80.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931701462_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2030.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{221.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931801463_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{290.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900979_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900980_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900981_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900982_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900983_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852900984_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500589_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500590_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500591_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500592_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500593_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119500594_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309200792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000730_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000731_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000732_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000733_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000734_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000735_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000736_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000737_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941857000738_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400589_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400590_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400591_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400592_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400593_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400594_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100785_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100786_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100787_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100788_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100789_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100790_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434100792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153600737_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153600738_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800785_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800786_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800787_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800788_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800789_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800790_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568800791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501142_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501143_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501144_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501145_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392501146_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601147_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392601148_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600589_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600590_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600591_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600592_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600593_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595600594_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201380_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201381_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201382_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201383_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201384_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201385_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876201386_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700979_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700980_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700981_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700982_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700983_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891700984_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001183_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001184_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001185_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001186_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001187_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892001188_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801958_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801959_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801960_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801961_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801962_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801963_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801964_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801965_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801966_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801967_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{100.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968542801968_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135300790_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135300791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135300792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800590_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218800591_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900592_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900593_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900594_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601216_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601217_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601218_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601219_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601220_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601221_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601222_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601223_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601224_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601225_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601226_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601227_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601228_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601229_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033601230_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501275_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501276_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501277_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501278_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501279_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501280_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501281_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501282_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501283_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501284_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501285_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501286_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626501287_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901635_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901636_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901637_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901638_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901639_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902901640_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929601085_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929601086_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929601087_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929601088_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929601089_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_ReachabilityCardinalityComparison.tex <==

\section{Executions Reported for ReachabilityCardinalityComparison  (``Known'' models)}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200259_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200260_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200261_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{570.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{340.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300262_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1508.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300263_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1727.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300264_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2170.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2312.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201393_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201394_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201395_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301396_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{179.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301397_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{766.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2561.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301398_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1378.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{882.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301399_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1387.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301400_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{461.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100197_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{320.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100198_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301393_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301394_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301395_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{404.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{52.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301396_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{653.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301397_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1214.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{774.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301398_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1357.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{515.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301399_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1809.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2189.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301400_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{239.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001045_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001046_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{391.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{236.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001047_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{487.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001048_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001049_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{562.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001050_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{621.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400259_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{876.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400260_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400261_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400262_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400263_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400264_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547200518_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547200519_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547200520_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{823.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{363.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547200521_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1097.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547200522_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1671.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{930.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547200523_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1747.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{316.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547300524_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547300525_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{119.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547300526_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547300527_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{499.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547300528_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138201398_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1085.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{590.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138201399_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2057.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1440.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138201400_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2594.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{144.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905300435_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905300436_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{180.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905300437_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1707.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{299.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905300438_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{134.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905400439_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{409.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905400440_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{its-tools}}
\index{Execution!ITS-Tools!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{its-tools} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!CSRepetitions (colored)}
\subsubsection{Report for CSRepetitions (colored)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100253_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100254_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100255_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2792.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{557.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100256_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2822.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{617.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100257_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{970.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100258_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2777.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{574.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!DotAndBoxes (colored)}
\subsubsection{Report for DotAndBoxes (colored)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101257_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101258_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101259_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101260_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{752.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!DrinkVendingMachine (colored)}
\subsubsection{Report for DrinkVendingMachine (colored)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101261_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101262_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400943_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400944_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400945_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400946_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400947_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400948_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435001262_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!GlobalRessAlloc (colored)}
\subsubsection{Report for GlobalRessAlloc (colored)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000190_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000191_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{190.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000192_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/06 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1196.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{494.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000193_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2774.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{487.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000194_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/09 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2778.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{564.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000195_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2771.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{560.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000196_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/11 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2790.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{508.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!LamportFastMutEx (colored)}
\subsubsection{Report for LamportFastMutEx (colored)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900295_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900296_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900297_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1339.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{316.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900298_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1808.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{639.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900299_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{531.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900300_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2828.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{562.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900301_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2829.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{560.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!NeoElection (colored)}
\subsubsection{Report for NeoElection (colored)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878902199_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878902200_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878902201_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1410.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{336.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878902202_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{437.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878902203_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{465.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878902204_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2844.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{528.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878902205_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{606.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PermAdmissibility (colored)}
\subsubsection{Report for PermAdmissibility (colored)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600253_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600254_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2424.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{494.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600255_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2639.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{504.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600256_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2731.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{638.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600257_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2426.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{505.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600258_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2686.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{631.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Peterson (colored)}
\subsubsection{Report for Peterson (colored)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101885_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101886_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{442.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{39.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101887_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2802.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{369.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101888_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{423.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101889_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{427.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101890_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2835.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{412.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SharedMemory (colored)}
\subsubsection{Report for SharedMemory (colored)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100421_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100422_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100423_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100424_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100425_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200426_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200427_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000500 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200428_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/001000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200429_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/002000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200430_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/005000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200431_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/010000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200432_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/020000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200433_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/050000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200434_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/100000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200435_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200436_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200437_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200438_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200439_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896200440_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SimpleLoadBal (colored)}
\subsubsection{Report for SimpleLoadBal (colored)}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933301729_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933301730_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933301731_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{648.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{66.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933301732_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{470.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933301733_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2826.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{444.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700055_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700056_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{275.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{254.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700057_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1245.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700058_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{865.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700059_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700060_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100127_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100128_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{39.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100129_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{895.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100130_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2508.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100131_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2116.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100132_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1225.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200175_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200176_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2875.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{238.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600037_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{141.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600038_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600039_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{250.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600040_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{206.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600041_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{773.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600042_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{427.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600043_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600044_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{344.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600045_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{88.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000127_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000128_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000129_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000130_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000131_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1291.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000132_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1083.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100169_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100170_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200171_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{127.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200172_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{467.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200173_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{960.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200174_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{405.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200175_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{437.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200176_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{683.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300044_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300045_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{462.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800169_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800170_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1501.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{270.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800171_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{700.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800172_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{367.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800173_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800174_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{200.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800175_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1060.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800176_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{366.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300064_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300065_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300066_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300067_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300068_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300069_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300070_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500127_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{356.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{120.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500128_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{134.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600129_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600130_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{234.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600131_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{99.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600132_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{202.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800302_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800303_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{234.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2971.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{732.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800305_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{472.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{153.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800306_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800307_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800308_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1927.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200055_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200056_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1272.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200057_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{615.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200058_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200059_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2535.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200060_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500259_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500260_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{576.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{55.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500261_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{731.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500262_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{336.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500263_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500264_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530000110_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530000111_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530000112_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{671.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530000113_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530000114_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530000115_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530000116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{206.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530000117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{718.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{254.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530000118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2356.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530000119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1355.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530100120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{914.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132100174_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132100175_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{74.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{370.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132100176_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{458.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600128_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600129_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{214.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{77.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600130_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{494.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700131_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700132_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1061.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300061_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300062_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300063_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300064_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300065_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300066_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300067_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300068_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{364.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300069_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{66.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300070_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300071_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300072_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300073_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{98.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300074_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{355.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027300075_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{215.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600274_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{158.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600275_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600276_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600277_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600278_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600279_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600280_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600281_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600282_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600283_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600284_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600285_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300095_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300096_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{432.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{512.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300097_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{277.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300098_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300099_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{906.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{377.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300100_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2874.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{992.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800238_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800239_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800240_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800241_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800242_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1270.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300259_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300260_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{275.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{296.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300261_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1356.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300262_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{876.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300263_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300264_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500229_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500230_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{32.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500231_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{895.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500232_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2478.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500233_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2099.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941740700234_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400311_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400312_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2874.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{262.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100190_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{134.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100191_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100192_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{233.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100193_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{193.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100194_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{717.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100195_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{393.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100196_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100197_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{332.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100198_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{85.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300229_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300230_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300231_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300232_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300233_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1248.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300234_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1061.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400305_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400306_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400307_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{127.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400308_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{460.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400309_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{944.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400310_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{416.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400311_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{465.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400312_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{658.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500197_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500198_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{465.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200305_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200306_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1501.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{244.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200307_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{629.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200308_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{362.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200309_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200310_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{207.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200311_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1099.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200312_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{368.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800302_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800303_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800304_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800305_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800306_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800307_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800308_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000229_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{356.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{118.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000230_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{115.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000231_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000232_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{219.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000233_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{89.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000234_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{179.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500540_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500541_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{234.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500542_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2971.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{748.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500543_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{472.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{166.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500544_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500545_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500546_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1928.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700259_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700260_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1232.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700261_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{605.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700262_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700263_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2448.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700264_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200463_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200464_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{576.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{47.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200465_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{708.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200466_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{339.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200467_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200468_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532500518_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532500519_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532500520_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{741.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532500521_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532500522_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532500523_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532500524_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{205.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532600525_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{718.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{249.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532600526_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2338.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532600527_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1370.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532600528_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{978.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132800310_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132800311_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{73.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{382.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132800312_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{457.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900230_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900231_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{214.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{61.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900232_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{486.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900233_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900234_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1059.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400316_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500317_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500318_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500319_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500320_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500321_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500322_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500323_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{362.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500324_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{63.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500325_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500326_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500327_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500328_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{97.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500329_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{363.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028500330_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{251.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000495_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{158.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000496_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000497_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000498_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000499_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000500_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000501_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000502_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000503_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000504_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000505_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000506_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000507_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898400435_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898400436_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{432.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{501.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898500437_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{274.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898500438_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898500439_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{906.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{384.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898500440_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2874.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{979.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925800425_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925800426_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925800427_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925800428_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925800429_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1269.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900463_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900464_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{356.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{78.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900465_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1504.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900466_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1716.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900467_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900468_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100331_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100332_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100333_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1414.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2280.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2118.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1306.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600447_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600448_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2874.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{233.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600343_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600344_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600345_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600346_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600347_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600348_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600349_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600350_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600351_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600331_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{268.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600332_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{278.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600333_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600441_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600442_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600443_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600444_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{317.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{264.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600445_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2115.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600446_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{437.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600447_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{686.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600448_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2053.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700350_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700351_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{716.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700441_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700442_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{444.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{66.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700443_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{859.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700444_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{477.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700445_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700446_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{239.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700447_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{768.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700448_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{395.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300540_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300541_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300542_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300543_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300544_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300545_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300546_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500331_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{473.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500332_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2843.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{55.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500333_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{281.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{144.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2844.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{81.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{169.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200778_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200779_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{338.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{52.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200780_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{422.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200781_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{609.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200782_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{316.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200783_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200784_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1926.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200463_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200464_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300465_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300466_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300467_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300468_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900667_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900668_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900669_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900670_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{311.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900671_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900672_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{274.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500926_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500927_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500928_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{391.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500929_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500930_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500931_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500932_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{205.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500933_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{718.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{263.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500934_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2300.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500935_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1374.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535500936_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1020.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133600446_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133600447_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{367.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133600448_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{543.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200332_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200333_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{359.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{761.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2636.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{875.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800571_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800572_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800573_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800574_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900575_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900576_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900577_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900578_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{307.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900579_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900580_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900581_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900582_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900583_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900584_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1008.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029900585_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{443.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300716_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{275.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400717_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{283.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400718_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400719_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{285.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400720_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400721_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400722_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400723_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400724_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400725_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400726_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400727_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{309.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400728_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{358.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899600775_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899600776_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{208.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899600777_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1011.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899600778_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899700779_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{906.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{343.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899700780_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{999.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927000612_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{288.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927000613_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927000614_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2328.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927000615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1705.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927000616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{597.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700667_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700668_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700669_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{502.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800670_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{98.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800671_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800672_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600433_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600434_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600435_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{116.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600436_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600437_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600438_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{379.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308800583_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308800584_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2874.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{243.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100496_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100497_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1864.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100498_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1432.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100499_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1518.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100500_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100501_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100502_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2110.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100503_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100504_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1968.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900433_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900434_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900435_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900436_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900437_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900438_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800577_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800578_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800579_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800580_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800581_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800582_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800583_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800584_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000503_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{115.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000504_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{472.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{344.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100577_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100578_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200579_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200580_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200581_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200582_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200583_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200584_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800778_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800779_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800780_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800781_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800782_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800783_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800784_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000433_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000434_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000435_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{461.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000436_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{582.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100437_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{909.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100438_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{931.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901016_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901017_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{126.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{92.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901018_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1863.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901019_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{480.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{158.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901020_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901021_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901022_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1927.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700667_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700668_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{247.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700669_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{264.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800670_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{340.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800671_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{427.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800672_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600871_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600872_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600873_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1608.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600874_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2361.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600875_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600876_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501334_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501335_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501336_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{721.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501337_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501338_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501339_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501340_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{205.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501341_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{718.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{241.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501342_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2335.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501343_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538501344_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1030.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134300582_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134400583_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1641.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134400584_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{412.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400434_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400435_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{225.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{259.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400436_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1003.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400437_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400438_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{96.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400826_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500827_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500828_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500829_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500830_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500831_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500832_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500833_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1231.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500834_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1739.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500835_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500836_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500837_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500838_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500839_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031500840_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2512.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800937_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2371.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800938_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800939_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800940_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800941_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800942_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{94.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800943_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{527.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800944_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{330.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800945_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800946_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800947_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800948_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{104.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800949_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901101115_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901101116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901101117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901101118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901101119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{906.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{348.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901101120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2875.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{980.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927800799_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927800800_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927800801_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{207.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927800802_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927800803_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{143.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600055_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600056_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600057_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600058_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600059_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600060_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1141.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700637_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700638_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700639_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700640_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700641_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{753.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700642_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{928.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300855_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300856_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1333.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{158.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600037_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{922.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600038_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1096.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600039_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600040_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600041_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{870.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600042_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1105.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600043_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600044_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{940.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600045_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1107.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500637_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500638_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500639_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500640_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500641_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500642_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200849_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200850_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200851_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200852_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{673.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200853_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{861.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200854_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2405.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1519.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200855_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2339.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200856_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1993.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800044_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800045_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1016.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000849_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100850_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100851_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100852_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{750.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100853_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1819.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{67.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100854_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100855_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100856_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600064_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600065_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600066_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{759.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600067_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{844.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600068_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{829.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600069_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{799.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600070_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{852.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800637_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800638_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800639_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{680.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800640_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{845.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800641_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800642_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2009.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601492_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601493_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601494_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{800.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601495_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{949.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601496_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1151.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601497_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1175.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601498_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1196.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100055_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{683.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{85.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100056_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{805.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100057_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100058_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1314.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100059_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1289.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2597.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100060_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1287.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401279_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401280_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{838.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{52.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401281_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{744.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401282_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401283_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{771.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401284_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524800110_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524800111_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524800112_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524800113_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524800114_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{681.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524900115_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{735.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524900116_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{102.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524900117_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1185.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1183.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524900118_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1213.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524900119_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1290.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524900120_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135600854_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135600855_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135600856_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{772.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000638_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000639_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{716.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000640_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{724.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000641_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000642_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500061_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500062_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500063_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500064_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500065_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500066_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500067_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500068_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{674.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500069_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500070_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024600071_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024600072_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024600073_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024600074_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024600075_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{715.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601379_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{671.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601380_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601381_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601382_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601383_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601384_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601385_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{787.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{613.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601386_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{989.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601387_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601388_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1178.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{27.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701389_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701390_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{47.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701391_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{111.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200095_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200096_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200097_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200098_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200099_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1199.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200100_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901173_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930001174_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930001175_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1123.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1384.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930001176_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1112.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930001177_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1077.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500871_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500872_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500873_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500874_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500875_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500876_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119200535_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119200536_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119200537_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119200538_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119200539_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119200540_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100719_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100720_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700649_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700650_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700651_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700652_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700653_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700654_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700655_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700656_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700657_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200535_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200536_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200537_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200538_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200539_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200540_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000713_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000714_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000715_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000716_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000717_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000718_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000719_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000720_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153400656_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153400657_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600713_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600714_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600715_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600716_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600717_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600718_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600719_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600720_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301016_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301017_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301018_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301019_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301020_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301021_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301022_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500535_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500536_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500537_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500538_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500539_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{127.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500540_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701254_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701255_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701256_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{152.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701257_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{463.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{153.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701258_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701259_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701260_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1927.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300871_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300872_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300873_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300874_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300875_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300876_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501075_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501076_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501077_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501078_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501079_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501080_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541201742_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541201743_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541201744_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541201745_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541201746_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541201747_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541301748_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{205.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541301749_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{715.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{244.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541301750_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2225.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541301751_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1454.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541301752_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1043.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135000718_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135000719_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135000720_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700536_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700537_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700538_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700539_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700540_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901081_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901082_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901083_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901084_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901085_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901086_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901087_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901088_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901089_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901090_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901091_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901092_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901093_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901094_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901095_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201158_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201159_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201160_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201161_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201162_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201163_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201164_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201165_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201166_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201167_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201168_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201169_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201170_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301455_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301456_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301457_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301458_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301459_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301460_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929000986_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929000987_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929000988_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929000989_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929000990_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_ReachabilityDeadlock.tex <==

\section{Executions Reported for ReachabilityDeadlock  (``Known'' models)}
\subsection{Relevant Executions for \acs{cunf}}
\index{Execution!cunf!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{cunf} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933856300427_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933856300428_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2870.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{597.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933856300429_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{519.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933856300430_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933856400431_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{841.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933856400432_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2571.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941742201129_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941742201130_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941742201131_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941742201132_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{164.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941742201133_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1714.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{46.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310601511_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{200.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941893001129_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941893001130_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941893001131_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941893001132_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941893001133_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952155300323_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2989.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{353.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394400498_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394400499_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{143.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394400500_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2929.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{379.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394400501_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{833.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394400502_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{638.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394400503_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{792.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394400504_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{929.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959880102640_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959880102641_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{610.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{49.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893900427_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{393.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966896902263_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966896902264_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966896902266_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2161.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966896902267_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2263.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966896902268_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1932.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968555100854_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968555100855_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968555100856_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968555100857_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968555100858_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968555100859_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968555100860_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{106.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968555100861_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968555100862_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{874.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138701510_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2533.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138801512_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{466.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975220401130_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975220401131_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{392.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{304.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975220401132_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{932.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975220401133_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1820.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200526_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200527_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200528_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200529_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200530_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200531_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200532_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200533_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200534_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200535_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038200536_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038300537_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038300538_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038300539_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978038300540_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2869.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{74.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802446_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802447_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802448_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802449_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802450_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802451_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802452_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{160.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802453_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802454_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802455_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802456_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{115.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980628802457_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{349.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983909300715_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983909300716_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983909300717_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983909300718_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{85.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983909300719_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{177.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983909300720_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983935002075_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983935102076_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{230.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983935102077_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1375.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983935102078_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1497.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983935102079_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1270.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989902102265_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989902102266_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100223_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100224_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100225_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{490.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100226_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1417.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100227_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1791.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100228_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2170.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2390.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201369_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201370_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201371_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201372_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201373_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{111.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201374_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{370.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{116.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201375_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1396.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201376_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{463.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154000170_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{321.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154000171_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201369_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201370_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201371_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201372_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{102.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201373_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{446.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{68.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201374_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1357.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{531.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201375_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1809.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2224.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201376_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901027_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901028_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901029_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{286.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901030_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901031_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{562.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901032_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{621.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300223_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{889.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2432.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300224_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300225_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300226_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300227_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300228_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546700446_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546700447_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546700448_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{73.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546700449_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{714.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{163.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546700450_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1136.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546800451_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{981.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546800452_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546800453_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546800454_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{222.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546800455_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{502.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546800456_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138101374_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1060.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{166.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138101375_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2030.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1142.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138101376_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2594.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{153.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905000375_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905000376_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905000377_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1705.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{308.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905000378_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905000379_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{410.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905000380_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901402061_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901402062_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1744.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901402063_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1888.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{86.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901402064_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{its-tools}}
\index{Execution!ITS-Tools!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{its-tools} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!CSRepetitions (colored)}
\subsubsection{Report for CSRepetitions (colored)}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000217_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000218_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000219_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2793.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{601.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000220_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2822.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{573.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000221_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1010.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000222_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2776.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{641.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!DotAndBoxes (colored)}
\subsubsection{Report for DotAndBoxes (colored)}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001233_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001234_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001235_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001236_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{753.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!DrinkVendingMachine (colored)}
\subsubsection{Report for DrinkVendingMachine (colored)}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001237_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001238_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!GlobalRessAlloc (colored)}
\subsubsection{Report for GlobalRessAlloc (colored)}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000163_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000164_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{190.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000165_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/06 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1196.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{255.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000166_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2774.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{587.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000167_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/09 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2778.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{507.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000168_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2312.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{540.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000169_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/11 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2791.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{514.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!LamportFastMutEx (colored)}
\subsubsection{Report for LamportFastMutEx (colored)}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900253_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900254_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900255_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1339.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{352.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900256_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1808.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{574.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900257_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{641.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900258_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2828.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{622.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900259_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2829.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{596.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!NeoElection (colored)}
\subsubsection{Report for NeoElection (colored)}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702157_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702158_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702159_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1410.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{314.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702160_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{410.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702161_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{479.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702162_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2843.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{512.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702163_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{606.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PermAdmissibility (colored)}
\subsubsection{Report for PermAdmissibility (colored)}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500217_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500218_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2423.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{492.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500219_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2641.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{528.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500220_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2731.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{590.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500221_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2426.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{513.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500222_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2685.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{619.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Peterson (colored)}
\subsubsection{Report for Peterson (colored)}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001849_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001850_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{442.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001851_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2801.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{338.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001852_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{417.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001853_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{410.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001854_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2836.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{400.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SimpleLoadBal (colored)}
\subsubsection{Report for SimpleLoadBal (colored)}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933101696_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933101697_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933101698_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{648.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{64.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933101699_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{447.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933101700_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2825.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{423.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600019_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600020_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600021_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600022_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600023_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600024_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000109_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000110_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000111_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{890.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2527.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000112_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2131.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000113_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1070.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000114_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308100151_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308100152_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3166.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1505.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500010_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500011_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500012_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500013_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500014_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500015_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500016_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500017_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500018_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900109_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900110_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900111_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900112_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900113_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900114_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100145_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100146_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100147_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100148_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100149_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100150_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100151_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{74.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100152_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152200017_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152200018_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{583.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700145_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700146_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700147_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700148_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{555.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700149_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{129.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700150_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{126.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700151_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{118.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700152_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{119.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300022_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300023_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300024_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300025_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1997.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300026_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1743.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300027_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2394.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300028_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2760.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500109_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500110_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{205.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500111_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{123.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500112_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{91.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500113_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{80.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500114_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{77.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700260_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700261_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700262_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700263_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700264_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{87.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700265_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{131.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700266_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{211.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100019_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100020_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100021_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100022_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100023_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100024_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888300223_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888300224_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{86.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888300225_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{286.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888300226_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{196.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888300227_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{254.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400228_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2862.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{346.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529500038_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529500039_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529500040_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529500041_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529500042_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529500043_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529500044_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529500045_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529500046_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{115.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529600047_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{383.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529600048_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1190.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{104.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972131900150_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972131900151_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972131900152_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{356.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600110_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600111_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600112_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1102.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600113_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{786.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600114_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027000016_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027000017_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027000018_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027000019_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027000020_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027000021_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027000022_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100023_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100024_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100025_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100026_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100027_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100028_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100029_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100030_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500235_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{122.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500236_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500237_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500238_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500239_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500240_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500241_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500242_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{105.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500243_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500244_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500245_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500246_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500247_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897100035_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897100036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897100037_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{279.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897100038_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2869.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{898.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897100039_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2923.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{562.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897100040_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3114.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{505.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924700205_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924700206_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924700207_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{896.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{650.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924700208_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{954.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924700209_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{515.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894900225_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894900226_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894900227_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{337.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894900228_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{595.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200223_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200224_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200225_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200226_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200227_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200228_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400211_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400212_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400213_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{890.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2453.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400214_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2122.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117400215_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1071.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300287_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308300288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3175.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1479.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000163_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000164_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000165_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000166_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000167_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000168_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000169_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000170_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000171_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200211_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200212_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200213_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200214_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200215_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200216_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300281_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300282_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300283_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300284_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300285_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300287_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{76.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500170_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500171_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{261.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567100281_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200282_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200283_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200284_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{554.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200285_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{110.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{112.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200287_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{101.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{102.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700260_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700261_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700262_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{33.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700263_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1855.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700264_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1669.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700265_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2345.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700266_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2776.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900211_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900212_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{187.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900213_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{110.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900214_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{79.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900215_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{68.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593900216_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2844.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{63.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873300498_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400499_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400500_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400501_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400502_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{87.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400503_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{131.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400504_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{211.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600223_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600224_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600225_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600226_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600227_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600228_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889000427_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889000428_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{86.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889000429_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{244.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889000430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{201.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889000431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{252.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{359.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100446_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100447_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100448_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100449_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100450_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100451_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100452_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100453_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100454_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{111.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100455_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{384.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532100456_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1190.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{245.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132700286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132700287_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132700288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{356.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900212_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900213_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900214_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1085.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900215_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{788.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900216_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300271_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300272_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300273_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300274_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300275_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300276_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300277_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300278_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300279_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300280_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300281_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300282_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300283_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300284_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300285_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900456_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{136.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900457_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900458_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900459_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900460_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900461_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900462_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900463_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900464_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900465_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900466_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900467_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900468_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898200375_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300376_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300377_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{277.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300378_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2869.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{905.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300379_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2923.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{768.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300380_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3118.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{458.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925500392_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925600393_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925600394_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{897.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{605.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925600395_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{957.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925600396_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{514.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895600429_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895600430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895600431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{337.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895600432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{596.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850800427_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{283.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850800428_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{267.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850800429_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850800430_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850800431_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850800432_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000313_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000314_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000315_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1529.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000316_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2355.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000317_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1098.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000318_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{913.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600423_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{262.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600424_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3181.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1500.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500316_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500317_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500318_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500319_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500320_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500321_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500322_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{318.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500323_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{305.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500324_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{321.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500313_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{253.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500314_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{239.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500315_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500316_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{251.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500317_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{239.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500318_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500417_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{236.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500418_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{283.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500419_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{242.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500420_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500421_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500422_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500423_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500424_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700323_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{319.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700324_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{842.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600417_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{243.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600418_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{229.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600419_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600420_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600421_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{148.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600422_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{521.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600423_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{684.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600424_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{609.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200498_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{288.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200499_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200500_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{307.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200501_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{761.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200502_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200503_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{421.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200504_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{346.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400313_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{253.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400314_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2103.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{818.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400315_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{147.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400316_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{114.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400317_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{109.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400318_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{119.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100736_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{229.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100737_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{272.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100738_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{267.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100739_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{323.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100740_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{349.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100741_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{390.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100742_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{413.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200427_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200428_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{274.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200429_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200430_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200431_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200432_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889700631_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889700632_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889700633_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{375.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889700634_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800635_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800636_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{313.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900854_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900855_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900856_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{272.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900857_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900858_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900859_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900860_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{312.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900861_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{323.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900862_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{361.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900863_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{506.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968534900864_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{889.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{209.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133400422_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{237.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133400423_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133500424_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{608.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100314_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{241.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100315_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100316_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2501.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100317_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{630.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100318_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{422.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600526_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{268.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600527_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600528_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{271.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600529_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600530_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600531_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{274.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600532_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600533_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600534_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600535_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{279.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600536_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{279.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600537_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600538_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{286.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600539_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029600540_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300677_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{368.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300678_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300679_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{228.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{265.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300681_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{227.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300682_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{226.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300683_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{236.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300684_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300685_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{232.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300686_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{221.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300687_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{241.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300688_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{259.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300689_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{388.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899400715_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{270.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899400716_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899400717_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899400718_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{382.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899400719_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1231.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899400720_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3109.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{345.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926800579_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{277.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926800580_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926800581_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{312.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{578.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926800582_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{467.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926800583_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{399.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896200633_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{236.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896200634_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896200635_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896200636_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851600631_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851600632_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851600633_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851600634_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851600635_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851600636_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500415_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500416_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1081.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500417_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{121.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500418_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500419_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{121.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118500420_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{528.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308800559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308800560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3177.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1544.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000469_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000470_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000471_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000472_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000473_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000474_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000475_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{372.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856000476_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100477_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{135.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800415_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800416_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800417_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800418_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800419_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{69.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800420_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800553_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800554_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800555_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800556_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800557_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800558_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152900476_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{128.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2463.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000477_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{627.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1947.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100553_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100554_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100555_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100556_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100557_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100558_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700736_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700737_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700738_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700739_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{903.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2604.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700740_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1143.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700741_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1123.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700742_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1085.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594900415_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594900416_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594900417_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{205.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000418_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{598.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000419_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{979.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000420_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874700974_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874700975_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800976_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800977_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800978_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{108.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800979_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{165.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800980_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{229.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{41.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600631_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890600632_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700633_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700634_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700635_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700636_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890400835_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890400836_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500837_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1650.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500838_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2400.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500839_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1404.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500840_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2862.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1964.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538001262_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538001263_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538001264_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538001265_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538001266_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538001267_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1273.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538001268_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538001269_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538001270_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{84.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538001271_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{167.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538101272_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134200558_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134200559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134200560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{411.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400416_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400417_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400418_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1038.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400419_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400420_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031100781_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031100782_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031100783_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031100784_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031100785_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031200786_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031200787_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031200788_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031200789_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{49.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031200790_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031200791_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031200792_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031200793_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031200794_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031200795_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700898_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2404.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700899_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700900_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700901_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700902_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700903_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700904_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{122.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{161.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700905_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1471.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700906_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700907_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700908_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700909_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{40.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700910_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{401.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900801055_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900801056_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{823.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900801057_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900801058_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{120.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900801059_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{997.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900801060_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3116.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{340.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927600766_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927600767_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927600768_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{212.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1214.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927600769_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927600770_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{161.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896800837_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896800838_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896800839_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{127.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896900840_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{657.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500019_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500020_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500021_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500022_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500023_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500024_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600619_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600620_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600621_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600622_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600623_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{751.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{929.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300831_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300832_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1331.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500010_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{922.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500011_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1096.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500012_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600013_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600014_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{869.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600015_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1099.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600016_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600017_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{941.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600018_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1109.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500619_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{661.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500620_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500621_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500622_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500623_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200825_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200826_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200827_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200828_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{673.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200829_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{861.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200830_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2405.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1482.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200831_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2298.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200832_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1993.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800017_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{40.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800018_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1016.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000825_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000826_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000827_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000828_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{750.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000829_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1819.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000830_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000831_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000832_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500022_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500023_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500024_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{759.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{72.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500025_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{844.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500026_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500027_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{798.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500028_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{853.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700619_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700620_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700621_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{680.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700622_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{844.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700623_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2009.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401450_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401451_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{800.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401452_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401453_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{949.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401454_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1150.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401455_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1170.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401456_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1195.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000019_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{683.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{81.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000020_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{790.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000021_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000022_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1307.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000023_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1283.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000024_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1287.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201243_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201244_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{838.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{53.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301245_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{744.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301246_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301247_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{771.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301248_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524300038_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524300039_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524300040_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524300041_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524300042_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{681.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524400043_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{735.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524400044_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{70.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524400045_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{624.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524400046_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1212.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524400047_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1287.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524400048_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135500830_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135500831_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135500832_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{772.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900620_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900621_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{716.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900622_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{723.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900623_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300016_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300017_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300018_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300019_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300020_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300021_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300022_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300023_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{674.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300024_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300025_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300026_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300027_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300028_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300029_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400030_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{715.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601340_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{671.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601341_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601342_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601343_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601344_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601345_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601346_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{787.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{617.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601347_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{989.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601348_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2397.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601349_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1178.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601350_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601351_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601352_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{97.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000035_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000036_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000037_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000038_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000039_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1199.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000040_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929801140_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929801141_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929801142_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1123.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1365.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929801143_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1111.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929801144_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1073.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201245_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201246_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201247_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{702.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201248_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1153.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852400835_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852400836_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852400837_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852400838_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852400839_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852400840_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100517_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100518_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100519_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100520_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100521_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100522_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{188.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000695_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000696_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{499.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1454.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600622_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600623_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600624_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600625_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600626_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600627_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600628_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600629_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856600630_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100517_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100518_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100519_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100520_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100521_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100522_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000689_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000690_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000691_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000692_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000693_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000694_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000695_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000696_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153200629_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153200630_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{261.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1412.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500689_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500690_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500691_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500692_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500693_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500694_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500695_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500696_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200974_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200975_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200976_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200977_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200978_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200979_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200980_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400517_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400518_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400519_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400520_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400521_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400522_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875501212_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875501213_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875501214_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601215_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601216_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601217_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{91.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601218_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{122.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200835_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200836_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200837_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200838_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200839_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891200840_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891301039_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401040_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401041_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401042_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401043_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401044_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540701670_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540701671_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540701672_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540701673_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540701674_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540801675_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540801676_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540801677_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540801678_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{73.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540801679_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{134.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540801680_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{236.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134900694_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134900695_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134900696_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600518_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218600519_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700520_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700521_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700522_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032601036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032601037_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032601038_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032601039_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032601040_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032601041_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701042_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701043_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701044_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701045_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701046_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701047_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701048_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701049_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701050_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201119_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201120_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201121_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201122_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201123_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201124_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201125_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201126_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201127_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201128_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201129_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201130_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201131_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902101395_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902101396_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902101397_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902101398_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902101399_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902101400_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{316.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{234.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928800953_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928800954_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928800955_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928800956_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928800957_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897601041_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897601042_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897601043_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897601044_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{383.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_ReachabilityFireability.tex <==

\section{Executions Reported for ReachabilityFireability  (``Known'' models)}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100235_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100236_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200237_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{845.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{624.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200238_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1508.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200239_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1720.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200240_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2170.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2435.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201377_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201378_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201379_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201380_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{79.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201381_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{439.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201382_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{156.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201383_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1399.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201384_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{462.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154000179_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{343.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154000180_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201377_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201378_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201379_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{95.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201380_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{285.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201381_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{770.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201382_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1357.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{514.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201383_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1810.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2339.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201384_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901033_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901034_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001035_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{564.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001036_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001037_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{562.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001038_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{621.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400235_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{890.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400236_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400237_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400238_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400239_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400240_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900470_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900471_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900472_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900473_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1612.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{292.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900474_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1622.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{298.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900475_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1640.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{209.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900476_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900477_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900478_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{212.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900479_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{500.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546900480_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138101382_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{279.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138101383_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2036.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1075.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138101384_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2592.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{123.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905100395_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905100396_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905100397_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1707.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{277.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905100398_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905100399_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{412.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905200400_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901402073_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901402074_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1780.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901402075_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1890.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{93.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901402076_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{its-tools}}
\index{Execution!ITS-Tools!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{its-tools} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!CSRepetitions (colored)}
\subsubsection{Report for CSRepetitions (colored)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000229_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000230_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000231_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2792.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{573.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000232_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2822.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{689.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000233_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2844.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{931.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000234_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2776.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{632.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!DotAndBoxes (colored)}
\subsubsection{Report for DotAndBoxes (colored)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001241_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001242_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001243_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001244_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{782.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!DrinkVendingMachine (colored)}
\subsubsection{Report for DrinkVendingMachine (colored)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001245_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001246_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400931_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400932_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400933_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400934_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400935_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400936_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435001246_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!GlobalRessAlloc (colored)}
\subsubsection{Report for GlobalRessAlloc (colored)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000172_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!LamportFastMutEx (colored)}
\subsubsection{Report for LamportFastMutEx (colored)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900267_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900268_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900269_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1339.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{316.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900270_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1808.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{584.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900271_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{581.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900272_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2827.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{540.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900273_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2829.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{514.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!NeoElection (colored)}
\subsubsection{Report for NeoElection (colored)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802171_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802172_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802174_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{426.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802176_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2844.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{514.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PermAdmissibility (colored)}
\subsubsection{Report for PermAdmissibility (colored)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500229_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500230_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2422.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{495.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500231_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2640.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{501.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500232_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2731.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{592.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500233_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2425.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{501.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500234_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2685.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{614.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Peterson (colored)}
\subsubsection{Report for Peterson (colored)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001861_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001862_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{443.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001863_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2802.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{364.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001864_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{428.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001865_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{444.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895001866_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2837.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{415.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SimpleLoadBal (colored)}
\subsubsection{Report for SimpleLoadBal (colored)}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933101707_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933201708_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933201709_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{648.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{56.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933201710_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{420.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933201711_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2826.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{403.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600031_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600032_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{320.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600033_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1389.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{297.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600034_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{509.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600035_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{676.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{455.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000115_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000116_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000117_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000118_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000119_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000120_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{260.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308100159_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308100160_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2879.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{235.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500019_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2844.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854500020_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600021_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600022_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600023_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600024_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{429.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600025_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600026_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600027_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{364.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900115_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900116_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900117_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900118_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900119_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900120_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100153_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100154_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100155_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100156_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100157_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100158_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100159_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100160_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300026_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{320.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300027_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1742.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700153_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700154_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700155_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700156_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700157_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700158_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700159_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700160_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300037_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300038_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300039_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300040_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300041_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300042_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500115_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500116_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500117_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500118_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500119_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500120_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700274_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700275_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{203.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{97.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700276_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700277_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700278_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700279_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2781.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872700280_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1339.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100031_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100032_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{198.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100033_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100034_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100035_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400235_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400236_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{587.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{96.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400237_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1181.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400238_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{538.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400239_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{619.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400240_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{558.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700062_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700063_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700064_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{528.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700065_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{108.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700066_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700067_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{88.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700068_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{244.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700069_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{116.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700070_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{274.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700071_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2817.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{449.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529700072_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2870.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2560.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132000158_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132000159_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132000160_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{769.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600116_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600117_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{220.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{92.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600118_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1823.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600119_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600120_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1204.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100031_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100032_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100033_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100034_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100035_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{506.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{78.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100037_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100038_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100039_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100040_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100041_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027100042_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200043_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200044_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200045_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500248_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{290.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500249_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500250_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500251_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500252_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500253_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500254_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500255_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500256_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500257_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500258_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500259_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500260_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897200055_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897200056_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{416.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{179.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897200057_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{406.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897200058_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1863.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897200059_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2033.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897200060_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2867.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1012.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800216_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800217_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800218_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800219_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800220_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1203.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894900237_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894900238_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894900239_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{871.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894900240_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{326.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{60.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200235_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200236_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{334.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200237_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1389.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{278.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200238_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{507.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200239_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{697.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850200240_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{450.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500217_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500218_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500219_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500220_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500221_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500222_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{260.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400295_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400296_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2876.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{264.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000172_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855000173_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100174_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100175_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100176_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100177_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{399.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100178_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100179_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100180_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{330.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200217_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200218_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200219_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200220_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200221_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200222_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300289_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300290_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300291_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300292_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300293_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300294_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300295_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300296_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500179_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{320.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500180_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1743.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200289_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200290_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200291_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200292_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200293_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200294_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200295_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200296_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700274_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700275_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700276_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700277_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700278_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700279_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700280_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000217_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000218_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000219_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000220_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000221_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000222_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400512_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400513_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{203.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{97.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400514_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400515_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400516_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400517_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2793.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400518_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1338.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600235_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600236_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{199.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600237_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600238_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600239_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889600240_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100439_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100440_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{587.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{94.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100441_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1177.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100442_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{523.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100443_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{602.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100444_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{552.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532200470_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532200471_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532200472_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{526.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532200473_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{108.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532200474_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532200475_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{91.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532300476_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{241.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532300477_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{121.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532300478_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{243.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532300479_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2837.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{456.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532300480_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2869.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1975.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132700294_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132700295_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{77.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{179.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132700296_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{770.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900218_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900219_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{88.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900220_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1823.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900221_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900222_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1207.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300286_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300287_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300288_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300289_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300290_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300291_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{506.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{79.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300292_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300293_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300294_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300295_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300296_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028300297_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400298_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400299_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400300_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900469_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{275.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900470_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900471_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900472_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900473_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900474_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900475_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900476_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900477_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900478_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900481_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300395_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300396_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{416.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{172.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300397_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{411.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300398_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1812.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300399_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2034.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898300400_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{995.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925600403_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925600404_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925600405_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925600406_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925600407_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1198.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895600441_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895600442_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895600443_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{868.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895600444_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{332.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900439_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900440_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{372.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{82.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900441_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{312.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{128.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900442_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900443_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2666.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900444_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{814.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000319_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000320_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000321_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000322_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{251.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118000323_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{331.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{254.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2875.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{233.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500325_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500326_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500327_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500328_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500329_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855500330_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600331_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600332_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600333_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500319_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500320_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500321_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{274.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500322_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890500323_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{265.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600324_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{278.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500425_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500426_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{255.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433500427_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600428_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600429_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{270.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700332_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{585.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700333_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1866.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600425_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{276.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600426_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600427_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600428_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600429_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567600432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200512_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200513_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200514_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200515_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200516_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200517_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200518_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400319_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400320_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400321_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400322_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400323_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594400324_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{275.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100750_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100751_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{80.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100752_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{313.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100753_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{309.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100754_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{348.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100755_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{358.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874100756_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{476.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200439_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200440_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200441_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{288.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200442_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200443_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200444_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800643_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800644_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800645_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800646_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800647_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{324.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800648_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{363.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535100878_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535100879_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535100880_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{811.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535100881_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{185.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535100882_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535100883_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{207.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535100884_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1404.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535100885_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{255.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535100886_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2332.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535200887_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{629.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535200888_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{765.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133500430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133500431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{332.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{171.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133500432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{917.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100320_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100321_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{364.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100322_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218100323_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2244.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200324_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{781.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700541_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700542_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{286.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700543_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700544_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700545_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700546_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{312.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700547_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700548_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700549_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700550_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700551_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700552_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700553_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{292.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700554_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700555_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300690_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{539.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300691_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300692_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{285.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300693_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300694_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300695_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300696_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300697_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300698_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300699_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{268.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300700_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300701_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{311.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300702_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899500735_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899500736_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{318.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{84.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899500737_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2355.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899500738_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1292.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899500739_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2155.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899500740_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{984.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926800590_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{283.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926800591_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926800592_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2090.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926800593_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1677.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926800594_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{566.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896200645_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{290.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896200646_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{307.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896200647_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{359.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896200648_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{326.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851600643_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851600644_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851600645_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700646_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{96.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700647_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700648_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600421_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600422_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600423_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1461.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600424_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600425_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600426_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{379.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308800567_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308800568_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2878.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{235.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100478_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100479_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100480_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1447.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100481_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100482_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100483_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100484_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2264.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100485_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100486_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1995.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800421_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800422_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800423_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800424_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800425_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890800426_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800561_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800562_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800563_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800564_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800565_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800566_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800567_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800568_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000485_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{376.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000486_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1741.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{552.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100561_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100562_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100563_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100564_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100565_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100566_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100567_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100568_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700750_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700751_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700752_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700753_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700754_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700755_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700756_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000421_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000422_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{27.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000423_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{209.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000424_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{590.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000425_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{965.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000426_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800988_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800989_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{84.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{147.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800990_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800991_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1378.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800992_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{649.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800993_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{510.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874800994_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{399.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700643_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700644_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{239.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700645_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{241.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700646_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{323.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700647_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{422.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700648_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{593.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500847_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500848_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500849_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500850_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1675.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500851_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500852_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2260.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201286_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201287_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201288_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{718.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201289_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{982.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201290_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{114.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201291_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201292_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201293_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201294_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{86.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201295_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{169.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538201296_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{186.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134300566_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134300567_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{79.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134300568_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{776.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400422_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400423_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400424_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{991.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400425_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400426_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{95.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300796_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300797_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300798_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300799_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300800_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300801_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300802_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{200.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{305.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300803_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1193.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300804_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1716.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300805_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300806_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300807_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300808_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300809_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031300810_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700911_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2376.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700912_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700913_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700914_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700915_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700916_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{86.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700917_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{152.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700918_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{330.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700919_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625700920_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800921_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800922_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{231.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800923_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900901075_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900901076_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900901077_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900901078_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900901079_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2036.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983900901080_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2866.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{976.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927600777_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927600778_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927600779_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{183.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927600780_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{242.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927700781_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896900849_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896900850_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{60.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896900851_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{132.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896900852_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{327.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500031_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500032_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{909.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{60.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500033_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500034_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500035_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500036_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1141.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600625_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600626_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{672.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600627_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{721.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700628_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700629_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{751.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700630_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{926.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300839_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300840_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1837.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{757.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600019_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{922.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600020_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1096.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600021_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600022_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600023_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{869.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600024_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1099.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600025_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600026_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{940.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600027_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1107.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500625_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{661.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500626_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500627_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500628_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500629_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{672.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500630_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{713.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200833_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200834_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200835_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200836_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{679.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200837_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1127.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200838_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2405.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1626.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200839_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2232.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200840_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1993.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800026_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{701.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{64.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800027_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1017.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000833_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000834_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000835_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000836_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{759.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000837_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{154.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000838_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000839_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000840_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500036_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500037_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{728.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500038_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{886.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500039_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{842.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500040_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{814.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500041_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{794.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500042_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{841.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700625_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700626_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700627_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{720.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700628_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2551.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{220.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700629_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1181.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700630_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2009.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401464_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{672.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501465_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{838.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501466_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{800.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501467_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{949.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501468_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1151.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501469_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1177.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501470_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1197.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000031_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{736.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{110.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000032_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000033_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{790.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000034_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1284.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000035_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1278.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000036_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1294.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2646.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301255_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{679.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301256_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1161.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301257_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{744.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301258_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301259_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{771.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301260_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524500062_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524500063_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524500064_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524500065_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{880.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524500066_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1156.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1135.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524500067_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1159.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524500068_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1169.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524500069_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524600070_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1212.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524600071_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1287.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524600072_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135500838_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{675.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135500839_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{712.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135500840_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{788.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900626_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900627_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{812.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{76.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900628_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{724.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900629_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000630_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400031_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400032_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400033_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400034_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400035_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400036_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400037_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400038_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{687.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400039_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{740.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400040_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400041_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400042_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400043_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400044_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{676.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024400045_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{774.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601353_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{706.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601354_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601355_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601356_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601357_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601358_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{150.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601359_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{788.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1184.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601360_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{989.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601361_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{987.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601362_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1177.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601363_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601364_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601365_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{88.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000055_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000056_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000057_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{739.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{670.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000058_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000059_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1214.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895000060_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901151_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901152_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{674.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901153_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1173.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2279.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901154_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1112.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901155_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1078.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898301257_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898301258_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{714.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898301259_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{725.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898301260_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1607.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500847_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500848_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{94.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500849_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{62.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500850_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2862.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{177.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500851_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2868.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{198.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500852_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2908.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{307.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100523_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100524_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100525_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{188.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309000703_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100704_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3179.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700631_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{214.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{200.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700632_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{227.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700633_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1109.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700634_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{586.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700635_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700636_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{687.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{938.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700637_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{161.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700638_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{269.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700639_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{85.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{649.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100523_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100524_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100525_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891100527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000697_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000698_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000699_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000700_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000701_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000702_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000703_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000704_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153300638_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2883.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{48.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153300639_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3013.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1477.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500697_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500698_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500699_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568500700_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600701_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600702_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600703_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600704_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200988_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200989_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200990_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200991_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200992_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200993_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392200994_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400523_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400524_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400525_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595400528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{643.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601226_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{47.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601227_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601228_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2866.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601229_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2868.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{61.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601230_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2905.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{77.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601231_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2901.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{481.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601232_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3707.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{181.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300847_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{200.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300848_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{676.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300849_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{368.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300850_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{617.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300851_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{169.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300852_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401051_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401052_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1123.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401053_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401054_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2479.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401055_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2314.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891401056_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2869.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901694_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901695_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901696_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1921.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{292.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901697_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{196.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901698_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{134.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901699_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2878.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{191.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901700_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2934.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{457.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901701_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3038.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{122.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901702_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{76.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901703_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{144.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968540901704_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{259.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134900702_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{76.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134900703_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2914.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{60.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134900704_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2970.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700524_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2203.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700525_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{118.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701051_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701052_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701053_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701054_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701055_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701056_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701057_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032701058_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801059_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801060_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801061_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801062_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801063_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801064_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801065_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201132_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201133_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201134_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201135_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201136_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201137_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201138_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{67.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201139_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{42.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201140_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201141_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201142_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201143_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{67.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201144_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{97.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902101415_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902101416_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{89.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902101417_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{114.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902201418_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2881.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1165.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902201419_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{141.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902201420_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{709.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928800964_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1760.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928900965_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928900966_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928900967_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928900968_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897601053_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2458.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897601054_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2870.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{339.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897601055_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{99.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897601056_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1020.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_ReachabilityMarkingComparison.tex <==

\section{Executions Reported for ReachabilityMarkingComparison  (``Known'' models)}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300271_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300272_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300273_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{365.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{66.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300274_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1508.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300275_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1746.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300276_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2170.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2327.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100206_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{312.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100207_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500271_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{884.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1406.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500272_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500273_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500274_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500275_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500276_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400542_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400543_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400544_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400545_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400546_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400547_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{76.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400548_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400549_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400550_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{215.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400551_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{500.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547400552_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138201406_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138201407_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{797.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138201408_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2593.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{150.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905400455_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905400456_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905400457_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1705.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{281.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905400458_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{122.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905500459_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{412.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905500460_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901502109_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901502110_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{397.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901502111_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1889.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{94.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901502112_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700067_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700068_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{243.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{113.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700069_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1334.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700070_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1141.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700071_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{944.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700072_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{926.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200183_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200184_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2874.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{261.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300053_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300054_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{504.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400078_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400079_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400080_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400081_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400082_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400083_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400084_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800316_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900317_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{151.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{55.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900318_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900319_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900320_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900321_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{150.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900322_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200067_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200068_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1094.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200069_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1229.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200070_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2280.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200071_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2121.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200072_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2636.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500271_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{604.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{137.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500273_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{848.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500274_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{790.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500275_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1860.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500276_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1059.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530100134_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530100135_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530200136_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{330.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530200137_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{433.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530200138_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{124.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530200139_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{189.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530200140_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{563.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530200141_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{174.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530200142_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2877.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{239.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530200143_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2901.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{545.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530200144_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2954.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2479.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132100182_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132100183_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{266.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132100184_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{457.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897400115_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897400116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{407.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897400117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897400118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897400119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1705.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897400120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3128.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1020.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900249_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900250_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900251_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900252_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2169.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900253_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2526.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895000273_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895000274_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895000275_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{868.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895000276_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{658.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300271_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300272_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{243.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{104.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300273_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1367.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300274_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1199.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300275_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{965.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300276_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{958.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400319_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400320_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2868.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{234.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500206_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500207_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{496.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800316_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800317_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800318_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800319_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800320_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800321_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800322_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500554_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500555_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{151.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{54.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500556_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500557_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500558_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500559_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{149.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500560_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700271_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700272_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1052.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700273_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1281.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700274_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2193.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700275_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1941.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700276_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2634.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200475_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200476_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{604.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{134.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200477_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{841.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200478_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{779.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1854.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1047.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700542_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700543_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700544_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{326.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700545_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{435.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700546_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{135.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700547_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{189.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700548_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{502.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700549_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{189.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700550_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2873.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{283.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700551_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2900.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{539.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532700552_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2954.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132900318_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132900319_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{254.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132900320_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{457.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898500455_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898500456_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{407.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898500457_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898500458_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2577.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898500459_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1787.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898500460_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3130.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{991.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925800436_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925800437_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925800438_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925900439_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2158.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925900440_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2536.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895700477_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895700478_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895700479_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{865.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895700480_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{654.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000475_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000476_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{342.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000477_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2314.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000478_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000479_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{623.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000480_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{320.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600455_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600456_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{246.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800359_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800360_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{770.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300554_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300555_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300556_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300557_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300558_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300559_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300560_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{267.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200793_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200794_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200795_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200796_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{317.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200797_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{415.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{52.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200798_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300475_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300476_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300477_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300478_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300479_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300480_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900679_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900680_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{84.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900681_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900682_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{305.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900683_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{321.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900684_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{363.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700950_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700951_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700952_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{708.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700953_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1280.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700954_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{339.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700955_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{312.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700956_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700957_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{341.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700958_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2877.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{508.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700959_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2900.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2601.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535700960_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{979.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133600454_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133600455_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{265.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133600456_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{607.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899700795_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899700796_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899700797_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1521.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899700798_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1284.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899700799_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1269.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899700800_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3129.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{986.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927100623_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927100624_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927100625_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2826.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927100626_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{852.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927100627_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1080.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896300681_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{272.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896300682_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896400683_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{341.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896400684_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{744.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800679_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800680_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800681_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800682_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{105.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800683_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800684_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308800591_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308800592_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2874.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{234.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000512_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{116.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000513_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{517.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{337.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800792_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800793_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800794_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800795_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800796_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800797_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800798_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901030_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901031_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{85.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{259.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901032_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1750.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901033_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1409.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901034_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{750.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901035_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{458.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874901036_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{384.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800679_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800680_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800681_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800682_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{334.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800683_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{428.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800684_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600883_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600884_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890700885_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1409.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890700886_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2090.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890700887_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890700888_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538601358_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538601359_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538601360_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{677.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538601361_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1004.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538601362_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{995.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538601363_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{312.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538701364_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538701365_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538701366_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538701367_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{210.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538701368_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134400590_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134400591_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1579.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134400592_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{411.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901201135_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901201136_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1747.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901201137_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901201138_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901201139_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1061.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901201140_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3130.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{985.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927900810_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927900811_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927900812_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{210.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927900813_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{234.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927900814_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{152.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897000885_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897000886_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{70.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897000887_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897000888_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{611.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600067_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600068_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600069_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600070_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600071_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600072_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300863_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300864_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1333.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{155.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800053_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{55.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800054_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1015.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600078_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600079_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600080_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{759.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{65.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600081_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{844.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600082_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{831.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600083_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{798.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600084_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{864.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601506_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601507_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{800.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601508_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{800.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601509_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{949.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601510_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1151.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601511_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1180.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601512_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1195.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100067_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{684.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{85.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100068_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100069_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100070_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1314.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100071_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1290.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100072_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1294.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401291_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401292_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{838.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{46.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401293_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{744.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401294_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501295_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{771.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501296_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{811.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000134_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000135_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000136_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000137_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000138_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{681.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000139_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{735.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000140_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{68.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000141_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1737.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000142_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1213.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000143_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1289.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525000144_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135600862_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135600863_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135600864_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{772.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200115_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200116_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200117_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200118_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{825.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200119_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1205.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895200120_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930001184_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930001185_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930001186_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1123.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1385.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930001187_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1106.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930001188_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1070.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898401293_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898401294_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898401295_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{702.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898401296_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1154.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600883_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600884_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1131.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600885_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2383.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600886_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2843.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600887_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{730.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600888_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100727_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1048.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100728_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{621.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153400665_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{644.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153400666_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301030_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301031_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301032_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301033_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301034_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301035_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{818.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701268_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701269_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701270_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701271_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701272_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{264.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{593.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701273_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875701274_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{178.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{606.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400883_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400884_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400885_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400886_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400887_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400888_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601087_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2369.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601088_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1694.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601089_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601090_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601091_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601092_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2882.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2356.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541401766_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541401767_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541401768_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541401769_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541401770_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2862.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2213.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541401771_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541401772_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541401773_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{74.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541501774_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541501775_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541501776_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{146.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135000726_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1479.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135000727_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{245.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135000728_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{144.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301475_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301476_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301477_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301478_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301479_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{99.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902301480_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{323.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929100997_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929100998_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1542.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929100999_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929101000_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929101001_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{812.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897701089_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897701090_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{600.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897701091_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2972.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{327.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897701092_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_ReachabilityMix.tex <==

\section{Executions Reported for ReachabilityMix  (``Known'' models)}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300283_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300284_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{393.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{27.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300285_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{652.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300286_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1508.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300287_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1579.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1650.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854300288_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2170.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2445.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301409_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301410_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301411_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301412_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{478.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{406.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301413_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{728.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{911.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301414_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1649.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{439.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301415_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1396.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435301416_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{457.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100215_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{342.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154100216_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301409_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401410_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401411_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{393.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{168.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401412_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{546.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1044.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401413_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1512.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{541.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401414_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1358.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{514.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401415_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1809.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2192.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571401416_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001057_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001058_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{371.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{206.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001059_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{676.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001060_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001061_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{562.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001062_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{621.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500283_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{890.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500284_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500285_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500286_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500287_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892500288_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600566_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600567_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600568_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600569_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1386.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600570_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1642.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{260.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600571_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1684.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{240.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600572_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600573_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{128.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600574_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600575_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547600576_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138301414_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1086.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{701.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138301415_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2056.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1350.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138301416_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2593.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{149.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905500475_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905500476_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{170.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905500477_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1707.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{281.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905600478_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{131.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905600479_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{408.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905600480_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901602121_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901602122_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1778.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901602123_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1888.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{87.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901602124_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{its-tools}}
\index{Execution!ITS-Tools!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{its-tools} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!CSRepetitions (colored)}
\subsubsection{Report for CSRepetitions (colored)}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849200277_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849200278_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849200279_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2792.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{474.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849200280_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2822.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{522.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849200281_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{867.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849200282_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2776.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{549.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!DotAndBoxes (colored)}
\subsubsection{Report for DotAndBoxes (colored)}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101273_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101274_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101275_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101276_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{744.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!DrinkVendingMachine (colored)}
\subsubsection{Report for DrinkVendingMachine (colored)}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101277_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101278_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400955_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400956_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400957_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400958_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400959_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400960_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435001278_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!LamportFastMutEx (colored)}
\subsubsection{Report for LamportFastMutEx (colored)}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390000323_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390000324_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390000325_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1339.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{403.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390000326_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1808.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{728.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390000327_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{615.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390000328_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2828.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{544.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390000329_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2829.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{567.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!NeoElection (colored)}
\subsubsection{Report for NeoElection (colored)}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878902227_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878902228_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PermAdmissibility (colored)}
\subsubsection{Report for PermAdmissibility (colored)}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888700277_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888700278_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2424.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{453.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888700279_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2639.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{498.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888700280_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2730.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{592.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888700281_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2426.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{503.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888700282_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2686.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{619.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Peterson (colored)}
\subsubsection{Report for Peterson (colored)}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895201909_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895201910_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{442.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895201911_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2802.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{360.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895201912_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{425.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895201913_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{426.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895201914_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2836.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{436.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SimpleLoadBal (colored)}
\subsubsection{Report for SimpleLoadBal (colored)}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933401751_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933401752_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933401753_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{648.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{65.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933401754_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{453.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933401755_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2826.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{435.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700079_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700080_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{260.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{331.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700081_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{432.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800082_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1825.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800083_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{995.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849800084_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{832.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100139_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100140_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100141_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1536.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100142_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117100143_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1682.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200191_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200192_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{238.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700055_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{98.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700056_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{117.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700057_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{411.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700058_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{146.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700059_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{97.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700060_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{504.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700061_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{173.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700062_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2841.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854700063_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000139_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000140_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000141_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2715.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000142_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1954.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000143_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000144_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200185_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200186_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200187_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200188_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2838.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{276.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200189_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{426.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200190_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{817.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200191_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{636.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433200192_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300062_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300063_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{510.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800185_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800186_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800187_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{546.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800188_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{397.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800189_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{883.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800190_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800191_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800192_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{370.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400092_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400093_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400094_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400095_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400096_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400097_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390400098_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600139_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{152.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600140_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600141_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{182.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600142_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600143_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593600144_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900330_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900331_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{172.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900332_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2972.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2473.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900333_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1300.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900334_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3230.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900335_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1486.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872900336_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2355.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200079_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200080_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1197.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200081_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200082_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{445.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200083_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200084_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500283_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500284_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{568.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{49.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888500285_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{445.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600287_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{757.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888600288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300158_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300159_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300160_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{396.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300161_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300162_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{141.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300163_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300164_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{109.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300165_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300166_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3713.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{882.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300167_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1387.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968530300168_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1020.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132100190_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132200191_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{232.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132200192_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{448.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700140_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700141_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{196.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{69.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700142_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1090.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700143_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217700144_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1603.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400091_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400092_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400093_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400094_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400095_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400096_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{933.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1011.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400097_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{296.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400098_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{560.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400099_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{247.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400100_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400101_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027400102_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500103_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500104_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027500105_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{108.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600300_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600301_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600302_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600303_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600305_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600306_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600307_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{79.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{39.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600308_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600309_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600310_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600311_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600312_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500135_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500136_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{395.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500137_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{957.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500138_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500139_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{903.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{384.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897500140_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2876.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1016.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900260_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900261_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900262_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900263_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2503.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924900264_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1245.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895100285_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895100286_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895100287_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{865.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895100288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400283_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400284_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{260.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{328.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400285_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{444.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400286_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1882.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400287_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1022.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850400288_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{852.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600241_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600242_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600243_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1536.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600244_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600245_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1686.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117600246_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{258.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400327_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400328_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2876.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{248.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200208_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{83.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200209_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{111.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200210_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{391.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200211_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{140.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200212_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{92.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200213_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{482.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200214_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{169.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200215_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2843.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{48.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855200216_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300241_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300242_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300243_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2738.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300244_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1903.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300245_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300246_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400321_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400322_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400323_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{258.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400324_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2838.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{253.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400325_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{380.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400326_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{787.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400327_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{638.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400328_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500215_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500216_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300321_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300322_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300323_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{524.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300324_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{355.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300325_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{806.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300326_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300327_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567300328_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{392.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800330_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800331_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800332_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800333_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800334_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800335_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800336_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100241_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{157.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100242_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100243_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{190.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100244_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100245_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594100246_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{42.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500568_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500569_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{172.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500570_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2972.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2446.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500571_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1295.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500572_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3231.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873500573_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1483.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873600574_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2345.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800283_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800284_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1283.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800285_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800286_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{460.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800287_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889800288_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200487_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889200488_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{568.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{54.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300489_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300490_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{437.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300491_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{786.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889300492_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532800566_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532800567_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532800568_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{347.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532800569_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532900570_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{173.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532900571_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532900572_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532900573_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{71.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532900574_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3710.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{920.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532900575_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1383.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532900576_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1022.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132900326_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132900327_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{245.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132900328_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{448.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900242_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900243_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{195.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{76.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900244_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1060.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900245_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900246_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1611.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600346_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600347_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600348_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600349_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600350_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600351_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{933.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1139.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600352_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{304.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600353_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{576.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600354_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{266.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600355_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600356_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600357_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600358_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028600359_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028700360_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{121.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000521_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000522_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000523_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000524_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000525_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000529_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000530_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000531_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000532_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000533_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898600475_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898600476_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{395.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898600477_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{897.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898600478_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898600479_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{903.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{351.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898600480_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2877.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{987.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925900447_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925900448_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925900449_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925900450_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2479.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925900451_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1242.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895800489_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895800490_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895800491_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{871.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989895800492_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000487_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000488_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{363.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{92.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000489_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{947.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000490_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000491_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{784.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851000492_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{309.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200343_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200345_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1518.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2099.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200346_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200347_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1688.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118200348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{525.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600463_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{285.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600464_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2874.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{234.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700361_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700362_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700363_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700364_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700365_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700366_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700367_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700368_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855700369_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600343_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600345_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600346_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600347_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{286.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{287.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600457_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{271.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600458_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600459_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600460_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{71.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600461_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{997.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600462_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1119.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600463_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{604.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600464_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800368_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{314.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152800369_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{777.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700457_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700458_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700459_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{576.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700460_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{401.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700461_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{957.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800462_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800463_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567800464_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{368.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300568_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300569_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300570_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300571_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300572_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300573_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391300574_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500343_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{445.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{41.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600345_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{157.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600346_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600347_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594600348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2840.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{41.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300806_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300807_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300808_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{422.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300809_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300810_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1422.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300811_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{537.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874300812_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{328.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300487_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300488_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300489_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300490_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300491_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890300492_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900691_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900692_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900693_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{241.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889900694_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{311.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000695_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{331.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890000696_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900974_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900975_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900976_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{335.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900977_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900978_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{747.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900979_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900980_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{376.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900981_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2309.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900982_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900983_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1383.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535900984_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1051.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133700462_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133700463_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{234.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133700464_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{543.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200344_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200345_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{33.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200346_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2239.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200347_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2132.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200348_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100601_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100602_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100603_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100604_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100605_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100606_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{333.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{351.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100607_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{330.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100608_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100609_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100610_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100611_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100612_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100613_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100614_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978030100615_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{215.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400742_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{265.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400743_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{281.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400744_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400745_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{264.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400746_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{280.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400747_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400748_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400749_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{42.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400750_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{270.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400751_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{278.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400752_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400753_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625400754_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{358.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899800815_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899800816_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{307.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{19.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899800817_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2338.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899800818_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{365.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899800819_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{903.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{344.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899800820_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2884.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{981.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927100634_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{247.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927100635_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927100636_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{278.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927100637_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{991.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927100638_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{567.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896400693_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896400694_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896400695_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{357.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989896400696_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800691_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800692_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851800693_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{165.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{578.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900694_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{92.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900695_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851900696_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700445_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700446_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2242.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700447_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{116.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700448_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118700449_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941741100450_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{379.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308900600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2875.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{245.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200514_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1653.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200515_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200516_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1445.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200517_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200518_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200519_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200520_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2178.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200521_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856200522_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2087.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900445_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900446_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900447_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900448_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900449_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900450_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800593_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800594_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800595_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800596_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800597_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000521_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000522_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{838.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{378.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200593_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200594_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200595_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200596_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200597_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568200600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800806_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800807_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800808_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800809_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800810_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800811_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800812_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100445_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100446_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100447_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{686.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100448_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100449_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{957.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595100450_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{950.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001044_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001045_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{85.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{165.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001046_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1853.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001047_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1409.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001048_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1578.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001049_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{472.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875001050_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{382.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800691_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800692_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800693_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{246.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800694_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{336.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800695_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890800696_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{671.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890700895_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890700896_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890700897_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890700898_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1832.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890700899_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890700900_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801382_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801383_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801384_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{638.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801385_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801386_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{903.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801387_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801388_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{111.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801389_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{65.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801390_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{942.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801391_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1379.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538801392_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1040.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134400598_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134500599_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1093.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134500600_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{405.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500446_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500447_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500448_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1019.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500449_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{255.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218500450_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{95.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031600856_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031600857_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031600858_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031600859_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031600860_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031600861_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{113.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700862_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{200.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{307.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700863_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1204.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700864_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1636.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700865_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700866_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700867_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700868_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700869_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031700870_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800963_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{172.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{231.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800964_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800965_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800966_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800967_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800968_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{67.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800969_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1234.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800970_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800971_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800972_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800973_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800974_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{90.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800975_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2138.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901201155_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901201156_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901301157_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901301158_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{53.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901301159_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{903.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{344.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901301160_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2880.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{982.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927900821_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927900822_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927900823_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927900824_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{278.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928000825_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{75.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897100897_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897100898_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897100899_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{131.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897100900_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600079_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600080_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1186.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{127.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600081_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600082_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600083_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848600084_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800649_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800650_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800651_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800652_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800653_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{751.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119800654_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{927.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300871_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300872_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1716.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{365.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700055_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{922.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700056_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1099.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700057_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700058_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700059_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{870.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700060_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1100.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700061_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700062_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{942.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853700063_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1110.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500649_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{661.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500650_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500651_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500652_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500653_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500654_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{699.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200865_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200866_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300867_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300868_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{673.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300869_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{864.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300870_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2443.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1606.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300871_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2363.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434300872_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1993.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800062_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800063_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1015.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100865_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100866_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100867_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100868_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{816.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100869_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1821.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{69.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100870_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100871_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569100872_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600092_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600093_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600094_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{425.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600095_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{853.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600096_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{825.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600097_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{798.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600098_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{864.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800649_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800650_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800651_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800652_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1397.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800653_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800654_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2009.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876601520_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701521_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{800.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701522_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701523_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{950.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701524_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1152.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701525_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876701526_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1195.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100079_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{683.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{84.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100080_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{805.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100081_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{804.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200082_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1315.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200083_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1290.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888200084_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1294.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2446.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501303_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{672.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501304_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1161.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{138.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501305_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{743.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501306_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501307_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{771.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892501308_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525100158_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525100159_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525100160_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525100161_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{707.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525100162_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{747.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525100163_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1155.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525200164_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1169.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525200165_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525200166_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1213.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525200167_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1290.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968525200168_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135700870_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135700871_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135700872_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{772.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000650_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000651_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{717.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000652_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{724.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000653_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000654_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700091_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700092_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700093_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700094_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700095_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700096_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700097_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700098_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{674.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700099_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{714.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700100_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700101_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700102_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700103_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700104_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{672.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024700105_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{738.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701405_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{678.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701406_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701407_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701408_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701409_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701410_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{62.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701411_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{787.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{628.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701412_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{989.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701413_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701414_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1177.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701415_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{32.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701416_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{39.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626701417_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{88.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895300135_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895300136_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895300137_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{749.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{386.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895300138_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895300139_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1199.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895300140_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930101195_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930101196_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930101197_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1434.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930101198_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1106.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930101199_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1077.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898401305_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898401306_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{714.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898401307_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{725.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898401308_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1607.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600895_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600896_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600897_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600898_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600899_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852600900_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{62.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300547_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300548_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300549_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300550_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300551_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119300552_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{188.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100735_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100736_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1451.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800667_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800668_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800669_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800670_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800671_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800672_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800673_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800674_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856800675_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200547_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200548_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200549_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200550_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200551_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200552_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000729_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000730_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000731_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000732_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000733_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000734_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000735_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000736_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153400674_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2871.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153400675_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3016.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600729_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600730_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600731_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700732_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700733_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700734_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700735_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568700736_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301044_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301045_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301046_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301047_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301048_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301049_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392401050_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500547_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500548_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500549_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500550_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500551_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500552_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801282_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801283_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801284_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{166.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801285_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{78.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801286_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1150.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{711.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801287_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{96.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875801288_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400895_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400896_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400897_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{91.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400898_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400899_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891400900_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601099_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2150.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601100_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601101_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601102_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891601103_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891701104_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{89.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601790_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601791_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601792_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601793_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601794_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{92.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601795_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601796_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2937.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{232.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601797_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2951.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{42.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601798_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{936.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{643.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601799_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1402.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541601800_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135000734_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135000735_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135100736_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{600.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700548_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700549_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700550_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700551_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700552_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033001111_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033001112_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033001113_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033001114_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101115_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101121_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101122_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101123_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101124_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{593.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033101125_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301184_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301185_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301186_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301187_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301188_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301189_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301190_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301191_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301192_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301193_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301194_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301195_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626301196_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902401495_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902401496_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902401497_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902401498_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2866.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{71.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902401499_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902401500_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{336.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{202.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929201008_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929201009_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929201010_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929201011_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929201012_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897801101_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2394.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897801102_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2874.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{750.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897801103_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{92.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989897801104_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1015.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_ReachabilityPlaceComparison.tex <==

\section{Executions Reported for ReachabilityPlaceComparison  (``Known'' models)}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200247_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200248_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{566.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{76.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200249_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{483.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{208.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200250_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1508.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200251_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1579.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1653.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854200252_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2170.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2277.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201385_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201386_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201387_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201388_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{463.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201389_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{766.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201390_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1356.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{399.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201391_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1397.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201392_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{461.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154000188_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{321.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154000189_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201385_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201386_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301387_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{168.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301388_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{549.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301389_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1306.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301390_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1358.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{526.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301391_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1809.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2203.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571301392_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001039_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001040_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{431.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{155.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001041_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1193.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001042_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001043_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{562.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956597001044_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{621.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400247_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{889.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400248_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400249_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400250_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400251_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892400252_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547000494_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547100495_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547100496_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{55.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547100497_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{844.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{348.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547100498_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{376.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{27.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547100499_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{638.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{66.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547100500_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547100501_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547100502_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{224.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547100503_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{502.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968547100504_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138101390_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1120.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{567.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138101391_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2059.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1321.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138101392_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2593.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{157.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905200415_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905200416_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905200417_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1705.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{308.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905300418_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905300419_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{412.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983905300420_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{its-tools}}
\index{Execution!ITS-Tools!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{its-tools} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!CSRepetitions (colored)}
\subsubsection{Report for CSRepetitions (colored)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100242_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100243_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2792.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{478.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100244_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2821.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{523.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100245_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{823.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849100246_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2776.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{454.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!DotAndBoxes (colored)}
\subsubsection{Report for DotAndBoxes (colored)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001249_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001250_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001251_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001252_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{729.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!DrinkVendingMachine (colored)}
\subsubsection{Report for DrinkVendingMachine (colored)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101253_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310101254_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400937_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400938_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400939_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400940_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400941_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892400942_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435001254_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!GlobalRessAlloc (colored)}
\subsubsection{Report for GlobalRessAlloc (colored)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000181_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000182_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{190.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000183_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/06 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1196.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{222.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000184_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2774.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{512.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000185_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/09 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2777.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{521.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000186_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2311.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{525.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000187_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/11 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2791.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{588.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!LamportFastMutEx (colored)}
\subsubsection{Report for LamportFastMutEx (colored)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900281_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900282_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900283_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1339.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{307.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900284_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1808.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{554.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900285_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{632.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900286_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2829.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{540.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900287_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2829.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{573.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!NeoElection (colored)}
\subsubsection{Report for NeoElection (colored)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802185_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802186_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{78.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{318.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802187_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1411.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{330.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802188_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{415.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802189_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{441.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802190_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2843.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{487.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878802191_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{593.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PermAdmissibility (colored)}
\subsubsection{Report for PermAdmissibility (colored)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600241_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600242_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2423.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{500.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600243_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2639.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{496.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600244_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2730.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{597.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600245_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2426.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{582.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888600246_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2686.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{614.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Peterson (colored)}
\subsubsection{Report for Peterson (colored)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101873_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101874_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{443.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101875_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2802.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{351.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101876_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{431.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101877_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{418.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966895101878_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2836.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{428.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SharedMemory (colored)}
\subsubsection{Report for SharedMemory (colored)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100401_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100402_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100403_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100404_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100405_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100406_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100407_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000500 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100408_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/001000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100409_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/002000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100410_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/005000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100411_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/010000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100412_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/020000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100413_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/050000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100414_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/100000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100415_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100416_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100417_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100418_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100419_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896100420_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SimpleLoadBal (colored)}
\subsubsection{Report for SimpleLoadBal (colored)}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933201718_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933201719_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933201720_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{648.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933201721_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{448.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933201722_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2824.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{405.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849600043_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700044_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{253.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{372.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700045_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1642.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700046_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1806.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700047_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1961.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849700048_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1234.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000121_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000122_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000123_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{892.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000124_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117000125_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200167_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308200168_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2875.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{251.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600028_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{106.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600029_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600030_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600031_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{200.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600032_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{232.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600033_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{842.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600034_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600035_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{142.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854600036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{159.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889900121_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000122_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000123_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000124_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000125_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890000126_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100161_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100162_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100163_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100164_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1030.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100165_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1178.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100166_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{231.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100167_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433100168_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{109.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300035_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152300036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{487.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700161_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700162_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{228.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700163_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{628.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566700164_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{995.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800165_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800166_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800167_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1230.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566800168_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{224.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300050_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300051_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300052_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300053_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300054_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300055_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390300056_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500121_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{474.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{196.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500122_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{272.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500123_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{285.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500124_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{467.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500125_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{89.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593500126_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{164.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800288_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800289_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{183.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{84.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800290_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1511.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800291_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800292_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800293_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872800294_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2569.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100043_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100044_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1396.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100045_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{191.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889100046_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{845.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200047_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{419.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889200048_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400247_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400248_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{567.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{50.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400249_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1138.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400250_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{439.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400251_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{180.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966888400252_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1106.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529800086_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529800087_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529800088_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{817.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529800089_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{68.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529800090_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{417.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529900091_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{193.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529900092_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{221.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529900093_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{290.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529900094_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{348.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529900095_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2933.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{832.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968529900096_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2986.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132000166_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132000167_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{177.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132000168_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{462.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600122_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600123_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600124_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1659.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600125_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217600126_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1663.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200046_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200047_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200048_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200049_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200050_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200051_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1483.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1896.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200052_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{915.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200053_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{552.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200054_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{269.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200055_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200056_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200057_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200058_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200059_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1710.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978027200060_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{192.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624500261_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{327.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600262_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600263_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600264_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600265_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600266_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600267_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600268_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600269_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600270_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600271_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600272_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624600273_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300075_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300076_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{411.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{242.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300077_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1195.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300078_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300079_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983897300080_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2846.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1008.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800227_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800228_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800229_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800230_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2288.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983924800231_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2024.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300247_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300248_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{253.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{391.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300249_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1684.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300250_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1835.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300251_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1989.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850300252_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1259.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500223_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500224_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{54.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500225_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{892.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500226_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500227_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932117500228_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400303_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308400304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2875.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{235.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100181_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{107.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100182_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100183_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100184_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{188.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100185_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{212.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100186_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{785.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100187_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100188_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2843.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{131.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855100189_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{151.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890200223_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300224_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300225_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300226_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300227_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890300228_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300297_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433300298_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400299_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400300_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1012.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400301_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1110.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400302_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{211.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400303_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433400304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{97.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500188_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152500189_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{476.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200297_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200298_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{228.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200299_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{641.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200300_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{942.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200301_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200302_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200303_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1169.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567200304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{196.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700288_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700289_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700290_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700291_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390700292_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800293_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955390800294_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000223_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{474.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{202.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000224_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{283.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000225_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{291.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000226_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{467.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000227_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{84.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594000228_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{161.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400526_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400527_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{93.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400528_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1400.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400529_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400530_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400531_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2873.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959873400532_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2571.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700247_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700248_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1416.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700249_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{200.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700250_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{863.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700251_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{407.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959889700252_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100451_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100452_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{568.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{55.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100453_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1156.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100454_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{430.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100455_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{187.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889100456_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1139.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400494_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400495_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400496_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{805.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400497_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2843.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{60.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400498_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{340.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400499_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{173.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400500_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{270.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400501_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{264.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400502_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2872.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{271.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400503_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2936.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{762.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968532400504_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2987.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132800302_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132800303_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{164.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972132800304_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{463.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900224_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900225_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{57.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900226_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1653.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900227_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217900228_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1667.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400301_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400302_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400303_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400304_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400305_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400306_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1483.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2123.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400307_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{843.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400308_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{514.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400309_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{290.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400310_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400311_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400312_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400313_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400314_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1701.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978028400315_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{176.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900482_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{305.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900483_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900484_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900485_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900486_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900487_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900488_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900489_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{80.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624900490_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000491_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000492_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000493_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625000494_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898400415_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898400416_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{411.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{241.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898400417_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1151.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898400418_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898400419_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983898400420_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1004.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925700414_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925700415_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925700416_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925700417_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2305.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983925700418_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2024.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900451_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900452_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{366.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{103.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900453_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900454_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2811.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900455_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{429.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933850900456_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{742.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100325_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100326_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100327_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{697.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100328_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100329_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118100330_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1300.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600439_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{286.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308600440_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2875.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{245.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600334_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600335_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600336_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600337_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600338_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600339_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600340_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600341_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941855600342_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{303.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600325_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600326_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{284.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600327_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600328_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600329_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890600330_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600433_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{281.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600434_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600435_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600436_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{920.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600437_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600438_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1674.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600439_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{265.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433600440_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{185.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700341_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152700342_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{753.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700433_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700434_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700435_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{761.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700436_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1206.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700437_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{279.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700438_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{278.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700439_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{974.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950567700440_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{176.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200526_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200527_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200528_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200529_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200530_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200531_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391200532_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500325_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{539.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{54.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500326_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{140.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500327_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{169.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500328_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{317.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500329_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{93.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956594500330_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{176.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200764_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200765_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{306.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{85.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200766_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200767_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200768_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{321.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200769_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{402.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874200770_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{333.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200451_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200452_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200453_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200454_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200455_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890200456_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800655_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800656_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{38.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800657_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800658_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800659_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{321.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966889800660_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{347.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300902_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{288.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300903_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300904_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{945.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300905_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{310.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300906_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1293.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300907_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1563.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300908_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300909_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2866.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{543.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300910_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2874.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300911_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2933.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968535300912_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{934.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133500438_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133500439_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{177.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972133500440_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{546.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200326_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200327_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{363.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200328_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200329_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2647.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218200330_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{988.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029700556_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800557_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800558_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800559_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800560_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800561_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{338.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{591.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800562_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{322.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800563_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{360.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800564_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{302.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800565_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800566_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800567_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800568_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800569_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{485.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978029800570_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300703_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{493.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300704_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{280.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300705_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{256.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300706_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300707_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300708_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300709_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300710_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300711_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{296.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300712_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300713_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{304.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300714_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{315.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625300715_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{358.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899600755_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899600756_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{312.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{126.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899600757_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1481.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899600758_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1530.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899600759_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1163.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983899600760_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2847.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1002.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926900601_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926900602_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926900603_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926900604_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{913.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983926900605_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{687.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700655_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700656_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700657_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{501.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700658_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{96.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700659_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933851700660_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600427_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600428_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600429_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{116.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932118600431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{83.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941741000432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{379.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308800575_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937308800576_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2875.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{232.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100487_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1677.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100488_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100489_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100490_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100491_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100492_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100493_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100494_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856100495_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1996.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900427_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900428_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900429_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941890900432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800569_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800570_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800571_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800572_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800573_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800574_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800575_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946433800576_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000494_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{115.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153000495_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{474.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{356.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100569_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100570_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100571_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100572_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100573_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100574_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100575_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568100576_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700764_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391700765_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800766_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800767_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800768_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800769_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955391800770_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000427_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000428_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000429_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{81.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{663.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{587.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{933.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595000432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{912.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874801002_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874801003_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{87.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{287.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874801004_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1753.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874801005_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{995.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874801006_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{802.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874801007_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{467.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959874801008_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{383.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700655_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700656_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{255.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700657_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{255.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700658_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{337.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700659_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{417.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959890700660_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500859_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890500860_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600861_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1415.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600862_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2381.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600863_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966890600864_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538301310_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538301311_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538301312_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{655.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538401313_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538401314_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{895.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538401315_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{246.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538401316_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538401317_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{75.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538401318_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{108.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538401319_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{247.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968538401320_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{337.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134300574_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134300575_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{933.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134300576_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{415.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400428_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400429_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400430_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1023.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400431_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{262.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218400432_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{95.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400811_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400812_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400813_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400814_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400815_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400816_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{149.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400817_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{200.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{647.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400818_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1209.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400819_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1708.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400820_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400821_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400822_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400823_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400824_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978031400825_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800924_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2365.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800925_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800926_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800927_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800928_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800929_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{86.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800930_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{331.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800931_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{330.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800932_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800933_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800934_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800935_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{421.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980625800936_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{94.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1422.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901001095_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901001096_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901001097_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901001098_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{119.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901001099_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{932.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983901001100_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2844.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{977.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927700788_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927700789_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927700790_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{210.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927700791_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{280.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983927700792_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{152.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500043_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500044_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{24.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500045_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500046_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500047_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848500048_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1141.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700631_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700632_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700633_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700634_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700635_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{751.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119700636_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{927.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300847_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300848_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1331.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{170.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600028_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{931.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600029_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1099.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600030_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600031_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600032_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{870.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600033_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1100.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600034_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600035_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{940.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853600036_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500631_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{661.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500632_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{661.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500633_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500634_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500635_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891500636_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200841_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200842_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200843_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200844_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{673.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200845_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{861.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200846_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2405.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1477.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200847_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2345.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200848_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1993.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800035_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{39.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800036_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1016.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000841_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000842_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000843_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000844_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{750.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000845_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1819.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{65.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000846_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000847_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000848_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600050_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600051_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600052_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{759.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{96.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600053_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{843.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600054_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{825.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600055_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{796.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389600056_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{843.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700631_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700632_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700633_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{680.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800634_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{845.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800635_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595800636_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2009.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501478_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501479_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501480_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501481_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{950.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501482_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1151.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501483_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1172.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876501484_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1195.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000043_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{683.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{104.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000044_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{803.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000045_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{790.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000046_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1284.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100047_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1278.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888100048_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1294.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2623.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301267_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892301268_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{838.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401269_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{744.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401270_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401271_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{771.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892401272_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700086_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700087_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700088_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700089_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700090_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{681.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700091_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{735.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700092_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{68.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700093_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1185.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1344.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700094_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1213.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700095_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1291.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524700096_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135500846_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135600847_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135600848_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{772.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000632_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000633_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{716.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000634_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{724.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000635_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219000636_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500046_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500047_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500048_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500049_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500050_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500051_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500052_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500053_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{674.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500054_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500055_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500056_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500057_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500058_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500059_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024500060_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{715.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601366_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{671.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601367_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601368_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601369_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601370_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601371_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{704.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{51.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601372_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{787.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{646.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601373_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{989.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601374_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601375_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1178.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{27.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601376_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601377_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{46.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601378_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{91.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895100075_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895100076_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895100077_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{688.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895100078_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895100079_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1199.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895100080_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901162_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901163_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901164_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1123.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1356.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901165_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1112.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929901166_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1077.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500859_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500860_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500861_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500862_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500863_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933852500864_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{523.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100529_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119100530_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119200531_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119200532_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119200533_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119200534_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100711_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309100712_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700640_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700641_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700642_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700643_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700644_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700645_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700646_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700647_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941856700648_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200529_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200530_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200531_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200532_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200533_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891200534_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000705_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000706_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000707_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000708_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000709_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000710_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000711_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434000712_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153300647_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952153300648_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600705_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600706_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600707_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600708_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600709_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600710_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600711_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568600712_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301002_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301003_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301004_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301005_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301006_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301007_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392301008_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500529_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500530_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500531_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500532_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500533_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595500534_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601240_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601241_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601242_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601243_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{52.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601244_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601245_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959875601246_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{102.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300859_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300860_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300861_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300862_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300863_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959891300864_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501063_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501064_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501065_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501066_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501067_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966891501068_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541001718_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541101719_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541101720_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541101721_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541101722_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541101723_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541101724_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2138.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{201.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541101725_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{211.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541101726_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541101727_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{115.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968541101728_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{191.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134900710_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134900711_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972134900712_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700530_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700531_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700532_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700533_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218700534_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801066_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801067_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801068_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801069_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801070_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801071_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801072_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801073_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801074_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801075_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801076_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032801077_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901078_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901079_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978032901080_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201145_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201146_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201147_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201148_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201149_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201150_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201151_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201152_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201153_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201154_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201155_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201156_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626201157_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902201435_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902201436_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902201437_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902201438_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902201439_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{527.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983902201440_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928900975_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928900976_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928900977_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928900978_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983928900979_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_known_StateSpace.tex <==

\section{Executions Reported for StateSpace  (``Known'' models)}
\subsection{Relevant Executions for \acs{alpina}}
\index{Execution!alpina!StateSpace}

This section reports here some information about the relevant execution of
\acs{alpina} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!CSRepetitions (colored)}
\subsubsection{Report for CSRepetitions (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600205_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{512.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600206_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1006.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{75.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600207_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2477.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600208_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2492.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600209_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{528.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600210_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{762.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600211_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{519.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600212_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1006.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{71.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600213_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2480.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600214_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2488.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600215_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{534.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933855600216_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{765.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600817_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120600818_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120700819_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2512.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120700820_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1063.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{41.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120700821_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1939.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{953.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120700822_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{889.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!DotAndBoxes (colored)}
\subsubsection{Report for DotAndBoxes (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309701089_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{513.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309801090_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{536.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309801091_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{536.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309801092_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{563.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!DrinkVendingMachine (colored)}
\subsubsection{Report for DrinkVendingMachine (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309801093_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{683.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309801094_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1733.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309801095_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{692.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309801096_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1731.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858700154_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{852.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858700155_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{820.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858700156_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{816.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{28.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858700157_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1036.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{80.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858700158_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858700159_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{818.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858700160_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1080.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{191.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858700161_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{831.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858700162_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1100.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{244.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000817_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{477.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000818_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{500.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000819_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{623.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000820_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000821_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1212.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892000822_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{542.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701089_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{608.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701090_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1608.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701091_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2510.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701092_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2522.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701093_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2510.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701094_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2517.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701095_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2521.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434701096_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!GlobalRessAlloc (colored)}
\subsubsection{Report for GlobalRessAlloc (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154600154_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2485.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154600155_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154600156_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/06 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154600157_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154600158_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/09 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2512.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154600159_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2508.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154600160_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/11 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2512.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154600161_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2490.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154600162_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570001089_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1139.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570001090_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2500.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2531.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570001091_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2510.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570001092_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2525.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570001093_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2535.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570001094_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2510.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570001095_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2533.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570001096_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2510.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!LamportFastMutEx (colored)}
\subsubsection{Report for LamportFastMutEx (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000239_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000240_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{802.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000241_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2506.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000242_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1719.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000243_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2512.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000244_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2505.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000245_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2512.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000246_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{528.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000247_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{804.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000248_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2505.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000249_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1839.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000250_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000251_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2509.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955394000252_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2512.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300817_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300818_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2510.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300819_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2510.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300820_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300821_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596300822_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2512.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!NeoElection (colored)}
\subsubsection{Report for NeoElection (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901905_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{791.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{18.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901906_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2379.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{607.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877901907_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{839.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001908_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{847.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001909_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{895.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001910_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{886.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001911_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{865.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001912_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{790.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001913_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2380.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{606.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001914_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{840.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001915_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{845.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001916_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{893.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001917_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{884.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878001918_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{860.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PermAdmissibility (colored)}
\subsubsection{Report for PermAdmissibility (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893300205_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1550.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{39.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893300206_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2508.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893300207_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893300208_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893300209_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893400210_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893400211_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1551.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{47.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893400212_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893400213_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2508.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893400214_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893400215_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2508.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959893400216_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2508.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Peterson (colored)}
\subsubsection{Report for Peterson (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901633_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{810.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901634_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2509.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1563.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901635_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2509.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901636_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{547.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901637_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{606.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893901638_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{660.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894001639_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{810.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894001640_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2509.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1593.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894001641_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2509.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894001642_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{535.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894001643_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{606.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894001644_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{677.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Philosophers (colored)}
\subsubsection{Report for Philosophers (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300409_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{474.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300410_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{476.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300411_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{499.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300412_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{757.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300413_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{782.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300414_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{793.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300415_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{586.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300416_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{444.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300417_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{442.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300418_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{333.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300419_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300420_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/050000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{341.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552300421_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/100000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{339.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400422_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400423_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{476.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400424_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{493.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400425_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{755.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400426_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{782.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400427_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{791.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{33.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400428_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{598.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400429_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{443.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400430_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{441.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400431_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{334.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968552400432_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{332.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PhilosophersDyn (colored)}
\subsubsection{Report for PhilosophersDyn (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136801089_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{516.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136801090_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{841.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136801091_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1116.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136801092_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/50 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1412.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136801093_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/80 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1053.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136801094_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{506.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136801095_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{840.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136801096_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1141.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Planning (P/T)}
\subsubsection{Report for Planning (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500817_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Planning/ (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{217.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500818_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{872.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500819_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500820_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2514.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500821_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1032.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219500822_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1880.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{770.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200256_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{474.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200257_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{473.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200258_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{483.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200259_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{604.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200260_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200261_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200262_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200263_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200264_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{837.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200265_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{484.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200266_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{851.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200267_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200268_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200269_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978037200270_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501769_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501770_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{845.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501771_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{883.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501772_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1294.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501773_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2381.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501774_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1112.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501775_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1116.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{53.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501776_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1405.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{227.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501777_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2512.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501778_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501779_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1065.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501780_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1069.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{67.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627501781_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1381.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{280.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SharedMemory (colored)}
\subsubsection{Report for SharedMemory (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907800341_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{479.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907800342_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{580.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907800343_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{751.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900344_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{810.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{60.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900345_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{865.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1059.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900346_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{933.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900347_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000500 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{775.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900348_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/001000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{446.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900349_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/002000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{439.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900350_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/005000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{335.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900351_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/010000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{333.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900352_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/020000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{329.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900353_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/050000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{343.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900354_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/100000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{350.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900355_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{477.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900356_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{571.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900357_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{753.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900358_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{811.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{40.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900359_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{862.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1027.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983907900360_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{934.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SimpleLoadBal (colored)}
\subsubsection{Report for SimpleLoadBal (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901498_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{492.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901499_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{535.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901500_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{637.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901501_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{765.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901502_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{786.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983931901503_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{496.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983932001504_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{523.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983932001505_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{625.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983932001506_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{765.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983932001507_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{787.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!TokenRing (colored)}
\subsubsection{Report for TokenRing (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501634_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{487.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501635_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{547.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501636_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{793.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501637_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1090.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{93.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501638_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/100 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2501.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2303.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501639_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/200 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{947.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899501640_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/500 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{788.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899601641_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899601642_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{518.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899601643_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{795.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989899601644_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1090.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{113.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{greatspn}}
\index{Execution!greatSPN!StateSpace}

This section reports here some information about the relevant execution of
\acs{greatspn} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854000211_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100212_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100213_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{365.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{61.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100214_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1388.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100215_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1582.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1840.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854100216_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2166.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2505.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201361_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201362_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201363_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201364_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201365_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{111.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201366_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{362.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{104.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201367_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435201368_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{427.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154000161_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{311.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154000162_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571101361_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571101362_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571101363_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571101364_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{98.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201365_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{444.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201366_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1358.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{512.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201367_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1808.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2208.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950571201368_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{240.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901021_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901022_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901023_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{235.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901024_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{527.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901025_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{563.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596901026_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{602.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300211_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{209.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300212_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300213_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300214_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300215_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892300216_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546500422_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546500423_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546500424_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546600425_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546600426_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{59.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546600427_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{74.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546600428_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1176.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546600429_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{131.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546600430_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{226.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546600431_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{502.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968546600432_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138001366_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138001367_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{798.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972138001368_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2594.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{139.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904900355_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904900356_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904900357_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1707.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{328.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904900358_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904900359_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{410.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983904900360_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901302049_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901302050_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{397.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901302051_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1889.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{99.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!greatSPN}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989901302052_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{greatspn}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{its-tools}}
\index{Execution!ITS-Tools!StateSpace}

This section reports here some information about the relevant execution of
\acs{its-tools} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!CSRepetitions (colored)}
\subsubsection{Report for CSRepetitions (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000205_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000206_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000207_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2792.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{482.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000208_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2821.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{529.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000209_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2845.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{869.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000210_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2776.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{477.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000211_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000212_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000213_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{54.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000214_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{122.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000215_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1985.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{477.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933849000216_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{510.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941741800919_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941741800920_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{469.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941741800921_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{353.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941741900922_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{362.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941741900923_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{475.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941741900924_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2871.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1969.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!DotAndBoxes (colored)}
\subsubsection{Report for DotAndBoxes (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001225_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001226_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001227_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001228_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DotAndBoxes/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2857.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{770.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!DrinkVendingMachine (colored)}
\subsubsection{Report for DrinkVendingMachine (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001229_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001230_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001231_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937310001232_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{506.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854000154_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{429.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854000155_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{434.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854000156_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{463.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854000157_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{451.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854000158_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{423.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854000159_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{445.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854000160_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2862.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{487.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854000161_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{446.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941854000162_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{464.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892300919_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892300920_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892300921_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892300922_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892300923_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941892300924_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{58.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434901225_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434901226_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434901227_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434901228_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434901229_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434901230_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435001231_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{120.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{253.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946435001232_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{539.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!GlobalRessAlloc (colored)}
\subsubsection{Report for GlobalRessAlloc (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000154_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000155_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{190.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000156_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/06 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1196.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{225.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000157_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/07 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2775.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{481.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000158_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/09 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2778.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{501.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000159_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2771.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{609.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000160_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/11 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2791.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{596.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000161_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{99.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952152000162_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570601225_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570601226_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570601227_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570601228_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{111.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570601229_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{331.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{110.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570601230_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1805.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2568.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570601231_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1470.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950570601232_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{660.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!LamportFastMutEx (colored)}
\subsubsection{Report for LamportFastMutEx (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389800239_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389800240_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389800241_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1339.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{386.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389800242_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1807.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{716.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389800243_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{542.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389800244_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2828.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{635.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389800245_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2829.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{511.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389800246_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389800247_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389800248_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900249_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{331.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900250_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{686.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900251_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2859.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{582.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389900252_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{768.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596600919_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596600920_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596600921_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{100.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596600922_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{632.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{128.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596600923_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1542.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596600924_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1589.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!NeoElection (colored)}
\subsubsection{Report for NeoElection (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702143_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702144_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702145_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1410.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{316.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702146_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{431.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702147_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{451.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702148_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2843.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{504.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702149_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2849.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{582.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702150_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702151_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702152_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1061.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{132.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702153_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2903.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{522.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702154_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2907.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1289.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702155_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{366.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959878702156_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{457.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PermAdmissibility (colored)}
\subsubsection{Report for PermAdmissibility (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500205_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{66.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500206_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2421.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{449.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500207_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2639.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{555.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500208_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2731.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{670.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500209_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2426.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{501.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500210_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2686.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{613.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500211_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{203.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500212_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{528.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500213_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{539.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500214_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{511.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500215_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{553.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888500216_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{594.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Peterson (colored)}
\subsubsection{Report for Peterson (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901837_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901838_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{442.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901839_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2802.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{353.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901840_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2856.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{417.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901841_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2858.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{419.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901842_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2836.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{420.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901843_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901844_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901845_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{156.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901846_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2559.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{619.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901847_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{357.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966894901848_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2862.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{488.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Philosophers (colored)}
\subsubsection{Report for Philosophers (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526600409_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526600410_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526600411_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526600412_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526600413_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526600414_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526600415_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526600416_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700417_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700418_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700419_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700420_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/050000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700421_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/100000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700422_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700423_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700424_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700425_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700426_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700427_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700428_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700429_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700430_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526700431_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968526800432_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972137301230_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{73.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972137301231_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{264.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972137301232_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2924.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1523.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219800920_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219800921_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2245.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{413.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219800922_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{288.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219800923_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{337.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219800924_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{373.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500256_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500257_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500258_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500259_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500260_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500261_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500262_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500263_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500264_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500265_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500266_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025500267_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{132.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025600268_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{682.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025600269_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{465.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978025600270_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{607.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627901990_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627901991_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627901992_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627901993_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627901994_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{198.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627901995_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{592.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{80.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627901996_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1122.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{142.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627901997_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2350.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1850.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627901998_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2896.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{322.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627901999_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2895.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{341.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627902000_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2897.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{497.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627902001_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2899.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1309.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627902002_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{204.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SharedMemory (colored)}
\subsubsection{Report for SharedMemory (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900341_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900342_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900343_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900344_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900345_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900346_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900347_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000500 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900348_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/001000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900349_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/002000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900350_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/005000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900351_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/010000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900352_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/020000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900353_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/050000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900354_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/100000 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900355_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900356_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900357_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900358_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983895900359_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983896000360_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SimpleLoadBal (colored)}
\subsubsection{Report for SimpleLoadBal (colored)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933001685_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933001686_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933001687_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{647.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{56.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933001688_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2855.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{433.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933001689_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2825.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{409.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933101690_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983933101691_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989900301845_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{31.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989900301846_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!StateSpace}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848400007_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848400008_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{714.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848400009_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1166.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848400010_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1145.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848400011_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1135.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933848400012_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600613_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600614_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{685.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{700.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600617_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{754.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932119600618_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{927.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300823_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937309300824_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1332.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{119.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500001_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{919.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500002_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1094.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500003_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500004_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1134.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500005_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{869.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500006_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1093.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500007_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1140.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500008_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{940.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941853500009_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400613_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{661.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400614_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400617_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891400618_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{680.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200817_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200818_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200819_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200820_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{673.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200821_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{861.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200822_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2405.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1476.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200823_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2363.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434200824_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1993.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800008_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{696.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952151800009_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1016.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900817_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900818_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900819_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950568900820_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{750.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000821_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1819.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000822_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2548.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000823_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569000824_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2549.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500008_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500009_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500010_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{727.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{61.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500011_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{843.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500012_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{819.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500013_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{797.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955389500014_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{852.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700613_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700614_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{680.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{844.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700617_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956595700618_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2009.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301436_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876301437_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{749.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401438_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{801.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401439_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{949.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401440_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1150.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401441_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1170.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959876401442_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000007_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{682.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{42.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000008_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{790.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000009_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{790.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000010_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1284.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000011_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1278.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959888000012_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1287.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201231_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201232_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{814.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{40.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201233_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{744.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201234_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{722.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201235_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{771.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966892201236_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{815.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524100014_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524200015_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524200016_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524200017_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{667.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524200018_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{681.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524200019_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{735.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524200020_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1108.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{33.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524200021_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1184.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{209.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524200022_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1212.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1401.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524200023_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1287.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968524200024_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{355.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135400822_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{669.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135400823_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{708.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972135400824_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{772.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Planning (P/T)}
\subsubsection{Report for Planning (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900613_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Planning/ (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900614_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900615_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{712.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900616_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{724.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900617_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{693.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975218900618_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{709.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024200001_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024200002_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024200003_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024200004_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024200005_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024200006_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024200007_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024200008_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{672.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300009_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{698.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300010_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300011_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300012_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300013_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300014_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{670.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978024300015_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{715.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601327_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{671.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601328_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601329_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601330_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601331_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601332_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{703.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601333_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{787.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{574.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601334_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{989.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601335_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{983.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1976.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601336_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1177.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{36.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601337_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1183.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{35.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601338_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{42.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980626601339_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1228.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{98.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983894900015_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983894900016_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983894900017_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{688.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{31.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983894900018_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{824.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983894900019_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1199.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983894900020_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{475.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929801129_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929801130_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{666.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929801131_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1118.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1271.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929801132_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1105.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983929801133_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1072.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201233_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201234_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{685.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201235_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{702.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898201236_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1153.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!StateSpace}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853300007_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853300008_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{442.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{54.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933853300009_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2910.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{137.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120100715_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120100716_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{374.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120100717_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1759.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1268.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932120100718_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2910.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{277.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891700715_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{124.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891700716_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941891700717_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2899.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{124.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434400953_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434400954_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{308.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434400955_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2480.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{81.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946434400956_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2505.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{101.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569400953_n_40.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{203.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569400954_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2413.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{214.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950569400955_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2417.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{186.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392700008_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392700009_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{313.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392700010_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{465.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{93.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392700011_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2668.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{250.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392700012_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2949.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{267.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392700013_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1445.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955392700014_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1981.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596000715_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{540.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{48.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956596000716_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2470.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{113.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959877201674_n_41.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1624.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{181.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893001435_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{282.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893001436_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{909.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966893101437_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2246.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{216.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543600014_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543600015_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{166.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968543600016_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2703.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{85.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136100958_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{404.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972136100959_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2990.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{320.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219200716_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219200717_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{415.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{34.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975219200718_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2882.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{180.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033900001_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033900002_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{125.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033900003_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033900004_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033900005_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{170.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033900006_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2614.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{91.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033900007_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2901.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{101.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033900008_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{741.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033900009_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2224.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978033900010_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034000011_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{145.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034000012_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{162.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034000013_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1433.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{142.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034000014_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2909.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{154.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978034000015_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1364.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001549_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{163.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001550_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{198.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001551_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{336.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001552_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{678.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{54.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001553_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2942.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{399.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001554_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{308.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001555_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{326.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001556_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{211.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{20.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001557_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0100w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{890.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001558_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0500w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{266.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001559_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r1000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{309.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980627001560_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2812.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{300.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903200015_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{162.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903200016_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{432.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{99.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983903200017_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2570.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{510.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930801316_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{152.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930801317_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{273.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930801318_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2797.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{364.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930801319_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3020.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{542.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983930901320_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{284.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898901437_n_38.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{214.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989898901438_n_39.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1490.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{127.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{pnxdd}}
\index{Execution!pnxdd!StateSpace}

This section reports here some information about the relevant execution of
\acs{pnxdd} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!CSRepetitions (P/T)}
\subsubsection{Report for CSRepetitions (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854900007_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854900008_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{51.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854900009_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/04 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1201.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{261.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854900010_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1005.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854900011_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136933854900012_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{CSRepetitions/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2869.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Dekker (P/T)}
\subsubsection{Report for Dekker (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932116500001_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932116500002_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932116500003_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{57.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932116500005_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{182.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136932116500006_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Dekker/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{310.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!DrinkVendingMachine (P/T)}
\subsubsection{Report for DrinkVendingMachine (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937307900007_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136937307900008_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{DrinkVendingMachine/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{733.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Echo (P/T)}
\subsubsection{Report for Echo (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858200001_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r09 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1469.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858200002_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r11 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858200003_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2595.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858200004_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d02r19 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1779.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858200005_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1313.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858200006_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2869.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2049.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858200007_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d03r07 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858200008_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d04r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2868.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1374.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941858200009_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Echo/d05r03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2880.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Eratosthenes (P/T)}
\subsubsection{Report for Eratosthenes (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889600001_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889600002_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889600003_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889600004_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889600005_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136941889600006_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Eratosthenes/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{58.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!FMS (P/T)}
\subsubsection{Report for FMS (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946432900001_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946432900002_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946432900003_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946432900004_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946432900005_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{213.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{300.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946432900006_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{734.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946432900007_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{636.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136946432900008_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{FMS/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{102.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!GlobalRessAlloc (P/T)}
\subsubsection{Report for GlobalRessAlloc (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154300008_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{142.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1957.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136952154300009_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{GlobalRessAlloc/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{384.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Kanban (P/T)}
\subsubsection{Report for Kanban (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566200001_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566200002_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566200003_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{37.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566200004_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{440.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566200005_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{370.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566200006_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{155.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566200007_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{203.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136950566200008_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Kanban/1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{205.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!LamportFastMutEx (P/T)}
\subsubsection{Report for LamportFastMutEx (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393600008_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393600009_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393600010_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{143.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393600011_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/5 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1344.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{303.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393600012_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1688.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393600013_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1557.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136955393600014_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{LamportFastMutEx/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1924.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!MAPK (P/T)}
\subsubsection{Report for MAPK (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593000001_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/008 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593000002_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593000003_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/040 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{103.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{56.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593000004_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/080 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{470.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593000005_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/160 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{616.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136956593000006_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{MAPK/320 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{614.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!NeoElection (P/T)}
\subsubsection{Report for NeoElection (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872000008_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872000009_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{72.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{32.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872000010_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1719.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1919.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872000012_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/6 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{238.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872000013_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/7 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{253.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959872100014_n_37.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{NeoElection/8 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{252.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PermAdmissibility (P/T)}
\subsubsection{Report for PermAdmissibility (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892800007_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/01 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{133.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892800008_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892800009_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2865.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892800010_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1707.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892800011_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1612.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136959892800012_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PermAdmissibility/50 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2864.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1624.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Peterson (P/T)}
\subsubsection{Report for Peterson (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966887600007_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/2 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966887600008_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/3 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{163.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136966887600009_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Peterson/4 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2863.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{768.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Philosophers (P/T)}
\subsubsection{Report for Philosophers (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549500014_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549500015_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549500016_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549500017_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549500018_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549500019_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{48.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549500020_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/000500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{29.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549600021_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/001000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{86.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{171.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549600022_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/002000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{139.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{893.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549600023_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/005000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{186.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136968549600024_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Philosophers/010000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!PhilosophersDyn (P/T)}
\subsubsection{Report for PhilosophersDyn (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972131100006_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/03 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972131100007_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{504.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{433.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136972131100008_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{PhilosophersDyn/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{162.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Railroad (P/T)}
\subsubsection{Report for Railroad (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217400002_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217400003_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{861.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{59.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136975217400006_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Railroad/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{220.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!RessAllocation (P/T)}
\subsubsection{Report for RessAllocation (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036200001_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R002C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036200002_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300003_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C003 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300004_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300005_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300006_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C015 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300007_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300008_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300009_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R003C100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300010_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R005C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300011_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R010C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300012_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R015C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300013_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R020C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300014_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R050C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136978036300015_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RessAllocation/R100C002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Ring (P/T)}
\subsubsection{Report for Ring (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624200001_n_24.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Ring/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!RwMutex (P/T)}
\subsubsection{Report for RwMutex (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624200002_n_25.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624200003_n_26.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624200004_n_27.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624200005_n_28.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624200006_n_29.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w0500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{71.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{157.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624200007_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w1000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{271.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{705.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624200008_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0010w2000 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{121.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624200009_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r0020w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{795.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{64.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136980624200013_n_36.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{RwMutex/r2000w0010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{128.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SharedMemory (P/T)}
\subsubsection{Report for SharedMemory (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906600015_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906600016_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906600017_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{389.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906600018_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2876.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906600019_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{93.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983906600020_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SharedMemory/000200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{257.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!SimpleLoadBal (P/T)}
\subsubsection{Report for SimpleLoadBal (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983923500007_n_30.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983923500008_n_31.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/05 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{53.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983923500009_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1762.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{267.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983923500010_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/15 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2866.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{707.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136983923500011_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{SimpleLoadBal/20 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2871.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1047.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!TokenRing (P/T)}
\subsubsection{Report for TokenRing (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894200009_n_32.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894200010_n_33.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{50.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894200011_n_34.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{327.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1390.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_136989894200012_n_35.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{TokenRing/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{644.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_CTLCardinalityComparison.tex <==

\section{Executions Reported for CTLCardinalityComparison  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400073_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400074_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400075_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400076_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400077_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400078_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400079_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400080_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900145_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{250.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900153_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900154_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900155_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900156_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900157_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900158_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900159_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900160_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700209_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700210_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700211_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700212_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700213_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700214_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700215_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700216_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800417_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2848.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{256.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800425_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800426_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800427_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800428_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800429_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800430_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800431_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800432_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300345_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300346_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300347_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300348_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300349_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300350_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300351_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300352_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500689_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500697_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500698_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500699_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500700_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500701_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500702_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500703_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500704_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{288.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100481_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100482_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100483_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100484_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100485_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100486_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100487_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100488_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400961_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{27.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400969_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400970_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400971_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400972_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400973_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400974_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400975_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{185.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{47.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400976_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900073_n_42.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900074_n_43.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900075_n_44.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000076_n_45.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{105.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000077_n_46.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1429.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1232.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000078_n_47.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1675.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000079_n_48.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1427.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{722.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000080_n_49.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1713.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600145_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{706.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600153_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600154_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1082.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{100.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600155_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600156_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1091.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600157_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{252.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600158_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{366.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600159_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{254.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600160_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{730.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!CTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600617_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600618_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600619_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600620_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600621_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600622_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600623_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600624_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201233_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201241_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201242_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201243_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201244_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201245_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201246_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201247_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{185.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201248_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_CTLFireability.tex <==

\section{Executions Reported for CTLFireability  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!CTLFireability}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300057_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300058_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300059_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300060_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300061_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300062_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300063_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300064_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800113_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800121_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800122_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800123_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800124_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800125_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800126_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800127_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900128_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{428.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!CTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600193_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600194_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600195_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600196_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600197_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600198_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600199_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600200_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700385_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700393_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700394_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700395_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700396_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700397_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700398_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700399_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700400_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{405.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!CTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200329_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200330_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200331_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200332_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200333_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200334_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200335_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200336_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400657_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400665_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400666_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400667_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400668_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400669_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400670_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400671_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400672_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{639.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!CTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000465_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000466_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000467_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000468_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000469_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000470_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000471_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000472_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300929_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{153.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300937_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300938_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300939_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300940_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300941_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300942_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300943_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300944_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{101.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!CTLFireability}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900057_n_50.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900058_n_51.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{690.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900059_n_52.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1534.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{106.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900060_n_53.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2023.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900061_n_42.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1429.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1182.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900062_n_43.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1702.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900063_n_44.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1427.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{734.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900064_n_45.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1694.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500113_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1378.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500121_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500122_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1117.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{115.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500123_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500124_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1091.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500125_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1181.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{255.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500126_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{370.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500127_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1193.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{254.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500128_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{775.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{148.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!CTLFireability}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600601_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600602_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600603_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600604_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600605_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600606_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600607_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600608_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101201_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101209_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101210_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101211_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101212_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101213_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101214_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101215_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101216_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_CTLMarkingComparison.tex <==

\section{Executions Reported for CTLMarkingComparison  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000169_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000170_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000171_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000172_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000173_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000174_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000175_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800441_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800442_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800443_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800444_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800445_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800446_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800447_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500713_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500714_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500715_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600716_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600717_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600718_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600719_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416500985_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416500986_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416500987_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416500988_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416500989_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416500990_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416500991_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600169_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600170_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1082.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{94.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600171_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600172_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1091.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700173_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{249.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700174_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{342.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700175_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1193.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{254.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!CTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201257_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201258_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201259_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301260_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301261_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301262_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301263_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{199.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_CTLMix.tex <==

\section{Executions Reported for CTLMix  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!CTLMix}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400089_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400090_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400091_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400092_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400093_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400094_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400095_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400096_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000177_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000185_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000186_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000187_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000188_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000189_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000190_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000191_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{196.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000192_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!CTLMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700225_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700226_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700227_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700228_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700229_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700230_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700231_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700232_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900449_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900457_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900458_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900459_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900460_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.99 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900461_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900462_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900463_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{196.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900464_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!CTLMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400361_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400362_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400363_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400364_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400365_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400366_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400367_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400368_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600721_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{293.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600729_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600730_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600731_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600732_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600733_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600734_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600735_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{196.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600736_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!CTLMix}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200497_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200498_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200499_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200500_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200501_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200502_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200503_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200504_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416500993_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{23.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416501001_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416501002_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416501003_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416501004_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416501005_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416501006_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416501007_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{196.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416501008_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{114.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!CTLMix}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000089_n_46.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000090_n_47.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{674.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000091_n_48.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1348.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{57.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000092_n_49.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2458.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000093_n_50.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1429.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1130.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000094_n_51.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1782.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000095_n_52.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1427.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{740.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799000096_n_53.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1694.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700177_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700185_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700186_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1092.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{95.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700187_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700188_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1091.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700189_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{247.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700190_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{333.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700191_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{258.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412700192_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{730.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!CTLMix}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700633_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700634_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700635_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700636_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700637_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700638_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700639_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700640_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301265_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301273_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301274_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301275_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301276_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301277_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301278_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301279_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301280_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_CTLPlaceComparison.tex <==

\section{Executions Reported for CTLPlaceComparison  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300065_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300066_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300067_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300068_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300069_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400070_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400071_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400072_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900129_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{226.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900137_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900138_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900139_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900140_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900141_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900142_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900143_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413900144_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600201_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600202_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600203_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600204_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600205_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700206_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700207_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700208_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700401_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{199.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700409_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700410_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700411_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700412_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700413_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700414_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700415_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414800416_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300337_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300338_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300339_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300340_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300341_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300342_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300343_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801300344_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400673_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500681_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500682_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500683_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500684_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500685_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500686_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500687_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415500688_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000473_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000474_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100475_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100476_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100477_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100478_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100479_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802100480_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300945_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{26.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400953_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400954_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400955_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400956_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400957_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400958_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400959_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416400960_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{113.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900065_n_46.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900066_n_47.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900067_n_48.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900068_n_49.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{130.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900069_n_50.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1429.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1085.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900070_n_51.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1644.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900071_n_52.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1427.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{748.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798900072_n_53.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1741.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500129_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{517.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600137_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600138_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1082.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{91.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600139_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600140_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1091.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600141_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{251.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600142_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{348.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600143_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{254.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412600144_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{730.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{73.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!CTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!CTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600609_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600610_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600611_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600612_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600613_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600614_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600615_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600616_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201217_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201225_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201226_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201227_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201228_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201229_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201230_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201231_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!CTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!CTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417201232_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_LTLCardinalityComparison.tex <==

\section{Executions Reported for LTLCardinalityComparison  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400113_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400114_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400115_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500116_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500117_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500118_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500119_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500120_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100225_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200233_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200234_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200235_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200236_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200237_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200238_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{183.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200239_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{46.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200240_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800249_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800250_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800251_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800252_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800253_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800254_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800255_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800256_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000497_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000505_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000506_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000507_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000508_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000509_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000510_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{183.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000511_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{45.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000512_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500385_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500386_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500387_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600388_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600389_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600390_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600391_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600392_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800769_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800777_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800778_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800779_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800780_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800781_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800782_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{183.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800783_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800784_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300521_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300522_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300523_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300524_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300525_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300526_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300527_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300528_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601041_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701049_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701050_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701051_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701052_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701053_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701054_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{183.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{32.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701055_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{44.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701056_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400113_n_82.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400114_n_83.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400115_n_84.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400116_n_85.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400117_n_86.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400118_n_87.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400119_n_88.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{138.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400120_n_89.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{140.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100225_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{645.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{82.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100233_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{203.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100234_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{490.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{56.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100235_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1116.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{297.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100236_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2953.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{519.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100237_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2923.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{633.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100238_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2985.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{745.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418200239_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3045.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{844.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLCardinalityComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418200240_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2486.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{385.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!LTLCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700657_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700658_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700659_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700660_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700661_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700662_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700663_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700664_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401313_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401321_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401322_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401323_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401324_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{49.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401325_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{129.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401326_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{183.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{30.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401327_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{184.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401328_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_LTLFireability.tex <==

\section{Executions Reported for LTLFireability  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!LTLFireability}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400097_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400098_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400099_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400100_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400101_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400102_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400103_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400104_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000193_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000201_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414000202_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100203_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100204_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100205_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100206_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100207_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100208_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!LTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700233_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700234_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700235_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700236_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700237_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700238_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800700239_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800240_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900465_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900473_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900474_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900475_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900476_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900477_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900478_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900479_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900480_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!LTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400369_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400370_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801400371_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500372_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500373_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500374_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500375_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500376_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415600737_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700745_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700746_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700747_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700748_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700749_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700750_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700751_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700752_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!LTLFireability}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200505_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200506_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200507_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200508_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200509_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200510_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200511_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200512_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416501009_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601017_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601018_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601019_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601020_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601021_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601022_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601023_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601024_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!LTLFireability}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803300097_n_78.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803300098_n_79.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803300099_n_80.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803300100_n_81.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803300101_n_82.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803300102_n_83.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400103_n_84.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400104_n_85.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{140.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418000193_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{646.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{88.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418000201_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{202.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418000202_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{489.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{62.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418000203_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1118.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{280.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418000204_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2951.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{514.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418000205_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2925.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{646.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418000206_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2986.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{737.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418000207_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3044.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{847.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLFireability!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418000208_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2487.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{438.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!LTLFireability}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700641_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700642_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700643_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700644_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700645_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700646_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700647_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700648_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301281_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301289_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301290_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301291_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301292_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301293_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301294_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301295_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301296_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_LTLMarkingComparison.tex <==

\section{Executions Reported for LTLMarkingComparison  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200249_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200250_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200251_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200252_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200253_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200254_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200255_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100521_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100522_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100523_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100524_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100525_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100526_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100527_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900793_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900794_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900795_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900796_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900797_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900798_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900799_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701065_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701066_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701067_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701068_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701069_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701070_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701071_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418200249_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{202.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418200250_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{489.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{64.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418200251_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1116.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{293.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418200252_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2954.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{533.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418200253_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2925.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{625.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418200254_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2986.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{740.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418200255_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3045.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{791.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!LTLMarkingComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401337_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401338_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401339_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401340_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501341_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501342_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501343_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_LTLMix.tex <==

\section{Executions Reported for LTLMix  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!LTLMix}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500129_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500130_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500131_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500132_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500133_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500134_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500135_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500136_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414200257_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414300265_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414300266_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414300267_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414300268_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414300269_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414300270_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414300271_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414300272_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!LTLMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800900265_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800900266_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800900267_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800900268_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800900269_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800900270_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800900271_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800900272_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100529_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100537_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100538_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100539_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100540_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100541_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100542_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100543_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415100544_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!LTLMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600401_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600402_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600403_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600404_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600405_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801600406_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801700407_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801700408_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.04 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900801_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900809_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900810_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900811_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900812_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{60.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900813_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900814_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900815_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415900816_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!LTLMix}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802400537_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802400538_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802400539_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802400540_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802400541_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802400542_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802400543_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802400544_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416701073_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416801081_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416801082_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416801083_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416801084_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416801085_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416801086_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416801087_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416801088_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!LTLMix}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803500129_n_86.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803500130_n_87.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803500131_n_88.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803500132_n_89.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803500133_n_78.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803500134_n_79.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803500135_n_80.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803500136_n_81.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{140.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418200257_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{646.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{86.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418300265_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{202.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418300266_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{489.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{52.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418300267_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1118.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{266.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418300268_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2956.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{498.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418300269_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2925.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{631.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418300270_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2986.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{749.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418300271_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3045.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{790.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLMix!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418300272_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2486.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{379.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!LTLMix}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700673_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700674_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700675_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802800676_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802800677_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802800678_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802800679_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802800680_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501345_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501353_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501354_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501355_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501356_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{61.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501357_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501358_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{123.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{16.15 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501359_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417501360_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_LTLPlaceComparison.tex <==

\section{Executions Reported for LTLPlaceComparison  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400105_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400106_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400107_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400108_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400109_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400110_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400111_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800400112_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100209_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100217_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100218_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100219_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100220_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100221_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100222_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100223_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414100224_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800241_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800242_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800243_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800244_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800245_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800246_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800247_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800800248_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414900481_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000489_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000490_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000491_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000492_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000493_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000494_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000495_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415000496_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500377_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500378_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500379_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500380_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500381_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500382_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500383_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801500384_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700753_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700761_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700762_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700763_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700764_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415700765_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800766_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800767_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415800768_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200513_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802200514_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300515_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300516_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300517_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300518_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300519_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802300520_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601025_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601033_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601034_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{32.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601035_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601036_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601037_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601038_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601039_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416601040_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400105_n_86.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400106_n_87.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400107_n_88.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400108_n_89.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400109_n_78.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400110_n_79.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400111_n_80.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110803400112_n_81.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{140.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418000209_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{645.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{87.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100217_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{202.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100218_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{490.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{56.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100219_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1118.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{293.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100220_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2951.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{522.02 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100221_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2924.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{655.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100222_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2986.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{740.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100223_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3046.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{845.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLPlaceComparison!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107418100224_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2486.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{395.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!LTLPlaceComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!LTLPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700649_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700650_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700651_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700652_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700653_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700654_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700655_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802700656_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417301297_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401305_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401306_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401307_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401308_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401309_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401310_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401311_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!LTLPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!LTLPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417401312_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_ReachabilityCardinalityComparison.tex <==

\section{Executions Reported for ReachabilityCardinalityComparison  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200033_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200034_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200035_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200036_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200037_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200038_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200039_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200040_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700065_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700073_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700074_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700075_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{47.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700076_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{64.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700077_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{110.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700078_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{221.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700079_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{594.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{222.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700080_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600169_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600170_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600171_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600172_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600173_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600174_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600175_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600176_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500337_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500345_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500346_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500347_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500348_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600349_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{107.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600350_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{43.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600351_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{591.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{219.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600352_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100305_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100306_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100307_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100308_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100309_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100310_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100311_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100312_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300609_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.43 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300617_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300618_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300619_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.64 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300620_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300621_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{106.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300622_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{42.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300623_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{591.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{219.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300624_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{295.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801900441_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801900442_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801900443_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801900444_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801900445_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801900446_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801900447_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801900448_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100881_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{25.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100889_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200890_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200891_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.15 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200892_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{63.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200893_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{107.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.77 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200894_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{219.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{41.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200895_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{592.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{216.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200896_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{118.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700033_n_50.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700034_n_51.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700035_n_52.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700036_n_53.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{149.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700037_n_42.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1429.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1212.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700038_n_43.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1706.90 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700039_n_44.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1427.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{773.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798800040_n_45.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1684.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400065_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1359.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400073_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.18 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400074_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1082.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{87.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400075_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400076_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1079.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400077_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{286.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400078_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1192.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{317.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400079_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1194.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{271.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400080_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{730.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{86.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityCardinalityComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityCardinalityComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500577_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500578_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500579_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500580_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500581_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500582_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500583_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500584_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001153_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001161_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001162_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001163_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001164_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001165_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{106.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001166_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{215.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{40.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001167_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{588.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{212.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityCardinalityComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityCardinalityComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001168_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_ReachabilityDeadlock.tex <==

\section{Executions Reported for ReachabilityDeadlock  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{cunf}}
\index{Execution!cunf!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{cunf} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityDeadlock!cunf}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107421100569_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{cunf}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100009_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100010_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100011_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100012_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100013_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100014_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100015_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100016_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600017_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600025_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600026_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600027_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600028_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600029_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600030_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600031_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityDeadlock!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600032_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{524.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500145_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500146_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500147_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500148_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500149_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500150_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500151_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500152_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414400289_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414400297_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414400298_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414400299_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414400300_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414400301_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414400302_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414400303_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414400304_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{526.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000281_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{217.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000282_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{209.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000283_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{211.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000284_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{211.27 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000285_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{210.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000286_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{207.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000287_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{186.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000288_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{210.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200561_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{298.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200569_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{270.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200570_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{269.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200571_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{301.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200572_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{294.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200573_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{289.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200574_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{307.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200575_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{299.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityDeadlock!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200576_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2854.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{973.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801700417_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801700418_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801700419_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801700420_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801700421_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801700422_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800423_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800424_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000833_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000841_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000842_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000843_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000844_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000845_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000846_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000847_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{46.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityDeadlock!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000848_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{117.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600009_n_50.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600010_n_51.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.06 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600011_n_52.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600012_n_53.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{120.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600013_n_42.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1429.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1137.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600014_n_43.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1807.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600015_n_44.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1427.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{743.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600016_n_45.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1684.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300017_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{628.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300025_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.29 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300026_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1082.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{105.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300027_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300028_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1077.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300029_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1181.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{304.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300030_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{365.84 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300031_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1190.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{278.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityDeadlock!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300032_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{729.98 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{97.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityDeadlock}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityDeadlock!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802400553_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500554_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500555_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500556_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500557_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500558_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500559_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500560_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901105_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901113_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901114_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901115_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{30.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901116_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901117_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901118_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901119_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityDeadlock!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityDeadlock!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901120_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_ReachabilityFireability.tex <==

\section{Executions Reported for ReachabilityFireability  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100017_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100018_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800100019_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200020_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200021_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200022_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200023_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200024_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600033_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600041_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413600042_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700043_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.72 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700044_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.19 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700045_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700046_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700047_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityFireability!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700048_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1127.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500153_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500154_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500155_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500156_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500157_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500158_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500159_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500160_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414400305_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500313_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500314_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500315_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500316_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500317_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500318_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500319_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500320_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1093.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000289_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000290_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000291_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000292_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000293_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801000294_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100295_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100296_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.74 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200577_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200585_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200586_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200587_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415200588_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300589_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300590_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300591_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityFireability!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300592_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2111.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800425_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800426_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800427_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800428_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800429_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800430_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800431_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800432_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000849_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{105.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000857_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416000858_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100859_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100860_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100861_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.65 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100862_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100863_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityFireability!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100864_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{113.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600017_n_46.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600018_n_47.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700019_n_48.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{697.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700020_n_49.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2156.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{552.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700021_n_50.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1429.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1169.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700022_n_51.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1749.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700023_n_52.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1427.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{750.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700024_n_53.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1685.05 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300033_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400041_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400042_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1185.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{160.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400043_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400044_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1077.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400045_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1181.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{300.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400046_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{352.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400047_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{311.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityFireability!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400048_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{774.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{213.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityFireability}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityFireability!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500561_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500562_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500563_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500564_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500565_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500566_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500567_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500568_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901121_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901129_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901130_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901131_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901132_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901133_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901134_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901135_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityFireability!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityFireability!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416901136_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_ReachabilityMarkingComparison.tex <==

\section{Executions Reported for ReachabilityMarkingComparison  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800089_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800090_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800091_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800092_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800093_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800094_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800095_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{44.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600361_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600362_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600363_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600364_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600365_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.58 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600366_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600367_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300633_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300634_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400635_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400636_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400637_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400638_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400639_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200905_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200906_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200907_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200908_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200909_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200910_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200911_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{41.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.82 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500089_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500090_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1082.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{88.07 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500091_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500092_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1079.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500093_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1182.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{265.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500094_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1192.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{314.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500095_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1192.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{259.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityMarkingComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101177_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101178_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101179_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{56.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{3.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101180_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101181_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{104.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{22.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101182_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMarkingComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101183_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{62.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{4.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_ReachabilityMix.tex <==

\section{Executions Reported for ReachabilityMix  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300049_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300050_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300051_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300052_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300053_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300054_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300055_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800300056_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800097_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.48 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{626.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800105_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800106_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800107_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800108_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800109_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800110_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800111_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{46.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityMix!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413800112_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600185_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600186_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600187_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600188_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600189_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600190_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600191_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600192_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600369_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2850.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{572.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600377_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600378_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600379_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600380_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.07 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600381_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414600382_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.03 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700383_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{47.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityMix!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414700384_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200321_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200322_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200323_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200324_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200325_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200326_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200327_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801200328_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400641_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{300.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400649_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400650_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.44 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400651_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400652_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{68.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400653_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400654_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.02 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.97 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400655_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{47.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityMix!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415400656_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{297.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{7.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000457_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000458_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000459_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000460_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000461_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000462_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000463_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802000464_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416200913_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{218.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{106.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300921_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.35 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300922_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300923_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.57 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300924_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{69.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300925_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300926_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.98 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300927_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{189.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{46.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityMix!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416300928_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{335.76 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798800049_n_42.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.86 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798800050_n_43.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{665.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.27 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798800051_n_44.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.69 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798800052_n_45.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2109.31 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{348.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798800053_n_46.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1429.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1023.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798800054_n_47.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1758.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798800055_n_48.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1427.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{745.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798800056_n_49.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1675.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500097_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1241.16 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500105_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.28 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500106_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1086.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{92.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500107_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500108_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1077.68 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500109_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1181.55 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{271.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500110_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1193.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{346.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500111_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{254.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityMix!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412500112_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{761.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{111.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityMix}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityMix!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600593_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600594_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600595_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600596_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600597_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600598_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600599_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802600600_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101185_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.79 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101193_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101194_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.12 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101195_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101196_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{70.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101197_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.28 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101198_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101199_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{43.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityMix!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityMix!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417101200_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_ReachabilityPlaceComparison.tex <==

\section{Executions Reported for ReachabilityPlaceComparison  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{lola}}
\index{Execution!lola!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200025_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200026_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200027_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200028_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200029_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200030_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200031_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800200032_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700049_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700057_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.45 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.63 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700058_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700059_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700060_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.88 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700061_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{39.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.14 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700062_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.39 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700063_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107413700064_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2853.33 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1991.52 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic}}
\index{Execution!lola optimistic!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500161_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800500162_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.60 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600163_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600164_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600165_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600166_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600167_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110800600168_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500321_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500329_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500330_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.90 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.48 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500331_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500332_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.61 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500333_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.60 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500334_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500335_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.81 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107414500336_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2852.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1890.22 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-optimistic-incomplete}}
\index{Execution!lola optimistic incomplete!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-optimistic-incomplete} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100297_n_62.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100298_n_63.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100299_n_64.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100300_n_65.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100301_n_66.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100302_n_67.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100303_n_68.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.73 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801100304_n_69.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300593_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{291.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{6.79 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300601_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.22 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.40 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300602_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300603_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300604_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300605_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300606_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.91 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300607_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.94 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.05 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola optimistic incomplete}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107415300608_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-optimistic-incomplete}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2851.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{lola-pessimistic}}
\index{Execution!lola pessimistic!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{lola-pessimistic} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800433_n_54.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800434_n_55.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800435_n_56.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800436_n_57.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800437_n_58.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800438_n_59.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800439_n_60.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110801800440_n_61.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100865_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.47 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.53 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100873_n_7.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100874_n_8.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.58 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100875_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.89 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100876_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{36.14 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100877_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100878_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{38.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.81 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100879_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{42.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.74 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityPlaceComparison!lola pessimistic}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107416100880_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{lola-pessimistic}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{114.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700025_n_42.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700026_n_43.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.24 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700027_n_44.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.38 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700028_n_45.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{104.78 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700029_n_46.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1429.32 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1184.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700030_n_47.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1708.45 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700031_n_48.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1427.42 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{766.94 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798700032_n_49.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1675.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400049_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1344.71 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400057_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{664.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400058_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1082.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{77.18 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400059_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400060_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1079.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400061_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1181.56 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{302.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400062_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1191.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{342.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400063_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1193.36 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{282.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityPlaceComparison!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412400064_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{730.10 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{87.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{sara}}
\index{Execution!sara!ReachabilityPlaceComparison}

This section reports here some information about the relevant execution of
\acs{sara} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!ReachabilityPlaceComparison!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500569_n_70.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.01 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500570_n_71.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500571_n_72.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.12 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500572_n_73.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500573_n_74.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500574_n_75.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.80 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500575_n_76.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802500576_n_77.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001137_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{33.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001145_n_9.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.46 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.33 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001146_n_10.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.24 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001147_n_11.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{35.23 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.38 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001148_n_12.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.71 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.49 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001149_n_13.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001150_n_14.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{45.67 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001151_n_5.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{126.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.10 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!ReachabilityPlaceComparison!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!ReachabilityPlaceComparison!sara}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417001152_n_6.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{sara}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{34.35 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.29 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}


==> annexes/exec_report_surprise_StateSpace.tex <==

\section{Executions Reported for StateSpace  (``Surprise'' models)}
\subsection{Relevant Executions for \acs{alpina}}
\index{Execution!alpina!StateSpace}

This section reports here some information about the relevant execution of
\acs{alpina} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804800137_n_91.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{627.78 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.85 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804800138_n_92.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1296.55 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804800139_n_93.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2510.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804800140_n_94.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2510.53 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804800141_n_95.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804800142_n_96.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2514.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804800143_n_97.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2510.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804800144_n_98.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400273_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2511.64 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!QuasiCertifProtocol (colored)}
\subsubsection{Report for QuasiCertifProtocol (colored)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400274_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{494.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.09 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400275_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{499.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.80 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400276_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{529.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.26 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400277_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{635.09 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400278_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{765.92 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{9.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400279_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{668.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400280_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (colored)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{781.19 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{11.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400281_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{880.06 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.96 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400282_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2513.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400283_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2512.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400284_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{832.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{12.46 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400285_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{813.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{14.00 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400286_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{832.96 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{17.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400287_n_20.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{812.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{21.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!StateSpace!alpina}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107420400288_n_21.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{alpina}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{839.20 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{its-tools}}
\index{Execution!ITS-Tools!StateSpace}

This section reports here some information about the relevant execution of
\acs{its-tools} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799200137_n_46.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{37.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799200138_n_47.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{40.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799200139_n_48.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{130.52 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799200140_n_49.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1259.69 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{363.89 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799200141_n_50.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2861.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{624.67 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799300142_n_51.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2896.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{870.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799300143_n_52.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2860.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1516.70 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110799300144_n_53.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1454.65 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412900273_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{96.82 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2.51 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412900281_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{95.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412900282_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{209.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{15.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412900283_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2897.39 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{492.17 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412900284_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2896.93 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{559.03 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412900285_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2899.17 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{497.59 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412900286_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2898.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{571.47 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412900287_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2899.62 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{612.73 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!StateSpace!ITS-Tools}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412900288_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{its-tools}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2896.16 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{518.43 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{marcie}}
\index{Execution!marcie!StateSpace}

This section reports here some information about the relevant execution of
\acs{marcie} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600001_n_42.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{662.76 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600002_n_43.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{663.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600003_n_44.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{689.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600004_n_45.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1580.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{82.68 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600005_n_46.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1429.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1140.34 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600006_n_47.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1393.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1718.95 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600007_n_48.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1427.54 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{700.56 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110798600008_n_49.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1693.97 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300001_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1360.49 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{293.20 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300009_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{455.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.25 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300010_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{907.13 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{46.31 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300011_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1171.75 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300012_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1077.59 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300013_n_1.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1181.34 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{310.75 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300014_n_2.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1190.91 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{348.41 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300015_n_3.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1190.57 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{276.54 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!StateSpace!marcie}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107412300016_n_4.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{marcie}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{729.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{86.66 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{neco}}
\index{Execution!neco!StateSpace}

This section reports here some information about the relevant execution of
\acs{neco} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802900001_n_78.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{135.25 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.32 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802900002_n_79.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{156.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{10.36 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802900003_n_80.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2523.83 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{130.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802900004_n_81.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2501.44 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{108.21 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802900005_n_82.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2481.95 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{95.93 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802900006_n_83.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2498.21 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{111.62 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802900007_n_84.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{137.04 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.23 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110802900008_n_85.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{140.70 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{13.13 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417500001_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{646.84 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417500009_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{202.40 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{8.50 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417500010_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{491.08 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417500011_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1116.11 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417500012_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/18 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2951.63 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{519.08 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417600013_n_15.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/22 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2924.61 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{604.83 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417600014_n_16.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/28 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2985.51 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{700.30 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417600015_n_17.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/32 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{3045.87 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{844.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!StateSpace!neco}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107417600016_n_18.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{neco}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2486.72 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{499.01 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\subsection{Relevant Executions for \acs{pnxdd}}
\index{Execution!pnxdd!StateSpace}

This section reports here some information about the relevant execution of
\acs{pnxdd} (\emph{i.e.} the examination it participated).
We provide the execution status and a sampling of memory and CPU usage over the execution
(boot time is removed)

\index{Execution!StateSpace!HouseConstruction (P/T)}
\subsubsection{Report for HouseConstruction (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804300001_n_90.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/002 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{109.88 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.42 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804300002_n_91.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/005 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{109.99 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{0.92 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804300003_n_92.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/010 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{873.30 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2244.87 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804300004_n_93.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/020 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2882.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804300005_n_94.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/050 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2205.37 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804300006_n_95.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/100 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2883.66 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804300007_n_96.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/200 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1737.50 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137110804300008_n_97.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{HouseConstruction/500 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2373.26 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!IBMB2S565S3960 (P/T)}
\subsubsection{Report for IBMB2S565S3960 (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107419400001_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{IBMB2S565S3960/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2885.85 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{2104.11 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!QuasiCertifProtocol (P/T)}
\subsubsection{Report for QuasiCertifProtocol (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107419400009_n_22.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/02 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{114.41 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{1.37 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107419400010_n_23.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/06 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{136.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{5.86 s} & \\
      {End status: } & normal & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107419400011_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{QuasiCertifProtocol/10 (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{1568.00 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}
\index{Execution!StateSpace!Vasy2003 (P/T)}
\subsubsection{Report for Vasy2003 (P/T)}
\index{Execution!StateSpace!pnxdd}
\begin{center}
   \begin{tabular}{rlc}
      && \multirow{11}{*}{\includegraphics[scale=0.6]{charts/exec_chart_137107419400016_n_19.pdf}} \\
      & \\
      \multicolumn{2}{c}{\acs{pnxdd}, {\bf Execution Summary}} & \\
      \multicolumn{2}{c}{Vasy2003/none (P/T)} & \\
      & \\
      \textcolor{red}{Memory peak: } & \textcolor{red}{2402.77 MB} & \\
      \textcolor{blue}{CPU time: } & \textcolor{blue}{n.a.} & \\
      {End status: } & timeout & \\
      & \\
   \end{tabular}
\end{center}


==> macros-al.tex <==
\makeatletter
\define@choicekey*{result}{reached}[\val\nr]{nc,none,some,best,max}{%
\ifcase\nr\relax%
  \gdef\result@line{}%
  \cellcolor{white}%
\or%
  \gdef\result@number{}%
  \cellcolor{gray!50}%
\or%
  \cellcolor{gray!90}%
\or%
  \cellcolor{black!70}%
  \color{white}%
\or%
  \cellcolor{black}%
  \color{white}%
\fi%
}
\define@choicekey*{result}{typepn}[\val\nr]{no,pt,cn}{%
\ifcase\nr\relax%
  \gdef\result@line{}%
\or%
  \gdef\result@line{\hfill P}%
\or%
  \gdef\result@line{\hfill C}%
\fi%
}
\newcommand\result[2][]{%
  \gdef\result@number{#2}
  \setkeys{result}{#1}%
  \result@number\result@line%
}
\newcommand\legend{%
{%
  \scriptsize
  \begin{tabular}{|p{4em}|cl}
  \cline{1-1}
    \cellcolor{white}
    & & The tool does not participate.
    \\
    \cellcolor{gray!50}
    & & The tool participates, but cannot compute for any scaling value.
    \\
    \cellcolor{gray!90}
    & & The tool participates.
    \\
    \cellcolor{black!70}
    & & The tool participates and reaches the best parameter among tools.
    \\
    \cellcolor{black}
    & & The tool participates and reaches the maximum parameter.
    % \\
    % %$n$ \hfill T
    % & & The tool failed.
%     \\
%     $n$ \hfill 
%     & & The tool fails because of memory exhaustion, after reaching parameter~$n$.
%     \\
% %    $n$ \hfill \Laserbeam
% %    & & The tool fails because of stack overflow, after reaching parameter~$n$.
% %    \\
%     $n$ \hfill \Clocklogo
%     & & The tool fails because of maximum time is elapsed, after reaching parameter~$n$.
    \\
  \cline{1-1}
\end{tabular}
}%
}
\makeatother

